VideoFACT: Detecting Video Forgeries Using Attention, Scene Context, and Forensic Traces

Fake videos represent an important misinformation threat. While existing forensic networks have demonstrated strong performance on image forgeries, recent results reported on the Adobe VideoSham dataset show that these networks fail to identify fake content in videos. In this paper, we show that this is due to video coding, which introduces local variation into forensic traces. In response, we propose VideoFACT - a new network that is able to detect and localize a wide variety of video forgeries and manipulations. To overcome challenges that existing networks face when analyzing videos, our network utilizes both forensic embeddings to capture traces left by manipulation, context embeddings to control for variation in forensic traces introduced by video coding, and a deep self-attention mechanism to estimate the quality and relative importance of local forensic embeddings. We create several new video forgery datasets and use these, along with publicly available data, to experimentally evaluate our network's performance. These results show that our proposed network is able to identify a diverse set of video forgeries, including those not encountered during training. Furthermore, we show that our network can be fine-tuned to achieve even stronger performance on challenging AI-based manipulations.

==> figs/miley_cyrus_example.tex <==
\begin{figure*}[!t]

	\vspace*{-0.5\baselineskip}

    \centering
    \setlength{\fboxsep}{0pt}

    \begin{minipage}[t]{1\textwidth}
        \centering
        \fbox{\includegraphics[width=0.400\textwidth]{{figs/miley_cyrus_example_01.png}}}
        \fbox{\includegraphics[width=0.400\textwidth]{{figs/miley_cyrus_example_01_pred_mask.png}}}
        \smallskip
    \end{minipage}

	\vspace*{-0.1\baselineskip}

    \begin{minipage}[t]{1\textwidth}
        \centering
        \fbox{\includegraphics[width=0.400\textwidth]{{figs/miley_cyrus_example_02.png}}}
        \fbox{\includegraphics[width=0.400\textwidth]{{figs/miley_cyrus_example_02_pred_mask.png}}}
        \smallskip
    \end{minipage}

	\vspace*{-0.1\baselineskip}

    \begin{minipage}[t]{1\textwidth}
        \centering
        \fbox{\includegraphics[width=0.400\textwidth]{{figs/miley_cyrus_example_03.png}}}
        \fbox{\includegraphics[width=0.400\textwidth]{{figs/miley_cyrus_example_03_pred_mask.png}}}
        \smallskip
    \end{minipage}
    
	\vspace*{-0.5\baselineskip}

    \caption{\label{fig:miley_cyrus_example} This figure shows localization results from our proposed network as well as FSG \cite{FSG}, EXIFnet \cite{EXIFnet}, Noiseprint \cite{Noiseprint}, ManTra-Net \cite{ManTra-Net}, and MVSS-Net \cite{MVSS-Net} on six different datasets, VCMS, VPVM, VPIM, Deepfake Video, Inpainted Video and VideoSham \cite{VideoSham}. Our proposed network correctly identifies the manipulated area in videos 
    falsified using a wide variety of forgery operations.
    % with different tampering operations seen during training and ``in-the-wild''.
    }
    
    \vspace*{-0.5\baselineskip}

\end{figure*}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> sections/final/final_00_abstract.tex <==
\begin{abstract}
\label{sec:abstract}

Fake videos represent an important misinformation threat. While existing forensic networks have demonstrated strong performance on image forgeries, recent results reported on the Adobe VideoSham dataset show that these networks fail to identify fake content in videos. In this paper, we propose a new network that is able to detect and localize a wide variety of video forgeries and manipulations. To overcome challenges that existing networks face when analyzing videos, our network utilizes both forensic embeddings to capture traces left by manipulation, context embeddings to exploit forensic traces' conditional dependencies upon local scene content, and spatial attention provided by a deep, transformer-based attention mechanism. We create several new video forgery datasets and use these, along with publicly available data, to experimentally evaluate our network's performance. These results show that our proposed network is able to identify a diverse set of video forgeries, including those not encountered during training.  Furthermore, our results reinforce recent findings that image forensic networks largely fail to identify fake content in videos.

\end{abstract}

==> sections/final/final_01_intro.tex <==
\section{Introduction}
\label{sec:introduction}

Detecting fake and manipulated media is critical in the fight against misinformation. This has become an important challenge as recent advances in AI, such as deepfakes~\cite{ObamaDeepFake, DeepFaceLab, Pix2Pix, CondGAN, CycleGAN}, generative adversarial networks (GANs)~\cite{StarGAN, StyleGAN, StyleGAN2, StyleGAN3, GFP-GAN, StyleFlow, Goodfellow_2020_ACM}, and diffusion models~\cite{GLIDE, StableDiff, LatentDiff, CascadeDiff, VariationalDiff, DALLE2}, have enabled the creation of visually realistic fake images and videos.

In response to this, significant research has been devoted to developing media forensic approaches capable of detecting image and video forgeries.  These techniques operate by exploiting anomalous forensic traces left by manipulation or content falsification. Most existing forensics research has focused on detecting image forgeries.  Several  networks have achieved strong reported performance detecting and localizing fake content in images by directly learning to detect several known forgery types~\cite{Bayar_2018_TIFS, Zhou_2018_CVPR, Yang_2020_ICME, Zhang_2020_TIFS, Marra_2020_IEEEA, Yu_2019_IEEEA, Matern_2020_ICASSP, Bunk_2017_CVPRW, Bappy_2017_ICCV, Hu_2020_ECCV}, or by searching for localized anomalies in an image's forensic traces~\cite{Noiseprint, EXIFnet, FSG, MVSS-Net, ManTra-Net}.

\input{figs/front_page_graphics}

By contrast, comparatively little work has focused on video. Furthermore, the majority of existing video forensics research is devoted to detecting deepfakes.  Several successful deepfake detection networks have been developed~\cite{Wang_2019_ICCV, Guera_2018_AVSS, Zhao_2021_CVPR, Luo_2021_CVPR, Yang_2019_ICASSP, Jiang_2020_CVPR, Huang_2022_TIFS, Hsu_2020_JAS}.  However, many fake videos are not deepfakes and do not contain manipulated human faces.  Deepfake detectors are unable to protect against these types of video forgeries.

Often, it is assumed that image forensic networks will perform well when used to individually analyze each frame in a video as if it were an image.  Surprisingly, however, results presented in this paper as well as recent benchmarking results obtained by Adobe Research on its VideoSham dataset~\cite{VideoSham} show that these networks largely fail when applied to videos.  As a result, there is a significant gap in the ability to detect a wide variety of fake videos.

In this paper, we propose a new network designed to detect a wide variety of video forgeries and manipulations. We name our network VideoFACT: Video Forensics using Attention, Context, and Traces. To overcome challenges that existing networks face when analyzing video,  we observe that scene content has an important influence on the quality and quantity of local forensic information.  Prior work has shown that some regions contain more forensic information of higher quality, while others contain little-to-no forensic information~\cite{chu2015information, pasquini2018information, schlogl2021forensicability}.  As a result, forensic traces have implicit dependencies on the scene content in the region from which they are extracted. Similarly, editing and falsification does not occur in random, independent spatial positions throughout a scene.  Instead, a scene is typically modified to edit, add, or remove an object.  As a result, in falsified content, forensic traces implicitly depends on spatial information.

VideoFACT is explicitly designed to exploit forensic traces' contextual dependencies upon scene content as well as spatial dependencies. We accomplish this by producing both low-level forensic feature embeddings and low-level context embeddings for each local analysis region.  These context embeddings provide information that accounts for variations in the forensic embeddings due to scene content. We leverage both embeddings by using a deep, transformer-based attention module to provide spatial attention information to two different subnetworks that perform frame-level forgery detection and pixel-level forgery localization.

This deep attention mechanism provides our network with multiple benefits. It enables our network to attend to regions with high-quality forensic information while de-emphasizing regions with lower-quality information that may cause false alarms. It is also able to learn and exploit complex relationships between the forensic embeddings, context embeddings, and spatial position to better identify fake content.  We note that recent work has begun to utilize shallow attention mechanisms in forensic networks~\cite{MVSS-Net, ManTra-Net}.  However, as our results in Section~\ref{sec:experiments} show, these shallow mechanisms are unable to produce strong results on video forgeries.  By contrast, our deep transformer-based attention mechanism is able to overcome challenges encountered by prior work and produce strong video forgery detection and localization results.

The main contributions of this work are as follows:
(1) We propose a new network capable of detecting a wide many types of manipulations and fake content in video.
(2) We utilize the novel concept of context embeddings to account for natural variations in forensic traces due to scene content.
(3) We utilize spatial attention, produced by a deep transformer-based attention module, that enables our network to rely more heavily on scene regions with high-quality forensic information while de-emphasizing others with poor information.
(4) We develop multiple new datasets for training and benchmarking video forensic algorithms.  Currently, there are no video forgery datasets made for network training and only the VideoSham dataset for video forgery detection benchmarking.  Our new datasets are composed not only of standard video manipulations such as splicing, but also advanced AI-based content manipulation techniques.
(5) We provide experimental evidence that existing forensic networks designed on images largely fail when used to analyze videos forgeries.
(6) We experimentally demonstrate that our proposed network can detect a wide variety of video forgery and manipulation types.

==> sections/final/final_02_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Most previous work on forgery detection and localization focuses on images. The earliest work on this topic developed hand-designed detectors for specific types of image manipulation detection~\cite{Farid_2005_TSP, Stamm_2008_ICIP, Fridrich_2012_TIFS, Fridrich_2008_TIFS, Kirchner_2008_fast, Popescu_2005_IWIH, Kirchner_2010_TSOP}. Following the rise of deep learning, researchers developed a wide variety of new forensic networks capable of simultaneously identifying a broad range of editing operations~\cite{Bayar_2018_TIFS, Zhou_2018_CVPR, Yang_2020_ICME, Zhang_2020_TIFS, Marra_2020_IEEEA, Yu_2019_IEEEA, Matern_2020_ICASSP, Bunk_2017_CVPRW, Bappy_2017_ICCV, Hu_2020_ECCV}. These algorithms achieve strong performance detecting manipulations that they are trained on, but typically encounter difficulties when confronted with new manipulations outside of the training set. Similar approaches have been developed to detect synthetic image, following the rise of GANs capable of creating realistic fake human faces and objects~\cite{Marra_2018_MIPR, Wang_2020_CVPR, Chandra_2022_ECCV, Yu_2019_ICCV}. 

Most real world manipulated images are made using a combination of multiple editing operations that are unknown to the forensic algorithms at the time of analysis. To address this, researchers have developed approaches that extract local forensic features throughout an image, then search for anomalous traces~\cite{Zenati_2018_ICDM, FSG, EXIFnet, Noiseprint, ManTra-Net, MVSS-Net}. These algorithms have achieved strong performance detecting and localizing fake content in images. Little work has been done to develop similar approaches explicitly for video. There is a rapidly growing body of research devoted to detecting deepfake videos~\cite{Wang_2019_ICCV, Guera_2018_AVSS, Zhao_2021_CVPR, Luo_2021_CVPR, Yang_2019_ICASSP, Jiang_2020_CVPR, Huang_2022_TIFS, Hsu_2020_JAS}.  While these networks are able to successfully detect deepfakes, they cannot be used to detect other video forgeries because they explicitly or implicitly exploit physiological models of the human face or head.  Other work has focused on detecting temporal video manipulations, as opposed to content falsification~\cite{Gonzalez_2022_TITS, Brian_2019_ICASSP}.


==> sections/final/final_03_01_overview.tex <==

We now present VideoFACT, a system for detecting and localizing content forgery in video.
%
Our system includes \textbf{three critical and novel components} that enable us to overcome the negative effects of video coding.
%
\subheader{(1) Video-specific Forensic Feature (VFF)}
We learn forensic features specific to video to capture anomalous traces left by editing. We accomplish this by pre-training a Dedicated Forensic Network to discriminate between source video camera models. Prior research~\cite{Noiseprint, EXIFnet, Splicebuster, Mayer_2018_IHMMS, FSM, FSG} have shown that this process produces features that capture both forensic information about the source and processing history.
%
\subheader{(2) Contextualized Forensic Feature (CFF)}
Differ from forensic features, which is content-agnostic, we introduce context features to model the characteristics of local scene content such as gradient, texture, color, etc. Since video coding parameters implicitly depends on these aspects, we can account for their non-uniform application by contextualizing the forensic features above. We accomplish this by joining the context features with forensic ones for each analysis block.
%
\subheader{(3) Deep Self-Attention Module (DSAM)}
We leverage a Deep Self-Attention Module to examine the intricate relationship between each and every local contextualized forensic traces, and control the effect of non-uniform video coding by emphasizing regions containing high quality forensic traces or potential forgery and de-emphasizing those with low quality traces. 
%
While some existing networks use attention, they use it to weight the relative importance of different forensic features to the overall detection performance. This differs from self-attention, which captures how relevant forensic embeddings are with respect to one another.

A system diagram summarizing our network architecture is shown in Figure \ref{fig:system_overview_diagram}. In the following sections, we will discuss in detail each component of our network.

%We propose VideoFACT for detecting and localizing content forgery in video. Our network includes several critical/novel components that enable us to overcome the negative effects of video coding. 
%
%(1) We use dedicated forensic feature embeddings learned specifically for video to capture anomalous traces left by editing
%Do this by pre-training dedicated forensic network to discriminate between source camera models.  
%Say a little something more about this, but not sure what just yet
%
%(2) We introduce the concept of context embeddings to forensics, and use these to control for natural variation in real content caused by video coding and other effects
%Video coding parameters are dependent upon contextual info, such as scene content
%Distribution of forensic traces can vary depending on context - e.g. scene content, local coding parameters, etc
%Given pre-trained forensic embeddings, we learn context embeddings to capture this relevant contextual information for each patch
%Our network is able to use the info in our context embeddings to account for ..,
%
%(3) We introduce a deep self-attention mechanism that examines the relationship between all local forensic traces, identifies low quality traces relative to others, then de-emphasize these low quality traces so that the do not negatively effect forensic decision making
%to accurately detect anomalies, we shouldn’t look at each trace independently. instead we need to look at forensic traces relative to others within the video to identify anomalous content
%When doing this, we can exploit context info to control for natural variation in unaltered content and identify anomalous traces caused by content forgery
%Use self-attention accomplish this. 
%We note that the use of self-attention (implemented in our network using a transformer) to learn relationships between local forensic embeddings is a novel approach.
%While some existing networks use attention, they use attention to weight the relative importance of certain forensic feature subsets relative to the overall detection performance.  This is different from self-attention, which captures how relevant forensic embeddings are with respect to one another





%An overview of VideoFACT can be seen in Figure~\ref{fig:system_overview_diagram}. Our network first divides a frame into non-overlapping analysis blocks of size $128\times128$ pixels. Next, each block is sent to two parallel low-level feature extractors: one designed to produce forensic feature embeddings $f$ and another that produces context embedding $c$ that captures relevant local information about the scene. A joint set of low-level feature embeddings $x$, which is produced by concatenating the forensic and context embeddings, is passed to a transformer-based attention module, which produces a series of $L$ different spatial attention maps $m_\ell$.  These attention maps are then used to weight the joint feature embeddings by spatial attention. The resulting attention weighted embeddings $y$ are then used by two parallel subnetworks, which independently perform frame-level forgery detection and pixel-level forgery localization.

==> sections/final/final_03_02_low_level_feature_extraction.tex <==
\subsection{Low-Level Feature Extraction}
\label{subsec:low_level_feature_extraction}

VideoFACT's network architecture consists of two low-level feature extractors working in tandem: the Forensic Feature Extractor (FFE) and the Contextual Feature Extractor (CFE). Each analysis block $b_k$ is independently passed through each extractor to produce a forensic feature embedding $f_k$ and a context feature embedding $c_k$.

\subheader{Forensic Feature Embeddings}
We use a CNN $g(\cdot)$ to produce dedicated forensic feature embeddings for each block.  To produce these embeddings, $g$ is pre-trained to discriminate between the source camera model used to capture each block in a separate training set.  This is inspired by an approach widely taken in image forensics, where a CNN trained to discriminate between source camera models is utilized to learn generic forensic feature embeddings~\cite{Noiseprint, EXIFnet, Splicebuster, Mayer_2018_IHMMS, FSM, FSG}.  These embeddings have been shown to capture both forensic information about the source and manipulation or processing history of a block.

We implement $g$ using a MISLnet~\cite{MISLnet} backbone. This network was chosen because it is both lightweight and has been demonstrated to achieve strong performance on several forensic tasks in prior research \cite{FSM, FSG, Bayar_2018_ICASSP, Mayer_2018_ICASSP, MISLgan}. The loss used during the pre-training phase of $g$ is defined as:
\begin{equation}
        \mathcal{L}_{F} = - \sum\nolimits_{\ell=1}^{n}t_{\ell} \cdot log(g(d_k))_{\ell})
\end{equation}
where $n$ is the number of different camera models classes, $t_\ell=1$ if the block $d_k$ was captured by the $\ell^{th}$ camera model and $0$ otherwise. After pre-training, the softmax layer is discarded. This network is not updated during the initial training phase but is allowed to evolve slowly during subsequent fine-tuning phases.

\subheader{Context Feature Embeddings}
The context feature extractor $h(\cdot)$ produces embeddings $c$ that provide information about a scene that contextualizes the forensic embeddings. Prior research has shown that scene content can have important effects on forensic features. Specifically, the amount and quality of forensic information in an analysis window depends on the local illumination, texture, compression parameters, and several other factors~\cite{chu2015information, pasquini2018information, schlogl2021forensicability}. By jointly analyzing forensic and context feature embeddings, later portions of our network can adjust how they interpret forensic features in a particular block to make better forensic decisions. We implement $h$ by using an Xception~\cite{Xception} network backbone that is modified to use only a single middle flow module, followed by a $1\times 1$ layer to reduce the feature embedding dimension. 

\subheader{Joint Feature Extraction}
After obtaining both forensic and context embeddings for each block, we produce the joint feature embeddings $x$ by concatenating $f$ and $c$, i.e.,
\begin{align}
        x_k = \text{Concat}(f_k, c_k)  
\end{align}
This process is repeated for every analysis block in the video frame to produce $N$ arrays of joint feature embedding. Each embedding is 768 elements long.

==> sections/final/final_03_02_low_level_feature_extraction_v1_MCS.tex <==
\subsection{Low-Level Feature Extraction}
\label{subsec:low_level_feature_extraction}

VideoFACT's network architecture consists of two low-level feature extractors working in tandem: the Forensic Feature Extractor (FFE) and the Contextual Feature Extractor (CFE). 
%
Our network first divides a frame into non-overlapping analysis blocks of size $128 \times 128$ pixels.
Each analysis block $b_k$ is independently passed through each extractor to produce a forensic feature embedding $f_k$ and a context feature embedding $c_k$.

\subheader{Forensic Feature Embeddings}
We use a CNN $g(\cdot)$ to produce dedicated forensic feature embeddings for each block.  To produce these embeddings, $g$ is pre-trained to discriminate between the source camera model used to capture each block in a separate training set.  This is inspired by an approach widely taken in image forensics, where a CNN trained to discriminate between source camera models is utilized to learn generic forensic feature embeddings~\cite{Noiseprint, EXIFnet, Splicebuster, Mayer_2018_IHMMS, FSM, FSG}.  These embeddings have been shown to capture both forensic information about the source and manipulation or processing history of a block.

We implement $g$ using a MISLnet~\cite{MISLnet} backbone. This network was chosen because it is both lightweight and has been demonstrated to achieve strong performance on several forensic tasks in prior research \cite{FSM, FSG, Bayar_2018_ICASSP, Mayer_2018_ICASSP, MISLgan}. The loss used during the pre-training phase of $g$ is defined as:
\begin{equation}
        \mathcal{L}_{F} = - \sum\nolimits_{\ell=1}^{n}t_{\ell} \cdot log(g(d_k))_{\ell})
\end{equation}
where $n$ is the number of different camera models classes, $t_\ell=1$ if the block $d_k$ was captured by the $\ell^{th}$ camera model and $0$ otherwise. After pre-training, the softmax layer is discarded. This network is not updated during the initial training phase but is allowed to evolve slowly during subsequent fine-tuning phases.

\subheader{Context Feature Embeddings}
The context feature extractor $h(\cdot)$ produces embeddings $c$ that provide information about a scene that contextualizes the forensic embeddings. Prior research has shown that scene content can have important effects on forensic features. Specifically, the amount and quality of forensic information in an analysis window depends on the local illumination, texture, compression parameters, and several other factors~\cite{chu2015information, pasquini2018information, schlogl2021forensicability}. By jointly analyzing forensic and context feature embeddings, later portions of our network can adjust how they interpret forensic features in a particular block to make better forensic decisions. We implement $h$ by using an Xception~\cite{Xception} network backbone that is modified to use only a single middle flow module, followed by a $1\times 1$ layer to reduce the feature embedding dimension. 

\subheader{Joint Feature Extraction}
After obtaining both forensic and context embeddings for each block, we produce the joint feature embeddings $x$ by concatenating $f$ and $c$, i.e.,
\begin{align}
        x_k = \text{Concat}(f_k, c_k)  
\end{align}
This process is repeated for every analysis block in the video frame to produce $N$ arrays of joint feature embedding. Each embedding is 768 elements long.

==> sections/final/final_03_03_transformer_module.tex <==
\subsection{Transformer-Based Attention Module}
\label{subsec:transformer_module}

The sequence of joint embeddings is passed to the transformer-based attention module, which is designed to produce a series of $L$ different spatial attention maps. To encode spatial position information, a vector of 1-D learnable spatial embeddings is added to the joint embeddings before being passed to the transformer. The transformer consists of twelve transformer encoder blocks stacked on top of one another. The output of the transformer is passed to an ``Attention Squeeze'' layer that consists of $L$, $1\times 1$ convolutional kernels.  This ``squeezes'' down the high dimensional output to a series of $L$ different $M\times N$ spatial attention maps $m_l$. Each entry of the $L$ attention maps $m_l$ corresponds to the network’s attention score for the corresponding joint feature embedding at that position. 

\input{figs/attention_map_example.tex}

Fig.~\ref{fig:spatial_attn_example} shows an example of a spatial attention map produced by our transformer-based attention module, as well as the corresponding the unaltered video frame.  From this example, we can see that VideoFACT attends to regions that contain high-quality forensic traces, i.e. regions with sufficient texture, illumination, etc.  By contrast, regions known to contain low-quality forensic information such as the sky are de-emphasized. Often, these regions will cause false alarms because their low-quality forensic traces will appear anomalous with respect to the rest of the traces throughout the scene.  By not attending to these regions, our network can avoid these false alarms.

==> sections/final/final_03_06_training_protocol.tex <==
\subsection{Multi-Stage Training Protocol}
\label{subsec:training_protocol}

Our network training protocol consists of five stages.  
In the first three stages, the training datasets consist of videos falsified with manipulations that are successively more difficult to detect.  
This enables the network to progressively learn better features by refining those learned in the previous stage. In Stage 1, we use the Video Camera Model Splicing dataset (VCMS), which contains spliced content from other videos.  Because splicing induces source camera inconsistencies within a frame, the forensic embeddings learned by the FFE in the pre-training phase are well suited to identify these manipulations. In Stages 2 and 3,  we train the network with the Video Perceptually Visible Manipulation dataset (VPVM) and Video Perceptually Invisible Manipulation datasets (VPIM), respectively.  These datasets, which are described in Section~\ref{sec:training_datasets},  contain videos manipulated using standard editing operations applied with different strengths.

In the last two stages, we improve the generalizability of our network by training on multiple datasets with varying manipulations and scene content. In Stage 4, we fine-tune the network using all three previous datasets simultaneously (VCMS, VPVM and VPIM). In Stage 5, we further fine-tune the model by incorporating three auxiliary datasets made from images in the Camera Model Identification Database (CMID) first used in \cite{Bayar_2018_ICASSP, MISLnet}. We create these auxiliary training datasets from the CMID, because it captures scenes with different content and distribution than the Video-ACID dataset.  This increases the diversity of data on which our network is trained.  These auxiliary datasets are made using the same process used to create the three video datasets, resulting in one dataset with spliced content (ICMS), one with perceptually visible manipulations (IPVM), and one with perceptually invisible manipulations (IPIM).

==> sections/final/final_04_02_set_b.tex <==
\subsection{Set B: In-the-Wild Manipulated Datasets}

We used three ``in-the-wild'' datasets to evaluate our network: VideoSham~\cite{mittal2022videoSham} created by Adobe Research, and both the Inpainted Video and Deepfake Video datasets created by us.  These datasets contain advanced, challenging manipulations applied to videos with scene content that significantly differs from our training datasets.

\textbf{VideoSham}~\cite{mittal2022videoSham} contains high-quality videos manipulated by professional editors using multiple techniques. Because this work focuses exclusively on identifying fake content, we excluded videos with audio track or temporal manipulations. Additionally, videos of with resolution less than our network’s input size of $1920 \times 1080$ pixels were also excluded. This resulted in 7897 frames from 32 manipulated videos, and 12746 frames from 64 authentic videos.

Our \textbf{Inpainted Video} dataset was made by using inpainting to remove objects specified by segmentation masks from videos in the Densely Annotated Video Segmentation (DAVIS) dataset~\cite{pont2017DAVIS}.  Inpainting was performed with E2FGVI-HQ~\cite{E2FGVI} using the authors' recommended settings, producing output videos in 540p resolution.  They were then resized to 1080p so that they could be analyzed by our network.  This dataset contains  both authentic and manipulated subsets that each contain  of 9312 frames from 90 videos.

Our \textbf{Deepfake Video} dataset was made by  creating deepfakes from a set of publicly available videos of celebrities downloaded from YouTube.  These deepfakes were generated using DeepFaceLab~\cite{DeepFaceLab} to ensure that all fake videos were of 1080p resolution, created as a video rather than a sequence of individually compressed images, and utilized deepfake creation software that is currently most commonly used in the wild. Our dataset consists of a manipulated subset of 300 frames from 10 high-quality deepfake videos and  an unaltered subset of 300 frames from 10 original videos. We note that this dataset was created to evaluate and demonstrate our network's ability to detect a wide variety of video forgeries.  Our purpose is not to create a dedicated deepfake detector.


==> sections/final/final_05_02_comparison.tex <==
\subsection{Detection and Localization Performance}
\label{subsec:comparison_with_prior_works}

We compared the performance of VideoFACT to several existing image forensic networks including Forensic Similarity Graphs (FSG) \cite{FSG}, EXIFnet \cite{EXIFnet}, Noiseprint \cite{Noiseprint}, ManTra-Net \cite{ManTra-Net}, and MVSS-Net \cite{MVSS-Net}, representing a broad spectrum of successful techniques for performing forgery detection and localization in images. We note that Noiseprint and ManTra-Net do not automatically perform detection.  To fairly compare against these networks, we obtain frame-level detection scores by computing the average normalized per-pixel detection probability.
%
Additionally, we benchmarked against three SOTA deepfake detectors: Efficient ViT (E.ViT), Convolutional Cross Efficient ViT (CCE.ViT), and CNN Ensemble.
%
We also note that these algorithms do not perform localization.

\subheader{Set A: Standard Video Manipulations}
Table \ref{table:results_on_our_datasets} shows the performance of our proposed network and competing networks on the three Standard Video Manipulations datasets in Set A. These results show that VideoFACT achieves the best performance by a large margin on these datasets. The only exception is for  the VCMS dataset, where MVSS-Net's localization performance is slightly better than ours, though still comparable. Except for this case, existing networks largely do no better than a random guess (i.e. $\mbox{mAP}=0.5$ and $\mbox{MCC}=0$).  This phenomenon can be clearly seen in both Table~\ref{table:results_on_our_datasets} and the qualitative results presented in Fig~\ref{fig:localization_results}.  These results reinforce similar findings reported in the VideoSham paper~\cite{VideoSham}, that is, existing networks are unable to adapt to forensic differences between image and video forgeries.

\subheader{Set B: ``In-the-Wild'' Datasets}
Table \ref{table:results_on_itw_datasets} shows the performance of our network and existing networks on the three ``in-the-wild'' datasets, which consists much more complex and challenging forgeries. These results show that VideoFACT uniformly achieves the best detection and localization performance over all three datasets.  By contrast, existing approaches typically fail on these challenging datasets.  This can be observed in the qualitative results presented in Fig.~\ref{fig:localization_results}. These results further solidify our observations on Set A and results reported in the VideoSham paper~\cite{VideoSham} that existing image forensic networks largely fail on falsified videos.

For the Deepfake Video dataset, we note that while our network significantly outperforms image forensic networks, it is unlikely to outperform dedicated deepfake detectors~\cite{Huang_2022_TIFS, Zhao_2021_CVPR, Luo_2021_CVPR, Jiang_2020_CVPR}.  This is because our network doesn't leverage useful semantic information such human face models that deepfake detectors typically do.  Despite this, these results show that our network can still achieve reasonable performance without explicitly training on deepfakes. 

Additionally, we note that videos in the Inpainted Video dataset have been resized up to  1080p resolution.  This is important because it is well-known that rescaling significantly downgrades the quality of forensic information.  Despite this, we can still achieve good detection and localization performance on this dataset. 

The results we obtain on the VideoSham dataset are  influenced by the size of the falsified region in each video.  Some of these videos contain fake content that is much smaller than the size of our network's $128 \times 128$ analysis windows. Our network has a difficult time identifying these forgeries.  Despite this, we still achieve better performance than other existing image forensic networks on this dataset.


==> sections/final/final_05_03_discussion.tex <==
\subsection{Discussion}
\label{subsec:discussion}

From the results presented in Tables~\ref{table:results_on_our_datasets} and \ref{table:results_on_itw_datasets}, we can see that existing approaches, which reported strong performance on image forgeries, largely fail on video.  
There are multiple reasons why this may occur.

\subheader{Effects of Video Compression}
Coding and compression is well-known to have a significant effect on forensic traces~\cite{Kirchner_2010_TSOP, Popescu_2005_ITSP, Bayar_2017_ICASSP}. One key reason why existing networks suffer significant performance decreases on video is likely due to differences between image and video compression.

Existing forgery detection networks are trained and validated using images.  While many of these networks are resilient to JPEG effects, it is important to note that JPEG operates in the same manner throughout an image, irrespective of the underlying scene content. As a result, JPEG has a uniform effect on the forensic traces throughout an image.

By contrast, video compression does not operate in a spatially uniform manner.  Modern  standards like H.264 utilize a large number of macroblock types within a single frame, which are chosen based on the underlying scene content, motion, and several other factors~\cite{H264}. Different macroblock types employ different coding techniques and parameters, resulting in different regional compression strengths throughout a frame.  This can induce localized inconsistencies in forensic traces, which will cause existing networks to incorrectly flag some regions as fake or manipulated.

\subheader{False Alarm Effects}
Another important reason why our network outperforms existing networks is its ability to avoid certain types of false alarms in unmanipulated regions.  An example of this can be seen in Fig.~\ref{fig:falsification_example}. Here, existing networks produce false alarms in different ways that can be grouped according to how each network operates.

One set of existing approaches, such as EXIFnet, FSG, and Noiseprint, identify fake content by searching for anomalous forensic traces.  These networks will produce false alarms in scene regions that contain little forensic information such as the sky.  This is because these networks will often mistake low quality forensic traces for anomalous traces.

Another set of approaches, such as ManTra-Net and MVSS-Net,  seek to learn good forgery detection features by analyzing noise residuals and edge information.  These techniques can false alarm when highly salient foreground objects naturally exhibit different statistics from background objects.  This effect occurs in the man sitting on the rock in Fig.~\ref{fig:falsification_example}.  This natural variation will cause the noise residuals and edge information in the foreground objects to appear anomalous to these networks.

\subheader{How Our Network Overcomes These Effects}
Our network's use of context embeddings and spatial attention enables it to be much more resilient to the effects described above. Our deep attention module allows our network to learn which scene regions contain high quality forensic information. Therefore, VideoFACT relies more heavily on these regions when making decisions and avoid many of the false alarm issues faced by other networks. Additionally, local context information enables our network to control for local variations in forensic traces induced by video compression as well as naturally occurring statistical variations induced by scene content.

\subheader{Failure Cases and Limitations}
We identified several common failure cases experienced by our network by examining videos in the  ``in-the-wild'' datasets. Specifically, our network often miss-detects when: 
(1) The falsified region is very small, in particular when its area is much smaller than our $128\times 128$ pixels analysis window. 
(2) Both the manipulated region and background have similar poor lighting conditions, and 
(3) The manipulated region has been altered by color swaps. 
Additionally, our network has limitations including: 
(1) It doesn't exploit temporal effects or correlations between frames. 
(2) Our current implementation is only suitable for a fixed input video resolution of 1080p.


==> sections/final/final_06_ablation_study.tex <==
\section{Ablation Study}
\label{sec:ablation_study}

We conducted multiple ablation experiments to validate the importance of various components in VideoFACT's architecture. We trained each of the network variants using the same settings as the proposed method and assessed their performance on VideoSham. A summary of our experiments is shown in Table \ref{table:ablation_evaluations}.

\input{tables/results_ablations}

\subheader{Influence of FFE}
Removing FFE, we see the detection mAP drops from 0.691 to 0.646 and localization F1 from 0.258 to 0.209. This shows that the FFE is necessary to boost both performance and generalizability.

\subheader{Influence of CFE}
Without the CFE, every metric has a significant reduction. This shows that contextual information is crucial in the network getting a more comprehensive picture of the video forensic information.

\subheader{Influence of the Transformer-Based Attention Module}
In this model variant, we removed the entire Transformer-Based Attention Module. The joint embeddings were fed directly into the detector and the localizer networks. This variant resulted in a substantial performance drop across the board. The detection metrics suggest that this network only does slightly better than random guess. Therefore, this module is a critical part of VideoFACT.

\subheader{Influence of the Transformer}
We measure the importance of the Transformer itself by replacing it with six fully connected layers with ReLU as the activation function. In this scenario, the model performs at a level close to random guess. Therefore, this cements the necessity of the Transformer for our network.

\subheader{Influence of the Attention Squeeze}
In this scenario, we connect the output of the Transformer directly to the detector and localizer, bypassing the Attention Squeeze component. From Table \ref{table:ablation_evaluations}, we see that this variant underperforms in both detection and localization. Hence, the Attention Squeeze component is essential in boosting the model's generalizability. We also try using 1, 3 (proposed) and 10 attention maps.  Results show that using 3 attention maps yields the best performance.

\subheader{Influence of different Feature Refinement approaches}
Instead of the proposed approach, we concatenate all three sets of weighted spatially contextualized forensic embeddings. Results show that both detection and localization performance drop significantly. Therefore, the proposed method is the optimal choice.


==> sections/revisions/00_abstract_v0_Tai.tex <==
\begin{abstract}
\label{sec:abstract}

With the proliferation of fake and manipulated videos, detecting such content has become an important problem in the field of media forensics. 
While existing forensic networks have shown strong performance on images, they do not work on videos, as highlighted in the benchmarks of the Adobe VideoSham dataset. 
This phenomenon is largely caused by non-uniform video compression, which 
introduces local variations in forensic traces, and 
decreases the quality of forensic traces in regions with stronger compression. 
Therefore, in this paper, we propose VideoFACT, a general video content forgery detection and localization network, that addresses negative effects of video compression by
leveraging the conditional dependencies of forensic traces on scene context to account for the natural variation in forensic traces,
and using a Deep Self-Attention Module to control for the difference in the quality of localized forensic traces.
We also present new datasets and a novel training procedure that enable our network to generalize to many manipulations not seen during training. 
Our results demonstrate that 
(1) VideoFACT outperforms existing state-of-the-art forensic methods on video forgery detection and localization, and 
(2) highlight the limitations of image forensic networks in identifying fake content in videos.


\end{abstract}

==> sections/revisions/01_intro_v0_Tai.tex <==
\section{Introduction}
\label{sec:introduction}

%Background on fake videos:
Proliferation of manipulated videos in the age of social media \& digital technologies has become a major concern for society.
With each new \& improved capability to create convincing fake videos, bad actors can easily spread false information, deceive people, and case irreparable harm to individuals and communities.
This has prompted the need for developing reliable and effective methods to detect video forgeries.

\input{figs/front_page_graphics}

%Background on existing forensic algorithms
Traditional forensic algorithms work by extracting hand-crafted features that can capture the differences between authentic and manipulated regions. They often model the divergence in compression artifacts, physical lighting, statistical trace in the frequency domain, local residual prediction and estimation, etc. 
However, due to the fast growing number of attacks and their capability, these methods failed to adapt and were mostly replaced by those which leveraged a deep learning framework. 
Deep neural networks used in forensics currently fall into two categories: forensic classifiers and anomaly detectors. 
Forensic classifiers work by modeling the distribution of forensic traces in authentic images and manipulated images. However, this approach suffers from similar problem as their ancestors: it is not feasible to model every possible manipulation and every images from every camera model. Hence, these approaches often have poor generalizability.
Anomaly detectors, on the other hand, model the joint distribution of forensic traces from each local analysis region of an image so that regions with anomalous content will appear out-of-distribution. And, by doing so, these methods can detect and localize fake content without prior knowledge about the method used and its location in an image. Therefore, they can achieve near perfect score on standard image manipulation datasets (e.g …).

%Introduce the problem and motivation:
However, our experiments and experiments presented in the Adobe Videosham dataset paper show that forensic algorithms, that are designed to work on images, cannot transfer its capability to videos. 
This limitation is due to the fact that these algorithms are ill-equipped to address video coding artifacts introduced into a frame. 
Specifically, video coding is applied non-uniformly within a frame - different parts of a frame can be allocated different amounts of data, depending on their level of detail and the content at similar locations in neighboring frames. 
% Generally, areas containing high detail or high temporal variation require more bits to encode, while areas with low detail or low temporal variation can be encoded with fewer bits. This allows for a more efficient use of bandwidth and results in higher visual quality with less data.
However, this results in inconsistencies in the forensic traces left by the compression process. For example, areas that have been allocated fewer bits may have less detail, resulting in lower-quality forensic traces, and vice versa.
These inconsistencies pose significant challenges for forensic anomaly detection algorithms that rely on consistent quality of forensic traces to identify anomalies within a video frame.

%Introduce the intuition:
One approach to address this problem is to exploit the fact that video coding parameters, such as the bit rate, resolution, and frame rate are dependent upon the scene content being encoded. 
This is because different regions have different levels of complexity and detail, and hence, require different amounts of data to be accurately represented.
Therefore, we can model the variation in video coding parameters, and as a consequence, the variation in forensic traces' quality, by producing context features that captures the characteristics of localized scene content of a frame (e.g. gradients, textures, colors).
As we will show, this is an effective way to account for the inconsistencies in forensic traces' quality caused by non-uniform compression. 
%By providing additional information to forensic anomaly detection algorithms, it is possible to improve the accuracy of the analysis and reduce false positives.

%Introduce the novelty:
In this paper, we introduce VideoFACT, an algorithm designed to explicitly exploit forensic traces' dependencies upon scene content and spatial information.
To facilitate this, we first learn video-specific low-level forensic traces by pre-training a dedicated forensic network on discriminating between 30 different camera models.
Then, to preserve feature asymmetry, we use a distinct network architecture for producing low-level context embedding, which provides information that accounts for variations in the forensic embedding due to non-uniform video compression and scene content.
% With these two subnetworks working in parallel, we extract both low-level forensic embedding and low-level context embedding for each local analysis region of a video frame.
Hence, for each analysis block, we form the contextualized forensic embedding by joining the context embedding with the forensic embedding.
Then, we condition this combined embedding by feeding it into a Deep Self-Attention Module.
This module examines the intricate relationship between all embeddings and produces attention maps which controls the effect of video coding by emphasizing regions containing high quality forensic traces or potential forgery and de-emphasizing those with low quality traces.
Finally, the conditioned contextualized forensic embeddings are analyzed separately by two distinct sub-networks: one producing a frame-level detection score, and the other producing a pixel-level forgery localization binary mask.

%In order for our network to generalize to a wide variety of content manipulations, we also present a novel training procedure, SMCM - Sucessively More Challenging Manipulations. 
%Due to the fact that there are seeming infinite combinations of forgery type, strength and size, a network exposed to manipulations that are too difficult to detect may collapse and overfit to forensically un-related traces. 
%Therefore, to control this, we expose the network to gradually more challenging manipulations. 
%We will show that, by finetuning our network on very little data of a specific task, we can reliably detect advanced manipulations like Deepfake and Inpainting on publicly available datasets. 

Overall, the following \textbf{contributions} are made in this paper:
\textbf{(1)} We develop a system that effectively detects and localizes content forgery in videos, specifically designed to counteract the impact of non-uniform video compression.
\textbf{(2)} We learn video-specific forensic feature to capture anomalous traces left by editing.
\textbf{(3)} We introduce the new concept of context features to forensics, and use these to account for variation in forensic traces' quality caused by non-uniform video compression.
\textbf{(4)} Unlike prior work which uses attention for direct forgery classification, we use a Deep Self-Attention mechanism to model the intricate relationships between each and every local analysis region and control the effect of non-uniform video coding by emphasizing regions with high quality forensic traces or potential forgery and de-emphasizing those with low quality traces.
\textbf{(5}) Extensive experiments on public datasets, and datasets we created show that VideoFACT learns superior feature for anomaly detection in video due to its understanding of the dependencies between forensic traces and scene context.
\textbf{(6)} Finally, we demonstrate that finetuning VideoFACT on very small amount of video data of an advanced manipulation like DeepFakes or Inpainting can achieve close to state-of-the-art performance of networks solely designed for such task. Particularly, (.....).


==> sections/revisions/01_intro_v1_MCS.tex <==
\section{Introduction}
\label{sec:introduction}

Detecting fake and manipulated content in videos is critical in the fight against misinformation, online fraud, and many other threats.  
%
While deepfake videos, i.e. AI-generated videos that falsify the face of a humane speaker with that of another, have caught the public's attention, deepfakes are far from the only form of video forgeries.  
Many forms of video 
Traditional  editing software enables users to convincingly add, remove, and alter  virtually any object in a video.  Furthermore, recent advances in AI-based video editing have caused dramatic advancements in how videos can be falsified.  For example, AI-based video inpainting makes it possible to seamlessly remove an object from a video and replace it with a visually convincing background.

To combat against this, researchers have invested significant effort into building media forensic techniques to identify media forgeries.  Several successful deepfake detection networks have been developed to comabt against this specific fake video threat~\cite{Wang_2019_ICCV, Guera_2018_AVSS, Zhao_2021_CVPR, Luo_2021_CVPR, Yang_2019_ICASSP, Jiang_2020_CVPR, Huang_2022_TIFS, Hsu_2020_JAS}.   

Deepfake detectors, however, are only designed to identify falsified video of human faces and are unable to detect general video editing or content forgery.   In parallel, a large body of research has been developed to detect general editing or content falsification in images.  Several  networks have achieved strong reported performance detecting and localizing fake content in images by directly learning to detect several known forgery types~\cite{Bayar_2018_TIFS, Zhou_2018_CVPR, Yang_2020_ICME, Zhang_2020_TIFS, Marra_2020_IEEEA, Yu_2019_IEEEA, Matern_2020_ICASSP, Bunk_2017_CVPRW, Bappy_2017_ICCV, Hu_2020_ECCV}, or by searching for localized anomalies in an image's forensic traces~\cite{Noiseprint, EXIFnet, FSG, MVSS-Net, ManTra-Net}.

Often, it is assumed that image forensic networks will perform well when used to individually analyze each frame in a video as if it were an image.  Surprisingly, however, results presented in this paper as well as recent benchmarking results obtained by Adobe Research on its VideoSham dataset~\cite{VideoSham} show that these networks largely fail when applied to videos.  As a result, there is a significant gap in the ability to detect a wide variety of fake videos.


\hrulefill



%Detecting fake and manipulated media is critical in the fight against misinformation. This has become an important challenge as recent advances in AI, such as deepfakes~\cite{ObamaDeepFake, DeepFaceLab, Pix2Pix, CondGAN, CycleGAN}, generative adversarial networks (GANs)~\cite{StarGAN, StyleGAN, StyleGAN2, StyleGAN3, GFP-GAN, StyleFlow, Goodfellow_2020_ACM}, and diffusion models~\cite{GLIDE, StableDiff, LatentDiff, CascadeDiff, VariationalDiff, DALLE2}, have enabled the creation of visually realistic fake images and videos.

I%n response to this, significant research has been devoted to developing media forensic approaches capable of detecting image and video forgeries.  These techniques operate by exploiting anomalous forensic traces left by manipulation or content falsification. Most existing forensics research has focused on detecting image forgeries.  Several  networks have achieved strong reported performance detecting and localizing fake content in images by directly learning to detect several known forgery types~\cite{Bayar_2018_TIFS, Zhou_2018_CVPR, Yang_2020_ICME, Zhang_2020_TIFS, Marra_2020_IEEEA, Yu_2019_IEEEA, Matern_2020_ICASSP, Bunk_2017_CVPRW, Bappy_2017_ICCV, Hu_2020_ECCV}, or by searching for localized anomalies in an image's forensic traces~\cite{Noiseprint, EXIFnet, FSG, MVSS-Net, ManTra-Net}.

\input{figs/front_page_graphics}

%By contrast, comparatively little work has focused on video. Furthermore, the majority of existing video forensics research is devoted to detecting deepfakes.  Several successful deepfake detection networks have been developed~\cite{Wang_2019_ICCV, Guera_2018_AVSS, Zhao_2021_CVPR, Luo_2021_CVPR, Yang_2019_ICASSP, Jiang_2020_CVPR, Huang_2022_TIFS, Hsu_2020_JAS}.  However, many fake videos are not deepfakes and do not contain manipulated human faces.  Deepfake detectors are unable to protect against these types of video forgeries.

Often, it is assumed that image forensic networks will perform well when used to individually analyze each frame in a video as if it were an image.  Surprisingly, however, results presented in this paper as well as recent benchmarking results obtained by Adobe Research on its VideoSham dataset~\cite{VideoSham} show that these networks largely fail when applied to videos.  As a result, there is a significant gap in the ability to detect a wide variety of fake videos.

In this paper, we propose a new network designed to detect a wide variety of video forgeries and manipulations. We name our network VideoFACT: Video Forensics using Attention, Context, and Traces. To overcome challenges that existing networks face when analyzing video,  we observe that scene content has an important influence on the quality and quantity of local forensic information.  Prior work has shown that some regions contain more forensic information of higher quality, while others contain little-to-no forensic information~\cite{chu2015information, pasquini2018information, schlogl2021forensicability}.  As a result, forensic traces have implicit dependencies on the scene content in the region from which they are extracted. Similarly, editing and falsification does not occur in random, independent spatial positions throughout a scene.  Instead, a scene is typically modified to edit, add, or remove an object.  As a result, in falsified content, forensic traces implicitly depends on spatial information.

VideoFACT is explicitly designed to exploit forensic traces' contextual dependencies upon scene content as well as spatial dependencies. We accomplish this by producing both low-level forensic feature embeddings and low-level context embeddings for each local analysis region.  These context embeddings provide information that accounts for variations in the forensic embeddings due to scene content. We leverage both embeddings by using a deep, transformer-based attention module to provide spatial attention information to two different subnetworks that perform frame-level forgery detection and pixel-level forgery localization.

This deep attention mechanism provides our network with multiple benefits. It enables our network to attend to regions with high-quality forensic information while de-emphasizing regions with lower-quality information that may cause false alarms. It is also able to learn and exploit complex relationships between the forensic embeddings, context embeddings, and spatial position to better identify fake content.  We note that recent work has begun to utilize shallow attention mechanisms in forensic networks~\cite{MVSS-Net, ManTra-Net}.  However, as our results in Section~\ref{sec:experiments} show, these shallow mechanisms are unable to produce strong results on video forgeries.  By contrast, our deep transformer-based attention mechanism is able to overcome challenges encountered by prior work and produce strong video forgery detection and localization results.

The main contributions of this work are as follows:
(1) We propose a new network capable of detecting a wide many types of manipulations and fake content in video.
(2) We utilize the novel concept of context embeddings to account for natural variations in forensic traces due to scene content.
(3) We utilize spatial attention, produced by a deep transformer-based attention module, that enables our network to rely more heavily on scene regions with high-quality forensic information while de-emphasizing others with poor information.
(4) We develop multiple new datasets for training and benchmarking video forensic algorithms.  Currently, there are no video forgery datasets made for network training and only the VideoSham dataset for video forgery detection benchmarking.  Our new datasets are composed not only of standard video manipulations such as splicing, but also advanced AI-based content manipulation techniques.
(5) We provide experimental evidence that existing forensic networks designed on images largely fail when used to analyze videos forgeries.
(6) We experimentally demonstrate that our proposed network can detect a wide variety of video forgery and manipulation types.

==> sections/revisions/02_effect_of_video_coding_v0_Tai.tex <==
\section{Effect of Video Coding}
\label{sec:effect_of_video_coding}

Video coding is essential in compressing video data to reduce storage and transmission costs. 
%
However, this compression process introduces artifacts into the video frames that can interfere with forensic analysis and make existing anomaly-based approaches fail on videos. 
%
Specifically, lossy video codecs like H.264 employ various techniques such as predictive coding, rate control, and macroblock types to compress frames efficiently.
%
This is significantly different and more complex than image codecs like JPEG.
%
Moreover, in order to get high degree of compression while maintaining visual fidelity, video coding is applied non-uniformly within a frame.
%
This is because different regions of a frame have different levels of complexity and detail, and hence, require different amounts of data to be accurately represented. 
%
%For example, scenes with high motion or complex detail, such as action scenes or scenes with intricate patterns, require higher bit rates to maintain visual quality and avoid compression artifacts. On the other hand, scenes with low motion or simple detail, such as a static shot of a landscape, can be encoded at lower bit rates without significant loss of visual quality.
%
Therefore, this introduce uneven compression traces spatially across a frame. 
%
As a result, existing forensic algorithms trained on images may operate incorrectly because it does not recognize video-specific traces, and algorithms, which rely on computing the similarity distance between patches, may become desensitized and unable to distinguish between 2 patches coming from different forensic regions.

\input{figs/effect_of_video_coding}

To illustrate this effect of video coding the distribution of forensic traces, we perform an experiment shown in Figure \ref{fig:effect_of_video_coding}. We used images from the Columbia dataset and two anomaly detection network, FSG and Noiseprint. Let the image $I$ be divided into patches $X=\{X_1...X_N\}$, in which $Q=\{Q_1...Q_N\}$ represents the patch label (authentic=0 or forged=1). We then compute the distribution of pair-wise forensic feature distances of authentic image regions, $P_{auth\_auth} = Histogram(D(X_i, X_j)), \{\forall i, j \in Q | Q_i=Q_j=0\}$, and of across forged regions, $P_{auth\_forged} = Histogram(D(X_i, X_j)), \{\forall i, j \in Q | Q_i=0, Q_j=1\}$, before and after video compression. We can see that, after images undergo video compression, $P_{auth\_auth}$ and $P_{auth\_forged}$ were altered such that they become indistinguishable.
%
This shows that forensic features in existing anomaly detection networks are no longer effective in videos. 


%(Paragraph 1)
%While existing anomaly-based approaches are SOTA for detecting forgeries, they all fail when applied to video
%This is because video does 
%The two things we described in the intro, but repeat with more detail
%(1) Introduces local variation into forensic traces.  
%How - coding parameters & strength is not uniformly applied throughout frame, but instead varies by macroblock (unlike images)
%Effect - introduces seemingly anomalous forensic traces into authentic frames that cause existing approaches to false alarm
%(2) Reduces quality of forensic traces in some regions
%How - some regions are “more compressed” than others due to locally variable coding strength.  Stronger local coding reduces quality of local forensic traces
%Effect - Low quality local forensic traces can cause forensic algorithms to make incorrect decision (both missed detection and false alarm)
%
%(Paragraph 2)
%We can see these effects by examining the example shown in Fig. X
%This figure shows the distribution of pairwise forensic embedding differences between two patches in an authentic image (or w/ new experiment - authentic image regions) as well as in a fake image (new experiment - across fake region)
%Produced by two leading algorithms on the widely used Y dataset
%Large differences correspond to anomalous forensic traces caused by content forgery
%We can see from this figure, that video coding changes the distribution of these differences such that fake content can no longer be identified by these algorithms


==> sections/revisions/02_related_work_v0_Shengbang.tex <==
\section{Background and Related Work}
\label{sec:related_work}

For decades, researchers have developed multiple passive forensic algorithms to fight against the forgery contents in images and videos. 
% cite from overview paper.
These algorithms includes traditional methods utilizing signal-processing techniques and recent deep-learning based methods. 

\subheader{Traditional Signal-Processing-Based Methods}
Signal processing method has widely being studied by researchers. Researchers develop many types of image forensic algorithms using signal processing methods to extract forensic features~\cite{}. Inspired by image forensics, researchers also develop forensic algorithms for early video~\cite{}. Previous research on video forgery utilize compression artifacts~\cite{a bunch}, noise residues~\cite{a bunch}, motion residues~\cite{a bunch}, and other statistical features~\cite{a bunch}. These algorithms either focus on specific types of forgeries, or only applied to early video codec with consistent compression like MPEG-2.  

\subheader{Deep-Learning-Based Methods}
% cite: A comprehensive survey on passive techniques for digital video forgery detection, A comprehensive survey on state-of-the-art video forgery detection techniques
Until recent, very few techniques are designed so far that can detect the general forgeries in the video with the help of machine/deep learning ~\cite{}, especially on the videos with popular H.264 codec. Existing deep-learning based algorithms can only detect or localize specific types of falsified contents. For example, many deep learning algorithms are developed for detecting synthetic contents like deepfakes ~\cite{}. But these algorithms cannot generalize to detecting other video forgeries. 

\subheader{Anomaly Detection in Image} 
Currently, the most relevant deep learning methods for general video forgery detection are algorithms using anomaly detection on images~\cite{placeholder}, although these algorithms are not designed to performs on videos. These algorithms are designed to implicitly or explicitly detect the out-of-group forensic features within an image to perform forgery detection and localization. 
Specifically, Forensic Similarity Graph~\cite{}, EXIF-Net~\cite{}, and Noiseprint~\cite{} do this by divided the full-size image into small patches, then compute patch-wise difference of forensic features and cluster patches into real and fake groups. 
ManTraNet~\cite{} computes the anomaly score by measuring the consistencies (distance) of the features within
a kernel. MVSS-Net~\cite{} scores the consistencies of the features within an analysis window but it uses a pyramidal resolution approach.
%Although these algorithms achieves good performance in images, where compression effects are consistent through the whole image, our experiments show that dynamic video codec like H.264 can significantly reduce their performance in frame level.


\begin{comment}
\subheader{Traditional forensic methods}
% (Explain forensic traces HERE)
Steganography -> forensitc traces = content independent features that is able to show the processing history of an image or a patch of an image.

\subheader{Forensic classifiers}
% (Deep learning methods which model the distribution of authentic vs manipulated forensic traces)
Can’t feasibly hand-craft perfect features for each manipulation -> use deep learning to automatically learn a set of good forensic traces that can model authentic and manipulated images.
However, can’t feasibly train a model for every manipulation.

\subheader{Anomaly detectors}
% (Deep learning methods which model the joint distribution of traces to detect anomalies)
No need to obtain specific traces for each manipulation, but representations that best separate regions with different underlying forensic traces.
This is achieved by implicitly or explicitly computing the distance or similarity distance of two patches within a frame. 
ManTra-Net computes the anomaly score using a modification of Average Pooling called ZPool2D. This pooling layer measures the consistencies (distance) of the features within a kernel.
MVSS-Net also scores the consistencies of the features within an analysis window but it uses a pyramidal resolution approach called ``Multi-view Feature Learning'', with each stage’s analysis window being widened by four fold.
Noiseprint computes the distance of two patches using the Euclidean distance between their computed residuals.
FSG computes the similarity score between two patches using a learned forensic similarity metric 
And similarly, EXIF-Net uses a learned ``metadata'' similarity score.
In general, all of these methods try to cluster regions with similar characteristics close together and push those with different characteristics far apart.
\end{comment}

==> sections/revisions/02_related_work_v0_Tai.tex <==
\section{Background and Related Work}
\label{sec:related_work}

\subsection{Existing Forensic Approaches}
\subheader{Traditional forensic methods}
% (Explain forensic traces HERE)
Steganography -> forensitc traces = content independent features that is able to show the processing history of an image or a patch of an image.

\subheader{Forensic classifiers}
% (Deep learning methods which model the distribution of authentic vs manipulated forensic traces)
Can’t feasibly hand-craft perfect features for each manipulation -> use deep learning to automatically learn a set of good forensic traces that can model authentic and manipulated images.
However, can’t feasibly train a model for every manipulation.

\subheader{Anomaly detectors}
% (Deep learning methods which model the joint distribution of traces to detect anomalies)
No need to obtain specific traces for each manipulation, but representations that best separate regions with different underlying forensic traces.
This is achieved by implicitly or explicitly computing the distance or similarity distance of two patches within a frame. 
ManTra-Net computes the anomaly score using a modification of Average Pooling called ZPool2D. This pooling layer measures the consistencies (distance) of the features within a kernel.
MVSS-Net also scores the consistencies of the features within an analysis window but it uses a pyramidal resolution approach called ``Multi-view Feature Learning'', with each stage’s analysis window being widened by four fold.
Noiseprint computes the distance of two patches using the Euclidean distance between their computed residuals.
FSG computes the similarity score between two patches using a learned forensic similarity metric 
And similarly, EXIF-Net uses a learned ``metadata'' similarity score.
In general, all of these methods try to cluster regions with similar characteristics close together and push those with different characteristics far apart.


==> sections/revisions/02_use_of_attention_v0_Tai.tex <==
\subsection{Use of Attention Mechanisms in Forensics}

The attention mechanism works by assigning different weights to different parts of the input data, based on their relevance to the task at hand. In the context of forensic networks, this mechanism can be used to fuse features from different layers of the network, by assigning higher weights to more relevant features.

This technique is recently employed by forensic networks such as MVSS-Net, which uses a Dual-Attention (DA) mechanism (spatial and channel). While DA helps MVSS-Net achieve good performance on image manipulation datasets, a draw back of this mechanism is that it is not designed to model the forensic relationship between different analysis region.
%
Hence, in forgery where this relationship matters, (e.g. the forgery is inside a background region, not in a salient foreground object where edge information can be heavily leveraged) the network often false alarm by latching on salient foreground objects.
%Since the purpose of this attention mechanism is to classify spatial locations containing anomalies within the fused features, it . 

To address the lack of context understanding in shallow attention mechanism, the self-attention mechanism was introduced. This mechanism looks at how relevant different parts of the input are to each other instead of how relevant different parts of the input are to the task at hand.
%
Because of this, our proposed approach, VideoFACT, employ a deep self-attention mechanism in order to model the intricate relationship between different local analysis regions.
%
This relationship allow us to control the negative effects of non-uniform video coding and obtain superior performance in detecting video forgery.




==> sections/revisions/05_03_discussion_v0_MCS.tex <==
\subsection{Discussion}
\label{subsec:discussion}

From the results presented in Tables~\ref{table:results_on_our_datasets} and \ref{table:results_on_itw_datasets}, we can see that existing approaches, which reported strong performance on image forgeries, largely fail on video.  
There are multiple reasons why this may occur.

The first reason, as mentioned before, is the effects of video compression. The dynamic video compression is very different from static image compression algorithms, which induce localized inconsistencies in forensic traces.

\begin{comment}
\subheader{Effects of Video Compression}
Coding and compression is well-known to have a significant effect on forensic traces~\cite{Kirchner_2010_TSOP, Popescu_2005_ITSP, Bayar_2017_ICASSP}. One key reason why existing networks suffer significant performance decreases on video is likely due to differences between image and video compression.

Existing forgery detection networks are trained and validated using images.  While many of these networks are resilient to JPEG effects, it is important to note that JPEG operates in the same manner throughout an image, irrespective of the underlying scene content. As a result, JPEG has a uniform effect on the forensic traces throughout an image.

By contrast, video compression does not operate in a spatially uniform manner.  Modern  standards like H.264 utilize a large number of macroblock types within a single frame, which are chosen based on the underlying scene content, motion, and several other factors~\cite{H264}. Different macroblock types employ different coding techniques and parameters, resulting in different regional compression strengths throughout a frame.  This can induce localized inconsistencies in forensic traces, which will cause existing networks to incorrectly flag some regions as fake or manipulated.
\end{comment}

Another important reason is the false alarms effects in unmanipulated regions.  An example of this can be seen in Fig.~\ref{fig:falsification_example}. Here, existing networks produce false alarms in different ways that can be grouped according to how each network operates.
%
One set of existing approaches, such as EXIFnet, FSG, and Noiseprint, identify fake content by searching for anomalous forensic traces. These networks will produce false alarms in scene regions that contain low-quality forensic information such as the sky, which is consistent with previous research~\cite{FSM}.
%
Another set of approaches, such as ManTra-Net and MVSS-Net,  seek to learn good forgery detection features by analyzing noise residuals and edge information.  These techniques can false alarm when highly salient foreground objects naturally exhibit different statistics, like sharper edges, from background objects. This effect occurs in the man sitting on the rock in Fig.~\ref{fig:falsification_example}.

\subheader{How Our Network Overcomes These Effects}
Our network's use of context embeddings and spatial attention enables it to be much more resilient to the effects described above. Our deep attention module allows our network to learn which scene regions contain high quality forensic information. Therefore, VideoFACT relies more heavily on these regions when making decisions and avoid many of the false alarm issues faced by other networks. Additionally, local context information enables our network to control for local variations in forensic traces induced by video compression, as well as naturally occurring statistical variations. % could be just focu length

\subheader{Failure Cases and Limitations}
We identified several common failure cases experienced by our network by examining videos in the  ``in-the-wild'' datasets. Specifically, our network often miss-detects when: 
(1) The falsified region is very small, in particular when its area is much smaller than our $128\times 128$ pixels analysis window. 
(2) Both the manipulated region and background have similar poor lighting conditions, and 
(3) The manipulated region has been altered by color swaps. 
Additionally, our network has limitations including: 
(1) It doesn't exploit temporal effects or correlations between frames. 
(2) Our current implementation is only suitable for a fixed input video resolution of 1080p.


==> sections/revisions_old/00_abstract_v2_MCS.tex <==
\begin{abstract}

%Fake and manipulated media represent an important misinformation threat.  Most existing forensics research has focused on developing networks to detect image forgeries.  Furthermore, existing video forensics research has focused largely on deteting deepfakes.  While deepfake detectors are important tools needed to protect against fake media, many video forgeries are not deepfakes.
% Such as splicing in content, removing objects via inpainting, etc.



Fake %and manipulated 
videos represent an important misinformation threat.  %Existing video forensics research has focused largely on detecting deepfakes.  While deepfake detectors are important tools needed to protect against fake media, many video forgeries are not deepfakes.  
%Furthermore, 
While existing forensic networks have demonstrated strong performance %detecting and localizing 
on 
image forgeries, recent results reported on the Adobe VideoSham dataset show that these networks fail to identify fake content in videos.  
%
In this paper, we propose a new network that is able to detect and localize a wide variety of video forgeries and manipulations. 
%
To overcome challenges that existing networks face when analyzing videos, 
our network utilizes both 
forensic embeddings to capture traces left by manipulation,  
context embeddings to exploit forensic traces' conditional dependencies upon local scene content,  
and spatial attention provided by a deep, transformer-based attention mechanism.
%
We create several new video forgery datasets and use these, along with publicly available data, to experimentally evaluate our network's performance.
 These results show that our proposed network is able to identify a diverse set of video forgeries, including those not encountered during training.  Furthermore, our results reinforce recent findings that image forensic networks largely fail to identify fake content in videos.

\end{abstract}

% Widely available software has made it easy for anyone to create and distribute fake videos.  This represents an important information security threat. Fake videos are often part of misinformation and disinformation campaigns, can be used to perform social engineering as part of financial crimes, and are frequently used in fake news. Several media forensic techniques have been developed in response to these threats.  The majority of these approaches are either designed to operate on digital images, i.e. by detecting fake content or identifying synthetic images, or exploit learned models of a human face to expose deep fake videos.  While existing forensic techniques perform strongly on images, we have found that these techniques largely fail when used to examine digital videos.  Furthermore, deepfake detectors that perform well on video are not designed to detect fake content that is not a modified human face.  As a result, there is a significant need for techniques that are capable of authenticating digital videos whose content may have been falsified using techniques other than deepfakes (e.g. adding or removing objects, editing writing in a scene, performing local editing, etc.).  In this paper, we propose a new technique to detect and localize fake content in videos.  Our approach uses a specially designed neural network to analyze small blocks within a video frame for evidence of manipulation and forgery.  Our network contains several components designed to overcome the challenges that prior work faces when analyzing video.  Our network extracts not only forensic embeddings designed to capture traces left by editing and falsification, but also context embeddings which can be used to inform local decisions made on forensic information.  Additionally, our network uses a transformer to produce spatial attention maps that scale local forensic and context features so that the network does not attend to image regions that contain low or poor quality forensic information.  We present a series of experiments to verify the performance of our network on a variety of different video forgeries.  Due to a lack of existing video forensic benchmark datasets, we developed a number of new datasets to benchmark our network.  Through our experiments we demonstrate that our network achieves strong performance on a wide variety of video forgeries, including video manipulations not encountered during training.  Additionally, our experiments show that our network significantly outperforms prior forgery detection approaches when they are applied to video.

==> sections/revisions_old/01_intro_v1.tex <==
\section{Introduction}
\label{sec:intro}

% The introduction is where you define the "problem" your study was performed to address, indicate your study goals and research questions, and state why the topic of the study is significant. The background is presented as part of your literature review.

% https://digger-project.com/digger-detecting-video-manipulation-synthetic-media/
% https://www.theverge.com/2019/4/3/18293526/adobe-after-effects-content-aware-fill-remove-unwanted-objects-videos
% https://www.theverge.com/23274291/pixel-6-phones-magic-eraser-how-to
% https://screenrant.com/iphone-remove-photobombers-eraser-like-feature-how/

Our modern world is \textit{besieged} by misinformation. Not only the number of available information manipulation techniques have increased dramatically [cite], but also their ability to generate believable forgeries [cite] has become a nightmare for every agencies around the world [cite]. Any person with a smartphone can run Deepfaking and Face-Swapping algorithms to generate hard-to-detect fake content with little effort. However, we must not forget that deepfakes are only half the story - the other half is just as dangerous and as quickly evolving. Big companies like Google, Apple, and Adobe are publishing AI-powered image/video editting tools [cite], in which users can insert or remove objects, texts, and people with a single click, without \textit{any} proactive actions to hinder bad actors from using them for ill purposes. Hence, it is of utmost importance to develop algorithms to expose \textit{general} manipulations in multimedia content. 

Image forgeries have been carefully studied with many successful algorithms being produced over the years. Traditional statistical methods unveiled evidence of forgeries by analyzing inconsistencies in lighting or physical boundaries using edge detection/object segmentation [cite], or identifying variations in imaging traces that are particular to a camera model or a method of image compression, such as lens aberrations [cite], sensor noise [cite], demosaicing filters [cite], and invisible forensic traces like image residuals [cite]. Since these methods all used human-designed filters, they functioned to a certain degree but quickly failed with new image editting softwares and new camera models. Deep Learning approaches, however, are able to leverage their ability to optimize for the best filters which give the best features for inspecting forgeries. Most state-of-the-art techniques [cite] designed their model to produce \textit{context-agnostic} features that are sensitive to manipulations but \textit{specific} enough to prevent false-alarms.
\cite{ManTra-Net}

% Lots of research has been put to uncovering forgeries in images [cite], but there's currently a lack of reliable systems for detecting and localizing forgeries in videos, especially those with high resolutions. Therefore, this paper presents a deep learning algorithm which can both discriminate authentic video frames from forged ones, and identify the tampered region at the pixel level. 







==> sections/revisions_old/01_intro_v2_MCS.tex <==
% 01_intro_v2_MCS.tex

\section{Introduction}

Detecting fake and manipulated media is critical in the fight against misinformation. This has become an important challenge as recent advances in AI, such as deepfakes~\cite{ObamaDeepFake, DeepFaceLab, Pix2Pix, CondGAN, CycleGAN}, generative adversarial networks (GANs)~\cite{StarGAN, StyleGAN, StyleGAN2, StyleGAN3, GFP-GAN, StyleFlow, Goodfellow_2020_ACM}, and diffusion models~\cite{GLIDE, StableDiff, LatentDiff, CascadeDiff, VariationalDiff, DALLE2}, have enabled the creation of visually realistic fake images and videos.

In response to this, significant research has been devoted to developing media forensic approaches capable of detecting image and video forgeries.  These techniques operate by exploiting anomalous forensic traces left by manipulation or content falsification.  
%Forensic traces correspond to local pixel value relationships induced by editing and other processing operations, such as synthetic content generation~\cite{Zhang_2019_WIFS, Verdoliva_2020_JSTSP, Stamm_2013_IEEEA, Piva_2013_ISRN}.
%
Most existing forensics research has focused on detecting image forgeries.  Several  networks have achieved strong reported performance detecting and localizing fake content in images by directly learning to detect several known forgery types~\cite{Bayar_2018_TIFS, Zhou_2018_CVPR, Yang_2020_ICME, Zhang_2020_TIFS, Marra_2020_IEEEA, Yu_2019_IEEEA, Matern_2020_ICASSP, Bunk_2017_CVPRW, Bappy_2017_ICCV, Hu_2020_ECCV}, or by searching for localized anomalies in an image's forensic traces~\cite{Noiseprint, EXIFnet, FSG, MVSS-Net, ManTra-Net}.

\input{figs/front_page_graphics}

By contrast, comparatively little work has focused on video. Furthermore, the majority of existing video forensics research is devoted to detecting deepfakes.  Several successful deepfake detection networks have been developed~\cite{Wang_2019_ICCV, Guera_2018_AVSS, Zhao_2021_CVPR, Luo_2021_CVPR, Yang_2019_ICASSP, Jiang_2020_CVPR, Huang_2022_TIFS, Hsu_2020_JAS}.  However, many fake videos are not deepfakes and do not contain manipulated human faces.  Deepfake detectors are unable to protect against these types of video forgeries.

Often, it is assumed that image forensic networks will perform well when used to individually analyze each frame in a video as if it were an image.  Surprisingly, however, results presented in this paper as well as recent benchmarking results obtained by Adobe Research on its VideoSham dataset~\cite{VideoSham} show that these networks largely fail when applied to videos.  As a result, there is a significant gap in the ability to detect a wide variety of fake videos.

In this paper, we propose a new network designed to detect a wide variety of video forgeries and manipulations.
%
We name our network VideoFACT: Video Forensics using Attention, Context, and Traces.  
%
To overcome challenges that existing networks face when analyzing video,  we observe that scene content has an important influence on the quality and quantity of local forensic information.  Prior work has shown that some regions contain more forensic information of higher quality, while others contain little-to-no forensic information~\cite{chu2015information, pasquini2018information, schlogl2021forensicability}.  As a result, forensic traces have implicit dependencies on the scene content in the region from which they are extracted.
Similarly, editing and falsification does not occur in random, independent spatial positions throughout a scene.  Instead, a scene is typically modified to edit, add, or remove an object.  As a result, 
%there are implicit spatial dependencies between forensic traces in falsified content.
in falsified content, forensic traces implicitly depends on spatial information.

VideoFACT is explicitly designed to exploit forensic traces' contextual dependencies upon scene content as well as spatial dependencies.
We accomplish this by producing both low-level forensic feature embeddings and low-level context embeddings for each local analysis region.  These context embeddings provide information that accounts for variations in the forensic embeddings due to scene content.
%
%We leverage these forensic and context embeddings  
We leverage both embeddings 
by using a deep, transformer-based attention module to provide spatial attention information to two different subnetworks that perform frame-level forgery detection and pixel-level forgery localization.

This deep attention mechanism provides our network with multiple benefits. It enables our network to attend to regions with high-quality forensic information while de-emphasizing regions with lower-quality information that may cause false alarms. It is also able to learn and exploit complex relationships between the forensic embeddings, context embeddings, and spatial position to better identify fake content.  We note that recent work has begun to utilize shallow attention mechanisms in forensic networks~\cite{MVSS-Net, ManTra-Net}.  However, as our results in Section~\ref{sec:experiments} show, these shallow mechanisms are unable to produce strong results on video forgeries.  By contrast, our deep transformer-based attention mechanism is able to overcome challenges encountered by prior work and produce strong video forgery detection and localization results.

The main contributions of this work are as follows:
(1) We propose a new network capable of detecting a wide many types of manipulations and fake content in video.
(2) We utilize the novel concept of context embeddings to account for natural variations in forensic traces due to scene content.
(3) We utilize spatial attention, produced by a deep transformer-based attention module, that enables our network to rely more heavily on scene regions with high-quality forensic information while de-emphasizing others with poor information.
(4) We develop multiple new datasets for training and benchmarking video forensic algorithms.  Currently, there are no video forgery datasets made for network training and only the VideoSham dataset for video forgery detection benchmarking.  Our new datasets are composed not only of standard video manipulations such as splicing, but also advanced AI-based content manipulation techniques.
(5) We provide experimental evidence that existing forensic networks designed on images largely fail when used to analyze videos forgeries.
(6) We experimentally demonstrate that our proposed network can detect a wide variety of video forgery and manipulation types.



==> sections/revisions_old/02_background_and_problem_formulation_v1.tex <==
\section{Background}
\label{sec:background}

% [{\color{green}{cite}}]

% TODO: What are Foregeries and how it applied to images 
% TODO: How Image Foregeries are detected using "forensic traces"
% TODO: How Video are different from Images
% TODO: How Video Foregeries are different from Image Foregeries
% TODO: Show successful Image Forensic Algorithms
% TODO: Show that these IFAs do not work on Videos Forgeries
% TODO: Explain why they don't work
% TODO: Explain in quick summary how we are addressing the problem
% TODO: How we address the problem: Attack it from all sides: 1) Data, 2) Training Protocol, 3) Model Architecture
% TODO: --> This is our contributions (summarize it very quickly).
% TODO: 



Video forgeries are actions performed on a video which alter any or some of the following: content, speed, and/or audio tracks. Many prior works has been done to detect abnormal temporal changes [{\color{green}{cite}}], and audio replacement/distortions [{\color{green}{cite}}], but little were accomplished to expose generic localizable edits. Although a lot of research has gone into detecting deepfakes by leveraging prior knowledge about the human face's anatomy or behavior (e.g. the locations, shapes, movements, etc.) [{\color{green}{cite}}], these algorithms cannot be used to detect any other manipulation techniques: adding or removing texts/objects, watermarking, video matting, in-painting, color correction, contrast enhancement, noise addition, etc. Therefore, in this paper, we focus solely on solving the problem of detecting and localizing confined manipulations in a video without having any prior knowledge about: the content (what is being edited), the location (where is it edited), and the manipulation technique (how is it edited). In addition, we will only be examining videos encoded in the H.264 format, because different video codecs contain distinct properties, which greatly influence the forensic traces analyzed by video forensic algorithms like ours [{\color{green}{cite}}]. However, we believe our approach is transferable across codecs, but an exhaustive investigation of all possible video codecs is beyond the scope of this work.








==> sections/revisions_old/02_background_and_problem_formulation_v1_Shengbang.tex <==
\section{Related Work}
\label{sec:background}

Most previous work on anomaly detection and localization focuses on images. Earliest work includes hand-designed features for specific types of image manipulation detection~\cite{Stamm_2008_ICIP, Farid_2005_TSP, Fridrich_2012_TIFS, Fridrich_2008_TIFS, Kirchner_2008_fast, Popescu_2005_IWIH, Kirchner_2010_TSOP} are proposed by signal processing community. As deep learning became popular, researchers applied this technique to adaptively identify a broad range of image editing operations~\cite{Bayar_2018_TIFS, Zhou_2018_CVPR, Yang_2020_ICME, Zhang_2020_TIFS, Marra_2020_IEEEA, Yu_2019_IEEEA, Matern_2020_ICASSP, Bunk_2017_CVPRW, Bappy_2017_ICCV, Hu_2020_ECCV}. These algorithms have specific architectural designs for extracting low-level features from images. Additionally, once generative models become ubiquitous, researchers proposed algorithms to detect synthetic image contents~\cite{Marra_2018_MIPR, Wang_2020_CVPR, Chandra_2022_ECCV, Yu_2019_ICCV}. 

However, most manipulated images in the real world are made using a combination of multiple editing operations that are unknown to the forensic algorithms at the time of analysis. To address this, researchers proposed multiple methods to detect image anomalies~\cite{Zenati_2018_ICDM, FSG, EXIFnet, Noiseprint, ManTra-Net, MVSS-Net}. These algorithms are successful in image anomaly detection and localization. However, few works have been done to detect and localize fake content in videos. It is noted that even though lots of work has focused on detecting deepfake and face manipulations in videos~\cite{Wang_2019_ICCV, Guera_2018_AVSS, Zhao_2021_CVPR, Luo_2021_CVPR, Yang_2019_ICASSP, Jiang_2020_CVPR, Huang_2022_TIFS, Hsu_2020_JAS}, these methods explicitly or implicitly exploit physiological model of human face or motions. Hence, they are only designed to detect synthetically generated faces and cannot be used to detect other kinds of manipulation in videos. While other works focus on exposing temporal or audio tampering~\cite{Gonzalez_2022_TITS, Brian_2019_ICASSP}, no existing viable techniques developed to reveal falsified contents in videos. The lack of research on this topic may come from the assumption that: applying image forgery detection and localization algorithms to each video frame will work. As we show in this paper, these algorithms perform poorly on videos, there is an urgent need for viable video-specific detection and localization approaches.


%%%% PREVIOUS VERSION %%%%%

% % Most work has focus on images.
% Most previous work on anomaly detection and localization focus on images.
% % 1. Narrative Earliest work hand Design in manip detectors from Signal Processing Commmunity
% Earliest work includes hand-designed features for specific types of image manipulation detection~\cite{Stamm_2008_ICIP, Farid_2005_TSP, Fridrich_2012_TIFS, Fridrich_2008_TIFS, Kirchner_2008_fast} are proposed by signal processing community.
% % 2. ML techniques have proven more adaptive at identifying a widest of editing
% As deep learning became popular, researchers applied this technique to adaptively identify a broad range of image editing operations~\cite{Bayar_2018_TIFS, Zhou_2018_CVPR, Yang_2020_ICME, Zhang_2020_TIFS, Marra_2020_IEEEA, Yu_2019_IEEEA, Matern_2020_ICASSP}
% %  -- forensic CNN classifiers
% %  -- Lots of research on early layer & whatever ML/CV calls low-level features
% These algorithms have specific architectural design for extracting low-level features from images.
% % 3. Synthetic Image Detector
% Additionally, once generative models become ubiquitous, researchers proposed algorithms to detect synthetic image contents~\cite{Marra_2018_MIPR, Wang_2020_CVPR, Chandra_2022_ECCV}. 
% % 4. Image Forgeries are typically sophisticated made using multiple editting operations that we may not have prior knowledge
% % make image forgery det & loc
% However, a majority of manipulated images in real world are often made using a combination of multiple editing operations that we may not have prior knowledge.
% % -- get local embeddings search for anomalies
% To address this, researchers proposed multiple method to detect image anomalies~\cite{Zenati_2018_ICDM, FSG, EXIFnet, Noiseprint, ManTra-Net, MVSS-Net}. These algorithms have been proven to be successful in image anomaly detection and localization.
% % -- whatever else ML/CV community has

% % 5. Comparatively less wrk on videos
% However, few works have been done to detect and localize fake contents in video. 
% % -- most on Deepfake
% It is noted that even though lots of work has focused on detecting deepfake and face manipulations in videos~\cite{Wang_2019_ICCV, Guera_2018_AVSS, Zhao_2021_CVPR, Luo_2021_CVPR, Yang_2019_ICASSP, Jiang_2020_CVPR, Huang_2022_TIFS, Hsu_2020_JAS}. 
% % -- explicitly or implicitly exploit physiological model of human face / motion
% %    cite lots & say they are good
% , these methods explicitly or implicitly exploit physiological model of human face or motions.
% %    but can only be used to ID fake faces. Can't work on generic vid manipulated object added/removed
% Hence, they are only designed to detect synthetically generated face and cannot be used to detect other kinds of manipulation in videos.
% % 6. small amount of other vidoe forensic work on diff topics
% While there are other works which focus on exposing temporal or audio tampering~\cite{Gonzalez_2022_TITS, Brian_2019_ICASSP}, no existing viable techniques developed to reveal falsified contents in videos. The lack of research on this topic may come from the assumption that: applying image forgery detection and localization algorithms to each frame of a video will work. However, as we show in this paper, these algorithms perform poorly on videos. As a result, there is an urgent need for viable video-specific detection and localization approaches.

% -- Source Cam ID

% -- Speed manipulation

\begin{comment}
Video forgeries are actions performed on a video which alter any or some of the following: content, speed, and/or audio tracks. Many prior works has been done to detect abnormal temporal changes [{\color{green}{cite}}], and audio replacement/distortions [{\color{green}{cite}}], but little were accomplished to expose generic localizable edits. Although a lot of research has gone into detecting deepfakes by leveraging prior knowledge about the human face's anatomy or behavior (e.g. the locations, shapes, movements, etc.) [{\color{green}{cite}}], these algorithms cannot be used to detect any other manipulation techniques: adding or removing texts/objects, watermarking, video matting, in-painting, color correction, contrast enhancement, noise addition, etc. Therefore, in this paper, we focus solely on solving the problem of detecting and localizing confined manipulations in a video without having any prior knowledge about: the content (what is being edited), the location (where is it edited), and the manipulation technique (how is it edited). In addition, we will only be examining videos encoded in the H.264 format, because different video codecs contain distinct properties, which greatly influence the forensic traces analyzed by video forensic algorithms like ours [{\color{green}{cite}}]. However, we believe our approach is transferable across codecs, but an exhaustive investigation of all possible video codecs is beyond the scope of this work.
\end{comment}







==> sections/revisions_old/02_background_and_problem_formulation_v2_MCS.tex <==
\section{Related Work}
\label{sec:background}

Most previous work on forgery detection and localization focuses on images. The earliest work on this topic %involved 
developed 
hand-designed detectors for specific types of image manipulation detection~\cite{Farid_2005_TSP, Stamm_2008_ICIP, Fridrich_2012_TIFS, Fridrich_2008_TIFS, Kirchner_2008_fast, Popescu_2005_IWIH, Kirchner_2010_TSOP}. %are proposed by signal processing community. 
%proposed by the signal processing community.  
%As deep learning became popular, researchers applied this technique to adaptively identify a broad range of image editing operations
Following the rise of deep learning, researchers developed a wide variety of new forensic networks capable of simultaneously identifing a broad range of editing operations~\cite{Bayar_2018_TIFS, Zhou_2018_CVPR, Yang_2020_ICME, Zhang_2020_TIFS, Marra_2020_IEEEA, Yu_2019_IEEEA, Matern_2020_ICASSP, Bunk_2017_CVPRW, Bappy_2017_ICCV, Hu_2020_ECCV}. 
%These algorithms have specific architectural designs for extracting low-level features from images. 
These algorithms achieve strong performance detecting manipulations that they are trained on, but typically encounter difficulties when confronted with new manipulations outside of the training set.
%
Similar approaches have been developed to detect synthetic image, following the rise of GANs capable of creating realistic fake human faces and objects~\cite{Marra_2018_MIPR, Wang_2020_CVPR, Chandra_2022_ECCV, Yu_2019_ICCV}. 
%Additionally, once generative models become ubiquitous, researchers proposed algorithms to detect synthetic image contents~\cite{Marra_2018_MIPR, Wang_2020_CVPR, Chandra_2022_ECCV, Yu_2019_ICCV}. 

Most real world manipulated images are made using a combination of multiple editing operations that are unknown to the forensic algorithms at the time of analysis. 
To address this, researchers have developed approaches that extract local forensic features throughout an image, then search for anomalous traces~\cite{Zenati_2018_ICDM, FSG, EXIFnet, Noiseprint, ManTra-Net, MVSS-Net}.  
%To address this, researchers proposed multiple methods to detect image anomalies 
%These algorithms are successful in image anomaly detection and localization. 
These algorithms have achieved strong performance detecting and localizing fake content in images.  
Little work has been done to develop similar approaches explicitly for video.  
There is a rapidly growing body of research devoted to detecting deepfake videos~\cite{Wang_2019_ICCV, Guera_2018_AVSS, Zhao_2021_CVPR, Luo_2021_CVPR, Yang_2019_ICASSP, Jiang_2020_CVPR, Huang_2022_TIFS, Hsu_2020_JAS}.  While these networks are able to successfully detect deepfakes, they cannot be used to detect other video forgeries because they explicitly or implicitly exploit physiological models of the human face or head.  Other work has focused on detecting temporal video manipulations, as opposed to content falsification~\cite{Gonzalez_2022_TITS, Brian_2019_ICASSP}.

%There is little-to-no existing work explicitly dedicated to detecting and localizing generic video forgeries, likely because it has commonly been assumed that image forensic networks can be successfully used analyze each video frame like an image.  However, very recent results obtained benchmarking image forensic techniques on the Adobe VideoSham dataset~\cite{VideoSham} have demonstrated that image forensic techniques fail when applied to video. 


%The lack of research on this topic may come from the assumption that: applying image forgery detection and localization algorithms to each video frame will work. 
%As we show in this paper, these algorithms perform poorly on videos, there is an urgent need for viable video-specific detection and localization approaches.




%However, few works have been done to detect and localize fake content in videos. It is noted that even though lots of work has focused on detecting deepfake and face manipulations in videos~\cite{Wang_2019_ICCV, Guera_2018_AVSS, Zhao_2021_CVPR, Luo_2021_CVPR, Yang_2019_ICASSP, Jiang_2020_CVPR, Huang_2022_TIFS, Hsu_2020_JAS}, these methods explicitly or implicitly exploit physiological model of human face or motions. Hence, they are only designed to detect synthetically generated faces and cannot be used to detect other kinds of manipulation in videos. While other works focus on exposing temporal or audio tampering~\cite{Gonzalez_2022_TITS, Brian_2019_ICASSP}, no existing viable techniques developed to reveal falsified contents in videos. The lack of research on this topic may come from the assumption that: applying image forgery detection and localization algorithms to each video frame will work. As we show in this paper, these algorithms perform poorly on videos, there is an urgent need for viable video-specific detection and localization approaches.









==> sections/revisions_old/03_attn_feat_refine_v1.tex <==
\subsection{Attention-Informed Feature Refinement}
\label{subsec:attn_informed_feat_refine}

After the transformer-based module produces a set of $L$ attention maps, these maps are used to weight the low-level joint feature embeddings by spatial attention. 
%To accomplish this, t
The joint feature embedding $x_k$ at the $k^{th}$ spatial location is weighted by the corresponding $k^{th}$ entry in the $l^{th}$ attention map. This enables the network to attend to feature embeddings at spatial locations with higher amounts of higher-quality forensic information. This process is repeated for all $L$ spatial attention maps. Then the resulting features are summed to produce the attention-informed features $y$, such that:
\begin{equation}
        y_k = \sum\nolimits_{\ell = 1}^{L} x_k m_{k,l}
\end{equation}



==> sections/revisions_old/03_comb_loss_v1.tex <==
\subsection{Combined Detection and Localization Loss}
\label{subsec:combined_loss}

We trained our model end-to-end by combining both the detection loss, $\mathcal{L}_{d}$, and the localization loss, $\mathcal{L}_{\ell}$, into a single combined loss, $\mathcal{L}_{c}$. 

\textit{The detection loss} is the Binary Cross Entropy loss:
\begin{align}
        \mathcal{L}_{d} = -w \cdot log(I_{d}) + (1 - w) \cdot log(1 - I_{d})
\end{align}
where $w$ is the binary ground-truth frame-level label (0 or 1), and $I_{d}$ is the frame-level prediction probability [0, 1].

Additionally, we gauge the correctness of the model's block-wise localization predictions by comparing them to the ratio of the number of manipulated pixels and total number of pixels in each block:
\begin{align}
        z_{k} = \frac{\sum_{i,j} \mathbbm{1}\cdot u_{i,j}}{\sum_{i,j} 1} , \forall (i,j) \in R_k
\end{align}
where $z_{k}$ is the target probability of block $k$ being manipulated, $R_{k}$ is the set of pixel coordinates corresponding to block $k$, and $u_{i,j}$ is the ground-truth binary label for the pixel at location $(i, j)$. Hence, we can define \textit{the localization loss} as:
\begin{align}
        \mathcal{L}_{\ell} = \sum_{k=1}^{N} -z_{k} \cdot log(b_{p}^k) + (1 - z_{k}) \cdot log(1 - b_{p}^k)
\end{align}

Finally, \textit{the combined loss} is the weighted sum of the detection loss and the localization loss:
\begin{align}
        \mathcal{L}_{c} = \alpha \cdot \mathcal{L}_{d} + (1 - \alpha) \cdot \mathcal{L}_{\ell}
\end{align}
where $\alpha \in (0,1)$ is the weight balancing the importance of the frame-level prediction and the pixel-level predictions.



==> sections/revisions_old/03_det_and_loc_v1.tex <==
\subsection{Detection and Localization}
\label{subsec:detection_and_localization}

Our model's Decision Module performs detection and localization simultaneously by passing the attention-informed embedding vectors, $y$, through the detector network, $p(\cdot)$, and the localizer network, $q(\cdot)$. 

\textit{The detector} consists of two fully connected layers with ReLU activation functions for dimensionality reduction, and a final linear + ReLU stack for mapping the flattened condensed feature embeddings to two decision neurons that outputs a frame-level detection probability, $I_d$:
\begin{align}
        I_d = p(y)
\end{align}

\textit{The localizer} is composed of four $1 \times 1$ layers, with reducing number of output channels: 192, 96, 12, 1. Each layer is activated by the ReLU activation function, except for the last layer, which uses the sigmoid activation function in order to produce probabilities for every block in the input frame:
\begin{align}
        [b_{p}^{1}, b_{p}^{2}, \cdots, b_{p}^{N}] = q(y)
\end{align}

When evaluating our localization results, we produce pixel-level binary masks by intelligently choosing a dynamic threshold based on the distributions of predicted probabilities. Since thresholding sometimes produces holes, we further fill these holes using the flood-fill \citelater{cite} algorithm. Finally, we eliminate outlying regions according to the number of potential manipulated areas and assign the block's final binarized decision to every pixel in that block.



==> sections/revisions_old/03_det_and_loc_v2Shengbang.tex <==
\subsection{Detection and Localization}
\label{subsec:detection_and_localization}

% Our model's Decision Module performs detection and localization simultaneously by passing the attention-informed embedding vectors, $y$, through the detector network, $p(\cdot)$, and the localizer network, $q(\cdot)$.
Our network produces two outputs: a frame-wide detection score and a pixel-level localization mask. The localization mask is disregarded if the detection score does not cross the threshold. 
%
To do this, our network separately analyzes the attention-informed feature embeddings using two different sub-networks for localization and detection. The whole network is trained to optimize the overall loss function, which is a linear combination of the detection and localization losses.
%\textit{The detector} consists of two fully connected layers with ReLU activation functions for dimensionality reduction, and a final linear + ReLU stack for mapping the flattened condensed feature embeddings to two decision neurons that outputs a frame-level detection probability, $I_d$:

\subheader{Detection Network} The detection network $p(\cdot)$ consists of two $1\times1$ Conv + ReLU layers for dimension reduction [{\color{green}{Need the number of kernels}}], followed by a fully connected and a softmax layer to output two neurons. The detection loss for this sub-network is the cross-entropy loss between the label and the predicted output:
\begin{align}
\mathcal{L}_{D} = - \sum_{n=1}^{2} w_n log(p_n)
\end{align}
where $p_n$ is the output of $p(\cdot)$ and the $w_n$ is the one-hot vector indicate whether the video is manipulated.
%\textit{The localizer} is composed of four $1 \times 1$ layers, with reducing number of output channels: 192, 96, 12, 1. Each layer is activated by the ReLU activation function, except for the last layer, which uses the sigmoid activation function in order to produce probabilities for every block in the input frame:
%\begin{align}
%        [b_{p}^{1}, b_{p}^{2}, \cdots, b_{p}^{N}] = q(y)
%\end{align}

\subheader{Localization Network} The localization network $q(\cdot)$ is composed of four $1\times1$ Convolution layers with 192, 96, 12, 1 kernels. We choose ReLU as the activation function except the last layer, which use sigmoid activation function to output block-wise probability of being manipulated.

The localization loss is built on top of this sub-network. We define the localization loss to be the sum of block-wise cross-entropy loss. Which is:
\begin{align}
\mathcal{L}_{L} = \sum_{k=1}^{N} -z_{k} log(q_k) + (1 - z_{k})log(1 - q_k)
\end{align}  
where $q_k$ is the prediction of $q(\cdot)$ for the corresponding block $b_k$, $z_k$ is the true probability of the block being manipulated. Considering a block could have partial manipulated region, we define the $z_k$ as the ratio of manipulated pixels in the ground-truth mask:
\begin{align}
z_{k} = \sum_{i,j \in \mathbbm{P}_k}M_{i,j}\; /\; |\mathbbm{P}_k|
\end{align}
where $\mathbbm{P}_k$ is the set of coordinates of pixels belong to block $k$, and $M$ is the ground-truth binary mask. 

During inference, we perform post-processing on the block-wise prediction to achieve pixel-level predicted mask. We first threshold the block-level prediction probabilities. Typically, there are two peaks in this histogram of block-level probabilities, one due to unaltered blocks and the other due to manipulated blocks. The threshold is chosen as the location of the first minima to the right of the first histogram peak (i.e. the one induced by unaltered blocks). After thresholding, we use the flood-fill morphological algorithm to remove holes from the localization mask. A final pixel-level mask is produced by scaling the block-level mask to the full video frame size using bilinear interpolation.

\subheader{Joint Training}
To train the entire model, we use the total loss $\mathcal{L}$, which is the linear combination of the detection loss and the localization loss:
\begin{align}
        \mathcal{L} = \alpha \cdot \mathcal{L}_D + (1 - \alpha) \cdot \mathcal{L}_L
\end{align}
where $\alpha \in (0,1)$ is the weight to balance the the frame-level detection loss and the block-level localization loss.



==> sections/revisions_old/03_det_and_loc_v3Shengbang.tex <==
\subsection{Detection and Localization}
\label{subsec:detection_and_localization}

% Our model's Decision Module performs detection and localization simultaneously by passing the attention-informed embedding vectors, $y$, through the detector network, $p(\cdot)$, and the localizer network, $q(\cdot)$.
Our network produces two outputs: a frame-level detection score and a pixel-level localization mask. The localization mask is disregarded if the detection score %does not %cross the threshold. 
indicates 
%that forged content is present.
no forged content exists.
%
%To do this, 
Our network separately analyzes the attention-informed feature embeddings using two different subnetworks for localization and detection. 
%The whole network is trained to optimize the overall loss function, which is a linear combination of the detection and localization losses.
%\textit{The detector} consists of two fully connected layers with ReLU activation functions for dimensionality reduction, and a final linear + ReLU stack for mapping the flattened condensed feature embeddings to two decision neurons that outputs a frame-level detection probability, $I_d$:

\subheader{Detection Network} The detection network $p(\cdot)$ consists of two $1\times1$ Conv + ReLU layers for dimension reduction with 200, and 2 kernels, respectively, followed by a fully connected and a softmax layer to output two neurons, one corresponds to pristine and the other corresponds to being falsified. The detection loss for this subnetwork is the cross-entropy loss between the label and the predicted output:
\begin{align}
\mathcal{L}_{D} = - \sum\nolimits_{n=1}^{2} w_n log(p_n)
\end{align}
where $p_n$ is the output of $p(\cdot)$ and the $w_n$ is the one-hot vector indicate whether the video is manipulated.
%\textit{The localizer} is composed of four $1 \times 1$ layers, with reducing number of output channels: 192, 96, 12, 1. Each layer is activated by the ReLU activation function, except for the last layer, which uses the sigmoid activation function in order to produce probabilities for every block in the input frame:
%\begin{align}
%        [b_{p}^{1}, b_{p}^{2}, \cdots, b_{p}^{N}] = q(y)
%\end{align}

\subheader{Localization Network} The localization network $q(\cdot)$ is composed of four $1\times1$ Convolutional layers with 192, 96, 12, and 1 kernel, respectively. 
% We choose ReLU as the activation function except the last layer, which use sigmoid activation function to output block-wise probability of being manipulated.
We use ReLU activation except in the last layer, which uses sigmoid activation to output the block-wise probability of being manipulated.

The localization loss is built on top of this subnetwork. We define the localization loss to be the sum of block-wise cross-entropy loss. Which is:
\begin{align}
\mathcal{L}_{L} = \sum\nolimits_{k=1}^{N} -z_{k} log(q_k) + (1 - z_{k})log(1 - q_k)
\end{align}  
where $q_k$ is the prediction of $q(\cdot)$ for the corresponding block $b_k$, and $z_k$ is the true probability of the block being manipulated. Because a block could contain a partial of manipulated region, we define $z_k$ as the ratio of manipulated pixels in the ground-truth mask:
\begin{align}
z_{k} = \sum\nolimits_{i,j \in \mathbbm{P}_k}M_{i,j}\; /\; |\mathbbm{P}_k|
\end{align}
where $\mathbbm{P}_k$ is the set of pixel coordinates that belong to block $k$, and $M$ is the ground-truth binary mask. 

During inference, we achieve the pixel-level predicted mask from the block-wise prediction. We first threshold the block-level prediction probabilities. Typically, there are two peaks in this histogram of block-level probabilities, one due to unaltered blocks and the other due to manipulated blocks. The threshold is chosen as the location of the first minima to the right of the first histogram peak (i.e. the one induced by unaltered blocks). After thresholding, we use the flood-fill morphological algorithm to remove holes from the localization mask. A final pixel-level mask is produced by scaling the block-level mask to the full video frame size using bilinear interpolation.

\subheader{Joint Training}
To train the entire network, %we use the total loss $\mathcal{L}$, which is the linear combination of the detection loss and the localization loss:
we define the total loss as a linear combination of the detection and localization losses:
\begin{align}
        \mathcal{L} = \alpha  \mathcal{L}_D + (1 - \alpha)  \mathcal{L}_L
\end{align}
where $\alpha \in (0,1)$ is the weight to balance the frame-level detection loss and the block-level localization loss.



==> sections/revisions_old/03_low_level_feature_extraction_v1.tex <==
\subsection{Low-Level Feature Extraction}
\label{subsec:low_level_feature_extraction}

Our network architecture \todolater{replace by net name} has two low-level feature extractors working in tandem - the Forensic Feature Extractor (FFE) and the Contextual Feature Extractor (CFE). Each block $b_k$ is independently passed through each extractor to produce a forensic feature embedding $f_k$ and a context feature embedding $c_k$.
% \begin{align}
%         f_k &= g(b_k) \\
%         c_k &= h(b_k)
% \end{align}

\subheader{Forensic Feature Extraction}
We use a CNN $g(\cdot)$ to produce dedicated forensic feature embeddings for each block. Many prior works in image forensics have proven that training a CNN to discriminate between source camera models enables it to produce generic forensic feature embeddings \citelater{cite a lot}. These embeddings have been shown to capture forensic information about the source camera and a block's manipulation and processing history. Therefore, inspired by this strategy, $g$ is pre-trained to discriminate between the source camera model capturing each block in a separate training set.

We implement $g$ using a MISLnet \citelater{cite} backbone. This network was chosen because it is both lightweight and has been demonstrated to achieve strong performance on several forensic tasks in prior research \citelater{cite a lot}. The loss used during the pre-training phase of $g$ is defined as:
\begin{align}
        \mathcal{L}_{F} &= - \sum_{\ell=1}^{n}t_{\ell} \cdot log(g(d_k))_{\ell})
\end{align}
where $n$ is the number of different camera models classes, $t$ is the target one-hot vector with a $1$ in the $\ell^{th}$ position if the block $d_k$ was captured by the $\ell^{th}$ camera model and $0$ otherwise.  After pre-training, the softmax layer is discarded. This network is not updated during the initial training phase but is allowed to evolve slowly during subsequent fine-tuning phases.

\subheader{Contextual Feature Extraction}
The context feature extractor $h(\cdot)$ produces embeddings $c$ that provide information about a scene that contextualizes the forensic embeddings. Prior research has shown that scene content can greatly influence forensic features. Specifically, the amount and quality of forensic information in an analysis window depend on the local illumination, texture, compression parameters, and several other factors \citelater{cite a lot}. Therefore, by jointly analyzing forensic and contextual features, later portions of our network can adjust their forensic decisions about a particular area based on the contextual information at that region. To accomplish this, we used the Xception \citelater{cite} network architecture as the backbone for our CFE. Xception produces good context-dependent features, making it ubiquitous in solving computer vision tasks like object detection and object segmentation \citelater{cite}. Note that we only employ a single deep block instead of eight in the ``middle flow'' module because 1) generic contextual features often lie in the shallow layers of a CNN, and 2) we want to prevent the network from overfitting to high-level features (i.e., objects or identities).

\subheader{Joint Feature Extraction}
After obtaining both forensic and context embeddings for each block, we produce a joint feature embedding $x$ by concatenating $f$ and $c$, i.e.,
\begin{align}
        x_k = \text{Concat}(f_k, c_k)  
\end{align}
This process is repeated for every analysis block in the video frame to produce $N$ arrays of joint feature embedding. Each embedding is 768 elements long.

% Xception: https://arxiv.org/abs/1610.02357




==> sections/revisions_old/03_low_level_feature_extraction_v2_MCS.tex <==
% 03_low_level_feature_extraction_v2_MCS.tex

\subsection{Low-Level Feature Extraction}
\label{subsec:low_level_feature_extraction}

VideoFACT's network architecture consists of two low-level feature extractors working in tandem: the Forensic Feature Extractor (FFE) and the Contextual Feature Extractor (CFE). Each analysis block $b_k$ is independently passed through each extractor to produce a forensic feature embedding $f_k$ and a context feature embedding $c_k$.

\subheader{Forensic Feature Embeddings}
We use a CNN $g(\cdot)$ to produce dedicated forensic feature embeddings for each block.  To produce these embeddings, $g$ is pre-trained to discriminate between the source camera model used to capture each block in a separate training set.  This is inspired by an approach widely taken in image forensics, where a CNN trained to discriminate between source camera models is utilized to %produce
learn generic forensic feature embeddings~\cite{Noiseprint, EXIFnet, Splicebuster, Mayer_2018_IHMMS, FSM, FSG}.  These embeddings have been shown to capture both forensic information about the source and manipulation or processing history of a block.
%source camera and the manipulation and processing history of a block.

We implement $g$ using a MISLnet~\cite{MISLnet} backbone. This network was chosen because it is both lightweight and has been demonstrated to achieve strong performance on several forensic tasks in prior research \cite{FSM, FSG, Bayar_2018_ICASSP, Mayer_2018_ICASSP, MISLgan}. The loss used during the pre-training phase of $g$ is defined as:
\begin{equation}
        \mathcal{L}_{F} = - \sum\nolimits_{\ell=1}^{n}t_{\ell} \cdot log(g(d_k))_{\ell})
\end{equation}
where $n$ is the number of different camera models classes, %$t$ is the target one-hot vector with a $1$ in the $\ell^{th}$ position if the block $d_k$ was captured by the $\ell^{th}$ camera model and $0$ otherwise.  
$t_\ell=1$ if the block $d_k$ was captured by the $\ell^{th}$ camera model and $0$ otherwise. 
After pre-training, the softmax layer is discarded. This network is not updated during the initial training phase but is allowed to evolve slowly during subsequent fine-tuning phases.

%The context feature extractor h produces embeddings c that provide information about a scene that contextualize the forensic embeddings.  Prior research has shown that scene content can have important effects on forensic feature embeddings.  The amount and quality of forensic information contained in an analysis block depends on the local illumination, texture, compression parameters, as well as several other factors.  By jointly analyzing both forensic and context feature embeddings, later portions of our network can adjust how they interpret forensic features in a particular block to make better forensic decisions.



\subheader{Context Feature Embeddings}
The context feature extractor $h(\cdot)$ produces embeddings $c$ that provide information about a scene that contextualizes the forensic embeddings. Prior research has shown that scene content can have important effects on forensic features. Specifically, the amount and quality of forensic information in an analysis window depends on the local illumination, texture, compression parameters, and several other factors~\cite{chu2015information, pasquini2018information, schlogl2021forensicability}. By jointly analyzing forensic and context feature embeddings, later portions of our network can adjust how they interpret forensic features in a particular block to make better forensic decisions. We implement $h$ by using an Xception~\cite{Xception} network backbone that is modified to use only a single middle flow module, followed by a $1\times 1$ layer to reduce the feature embedding dimension. 

%later portions of our network can adjust their forensic decisions about a particular area based on the contextual information at that region. 
%We implement $h$ by using an Xception backbone to extract low-level content features followed by a $1\times 1$ layer to reduce the feature embedding dimension.
%We implement $h$ by using a single block from the middle flow module of Xception to extract low-level content features, followed by a $1\times 1$ layer to reduce the feature embedding dimension.  

\subheader{Joint Feature Extraction}
After obtaining both forensic and context embeddings for each block, we produce the joint feature embeddings $x$ by concatenating $f$ and $c$, i.e.,
\begin{align}
        x_k = \text{Concat}(f_k, c_k)  
\end{align}
This process is repeated for every analysis block in the video frame to produce $N$ arrays of joint feature embedding. Each embedding is 768 elements long.

% Xception: https://arxiv.org/abs/1610.02357
%To accomplish this, we used the Xception \citelater{cite} network architecture as the backbone for our CFE. 
%Xception produces good context-dependent features, making it ubiquitous in solving computer vision tasks like object detection and object segmentation \citelater{cite}. 
%Note that we only employ a single deep block instead of eight in the ``middle flow'' module because 1) generic contextual features often lie in the shallow layers of a CNN, and 2) we want to prevent the network from overfitting to high-level features (i.e., objects or identities).

==> sections/revisions_old/03_motivation_v0_MCS.tex <==
%03_motiviation_v0_MCS.tex




Modern forensic approaches typically use a CNN to produce feature embeddings that capture the forensic traces within a local analysis neighborhood.  Some approaches directly map these embeddings to a forensic decision, e.g. a source camera classifier.  Others use a higher level system to examine these embeddings for localized inconsistencies in order to identify fake or manipulated content. 


Typically, these systems treat forensic traces as independent from a scene’s content or spatial position.  For example, ideally resizing traces should express themselves as specific, repeatable local pixel value relationships induced by resizing irrespective of what was resized or where resizing occurred.




%Often forensic systems view forensic traces as independent from a scene’s content.  For example, the traces left by blurring region ideally don’t depend on what content was blurred, but instead on local pixel value relationships induced by the blurring operation.  As a result, many modern forensic networks analyze forensic trace embeddings without accounting for their spatial position within an image or video frame.  


Typically, these systems treat forensic traces as independent from a scene’s content or spatial position.  For example, ideally resizing traces should express themselves as specific, repeatable local pixel value relationships induced by resizing irrespective of what was resized or where resizing occurred.

In reality, however, prior forensics research has shown that the quantity and quality of forensic information that can be extracted from an image or video frame depends on its content~\citelater{cite here}.  In this research, a local neighborhood of pixels is viewed as a communication channel through which forensic information is transmitted.  As a result, some regions contain more and higher quality forensic information, while others contain little-to-no forensic information.  Similar results have been obtained in related fields such as steganalysis and watermarking~\citelater{cite here}.

Similarly, fake and manipulated content does not occur in randomly chosen spatial locations.  Instead, a forger will manipulate content to splice in, alter, or remove an object located in a particular spatial position to change how an image or video is perceived.  As a result, it is likely that there are spatial dependencies between forensic traces.

Variations in forensic capacity are 

Because prior forensics research has largely focused on detecting image forgeries, they have been able to avoid significant drops in  performance without accounting for these issues.  Typically, experiments are performed on high quality images that are either uncompressed or JPEG compressed.   

Prior forensics research has been able to largely avoid these issues due to a f




%In reality, however, fake and manipulated content does not occur in randomly chosen spatial locations.  Instead, a forger will manipulate content to splice in, alter, or remove an object located in a particular spatial position to change how an image or video is perceived.  As a result, it is likely that there are spatial dependencies between forensic traces.




==> sections/revisions_old/03_motivation_v1_MCS.tex <==
%03_motiviation_v1_MCS.tex

\subsection{Motivation and Overview}


%Forensic traces correspond to local pixel value relationships induced by editing and content falsification, as well as by processing elements inside a source camera.  


%Forensic traces correspond to local pixel value relationships induced by editing and content falsification.  %, as well as by processing elements inside a source camera.  

%Our network operates by analyzing each video frame for evidence of anomalous forensic traces that are left by manipulation or content falsification.
Our network operates by analyzing each video frame for evidence of anomalous forensic traces left by manipulation or content falsification.
%
%Forgery detection and localization networks operate by searching for forensic traces left by editing and content falsification~\citelater{cite here}.  
%These traces 
Forensic traces correspond to local pixel value relationships induced by editing and other processing operations (e.g. synthetic content generation)~\citelater{cite here}.  When a video is forged, forensic traces in the falsified region will be inconsistent with the traces in the rest of the frame.

%Modern 
Existing forensic networks typically operate by dividing an image into small analysis regions, then capturing the forensic traces in each region as an embedding.  The sequence of embeddings is then analyzed for anomalies, irrespective of their underlying spatial position or scene content~\citelater{cite here}.
%irrespective of their spatial position or scene content within each analysis region.




Prior forensics research, however, has shown that scene content has an important influence on the quality and quantity of forensic information that can be extracted from an analysis region~\citelater{cite here}. 
Some regions contain more and higher quality forensic information, while others contain little-to-no forensic information.
As a result, forensic embeddings have implicit dependencies on the scene content in the region from which they are extracted.
%
Similarly, editing and falsification does not occur in random, independent spatial positions throughout a scene.  Instead, a scene is typically modified to edit, add, or remove an object.  As a result, there are implicit spatial dependencies between forensic embeddings in falsified content.




%Our network is explicitly designed to exploit both contextual dependencies upon scene content as well as spatial dependencies of forensic traces. 

Our network is explicitly designed to exploit forensic traces' contextual dependencies upon scene content as well as spatial dependencies.  
 We accomplish this by producing both low-level forensic feature embeddings as well as low-level context embeddings for each local analysis region.  These context embeddings provide information that accounts for variations in the forensic embeddings due to scene content.  
%
We leverage these forensic and context embeddings by using a deep transformer-based attention module to provide spatial attention information to two different subnetworks that perform frame-level forgery detection and pixel-level forgery localization. 

This deep attention mechanism provides our network with multiple benefits. It enables our network attend to regions with high quality forensic information while deemphasizing regions with lower quality information that may cause false alarms. I t is also able to learn and exploit complex relationships between the forensic embeddings, context embeddings, and spatial position to better identify fake content.  We note that recent work has begun to utilize shallow attention mechanisms in forensic networks~\citelater{cite MVSS, Maybe ManTra-Net?, others?}.  However, as our results in Section~\ref{sec:experiments} show, these shallow mechanisms are unable to produce strong results on video forgeries.  By contrast, our deep transformer-based attention mechanism is able to overcome challenges encountered by prior work and produce strong video forgerey detection and localization results.

%An overview of our network can be seen in Figure~\todo{ADD FIGURE}.  We note that our network is designed to operate on 1080p video encoded using h.264.


%\textbf{Overview} 
%An overview of our network can be seen in Figure~\todo{ADD FIGURE}.

%Our network operates by dividing a video frame into a sequence of non-overlapping analysis blocks of size $128\times128$ pixels.  Each block is sent in parallel to different modules that produce forensic feature and context embeddings








==> sections/revisions_old/03_overview_v1_MCS.tex <==
% 03_overview_v1_MCS.tex



\subsection{Network Overview}

Our network operates by individually analyzing each video frame for evidence of anomalous forensic traces that are indicative of manipulation or content falsification.
%Our network operates by individually analyzing each video frame and searching for forensic traces indicative of manipulation or content falsification.  
It does this by first dividing a video frame into non-overlapping analysis blocks of size $128\times128$ pixels.  Next, each block is sent to two parallel low-level feature extractors.  One is designed to produce forensic feature embeddings $f$ that capture information about the source and processing history of the content in an analysis block.  The other is a context embedding $c$ that captures relevant local  information about the scene that contextualizes the forensic embeddings. Context feature embeddings provide later layers of the network with important scene and content information that can be used to adjust forensic decisions made on the basis of forensic features.  A joint set of low-level feature embeddings $x$ is produced by concatenating forensic and context embeddings.

The joint feature embeddings $x$ are passed to a transformer-based attention module, which produces a series of $L$ different spatial attention maps $m_\ell$.  These attention maps are then used to weight the joint feature embeddings by spatial attention.  This enables the network to attend to regions with high-quality forensic information, while deemphasizing regions with low-quality information that may cause false alarms.  The resulting attention weighted embeddings $y$ are then used by two parallel sub-networks that independently perform frame-level forgery detection and pixel-level forgery localization.  While localization sub-network will produce a forgery localization mask for every video frame, this mask should be disregarded if the detection sub-network indicates that the frame is authentic.


==> sections/revisions_old/03_overview_v2_MCS.tex <==
% 03_overview_v2_MCS.tex



%\subsection{Network Overview}

%Our network operates by individually analyzing each video frame for evidence of anomalous forensic traces that are indicative of manipulation or content falsification.
%Our network operates by individually analyzing each video frame and searching for forensic traces indicative of manipulation or content falsification.  

An overview of VideoFACT can be seen in Figure~\ref{fig:system_overview_diagram}.
Our network first divides a frame into non-overlapping analysis blocks of size $128\times128$ pixels. 
%Our network individually analyzes each video frame by first dividing it into non-overlapping analysis blocks of size $128\times128$ pixels. 
Next, each block is sent to two parallel low-level feature extractors: one designed to produce forensic feature embeddings $f$ and another that produces context embedding $c$ that captures relevant local information about the scene.
%One is designed to produce forensic feature embeddings $f$ that capture information about the source and processing history of the content in an analysis block.  The other is a context embedding $c$ that captures relevant local  information about the scene that contextualizes the forensic embeddings. 
%Context feature embeddings provide later layers of the network with important scene and content information that can be used to adjust forensic decisions made on the basis of forensic features.  
%A joint set of low-level feature embeddings $x$ is produced by concatenating the forensic and context embeddings.  
%
%The joint feature embeddings $x$ are 
A joint set of low-level feature embeddings $x$, which is produced by concatenating the forensic and context embeddings, is
passed to a transformer-based attention module, which produces a series of $L$ different spatial attention maps $m_\ell$.  These attention maps are then used to weight the joint feature embeddings by spatial attention.  %This enables the network to attend to regions with high-quality forensic information, while deemphasizing regions with low-quality information that may cause false alarms.  
The resulting attention weighted embeddings $y$ are then used by two parallel subnetworks, which independently perform frame-level forgery detection and pixel-level forgery localization.  
%While the localization subnetwork will produce a forgery localization mask for every video frame, this mask should be disregarded if the detection subnetwork indicates that the frame is authentic.

==> sections/revisions_old/03_proposed_approach_v1.tex <==
\section{Proposed Approach}
\label{sec:proposed_approach}

This paper proposes a new approach that can jointly detect and localize manipulations in video frames. Given an input video frame $I$ of size $H \times W \times C$, our deep neural network model, $\mathcal{D}$, offers both a detection score, which indicates the probability of a frame having any manipulation, and a localization mask, which shows the location of the tampering operations. To accomplish this, we first split $I$ into a flattened sequence of non-overlapping blocks of size $128 \times 128$, $I = [b_1, b_2 \cdots b_N]$, where $N = \frac{HW}{128^2}$. Then, using two separate feature extractors, $g(\cdot)$ and $h(\cdot)$, we extract forensic embeddings $f$, and contextual embeddings $c$. A joint set of low-level feature embeddings $x$ is produced by concatenating $f$ and $c$. We then weight each joint embedding vectors using multiple spatial attention maps, $M$, generated from the Transformer-Based Attention Module. Their weighted versions, $y$, are fed into two separate networks, $p(\cdot)$ and $q(\cdot)$, to produce a detection score and a localization mask, respectively.



%%%%%% NOTES %%%%%%
% As shown in Figure [{\color{green}{cite}}], our proposed [{\color{green}{model name}}] is composed of 5 modules, namely: the low-level feature extractor, the learnable attention maps using Vision Transformer, the feature combinator and dimensionality reductor, the forgery detector, and the forgery localizer. Using this architecture, we make five(?) contributions to (maybe can word this differently) solve the problem of detecting and localizing video forgeries.

% First, we solved the problems of videos created in the H.264 format having varying compression schemes across blocks within a single frame. These schemes depend on: the type of frame (I, B, P), the bitrate allocated, the compression quality factor, and the content inside. Our feature extractor is designed and trained to be invariant to these factors but sensitive to manipulation traces.

% Second, we dealt with the issue of previous forensic algorithm having troubles with areas which have extreme lighting or textual conditions. We utilize the Vision Transformer in our model to simultaneously 1) suppress the importance of the features collected at "extreme" regions, and 2) amplify regions containing different forensic traces. This method allows our solution to have much lower false alarm rate and miss detection rate in the decision making process. 

% (Do we need to say: We will show that localization results conforms with our intent. ?)

% Third, our solution not only generalizes over many types of manipulations, or combinations of them, (i.e ...)

% but also performs well with infinitely varying degrees of alterations. We achieved this by applying a training protocol using increasingly difficult-to-detect-manipulations datasets. This guides our model gradually towards achieving the best performance on ALL of the datasets combined. Without doing this, we found that the model cannot even train to convergence on our hardest dataset.

% Fourth, we conducted experiments which shows that our novel solution is transferable to images using transfer learning. We achieved state-of-the-art performance on many image manipulation datasets ... (list them)
% on both the detection and localization tasks.

% Finally, we meticulously conduct many ablation experiments to optimize the network architecture, and to provide theoretical/empirical grounds to support our model design. 

% Prior arts, especially ones which utilized deep learning, can be describe as having some feature extractor obtaining an embedding for every analysis window, which are then either fed straight to a decision module, or first compared, then combined and analyzed 

% Prior state-of-the-art algorithms [cite a lot] can be generally described as having a feature extractor obtain scene-content-independent, forensic embeddings for every analysis window, which are then examined jointly or separately to produce a final decision. However, as we will see later, these approaches are suboptimal when analyzing videos because: 1) the quality of video-forensic information in an analysis window is controlled by both its scene content and dynamic compression parameters, and, 2) real-life forgeries are context and spatially dependent. 






==> sections/revisions_old/03_proposed_approach_v2MCS.tex <==
% 03_proposed_approach_v2MCS

\section{Proposed Approach}
\label{sec:proposed_approach}

%This paper proposes a new approach that can jointly detect and localize manipulations in video frames. Given an input video frame $I$ of size $H \times W \times C$, our deep neural network model, $\mathcal{D}$, offers both a detection score, which indicates the probability of a frame having any manipulation, and a localization mask, which shows the location of the tampering operations. To accomplish this, we first split $I$ into a flattened sequence of non-overlapping blocks of size $128 \times 128$, $I = [b_1, b_2 \cdots b_N]$, where $N = \frac{HW}{128^2}$. Then, using two separate feature extractors, $g(\cdot)$ and $h(\cdot)$, we extract forensic embeddings $f$, and contextual embeddings $c$. A joint set of low-level feature embeddings $x$ is produced by concatenating $f$ and $c$. We then weight each joint embedding vectors using multiple spatial attention maps, $M$, generated from the Transformer-Based Attention Module. Their weighted versions, $y$, are fed into two separate networks, $p(\cdot)$ and $q(\cdot)$, to produce a detection score and a localization mask, respectively.

%\subsection{Problem Formulation}



%Our network is designed to jointly address two distinct but related forensic problems: Detection - i.e. does a video contain any fake or manipulated content and Localization - i.e. identify where fake or manipulated content occurs within a frame.

%Our network is not designed to identify temporal manipulations (e.g. altering a video's speed, adding or deleting frames, etc.) or manipulations to the video's audio track.  Furthermore, we 



\subsection{Motivation and Overview}

%\input{sections/03_motivation_v0_MCS}
\input{sections/03_motivation_v1_MCS}




\subsection{Network Overview}

Our network operates by individually analyzing each video frame for evidence of anomalous forensic traces that are indicative of manipulation or content falsification.
%Our network operates by individually analyzing each video frame and searching for forensic traces indicative of manipulation or content falsification.  
It does this by first dividing a video frame into non-overlapping analysis blocks of size $128\times128$ pixels.  Next, each block is sent to two parallel low-level feature extractors.  One is designed to produce forensic feature embeddings $f$ that capture information about the source and processing history of the content in an analysis block.  The other is a context embedding $c$ that captures relevant local  information about the scene that contextualizes the forensic embeddings. Context feature embeddings provide later layers of the network with important scene and content information that can be used to adjust forensic decisions made on the basis of forensic features.  A joint set of low-level feature embeddings $x$ is produced by concatenating forensic and context embeddings.

The joint feature embeddings $x$ are passed to a transformer-based attention module, which produces a series of $L$ different spatial attention maps $m_\ell$.  These attention maps are then used to weight the joint feature embeddings by spatial attention.  This enables the network to attend to regions with high-quality forensic information, while deemphasizing regions with low-quality information that may cause false alarms.  The resulting attention weighted embeddings $y$ are then used by two parallel sub-networks that independently perform frame-level forgery detection and pixel-level forgery localization.  While localization sub-network will produce a forgery localization mask for every video frame, this mask should be disregarded if the detection sub-network indicates that the frame is authentic.


































%%%%%% NOTES %%%%%%
% As shown in Figure [{\color{green}{cite}}], our proposed [{\color{green}{model name}}] is composed of 5 modules, namely: the low-level feature extractor, the learnable attention maps using Vision Transformer, the feature combinator and dimensionality reductor, the forgery detector, and the forgery localizer. Using this architecture, we make five(?) contributions to (maybe can word this differently) solve the problem of detecting and localizing video forgeries.

% First, we solved the problems of videos created in the H.264 format having varying compression schemes across blocks within a single frame. These schemes depend on: the type of frame (I, B, P), the bitrate allocated, the compression quality factor, and the content inside. Our feature extractor is designed and trained to be invariant to these factors but sensitive to manipulation traces.

% Second, we dealt with the issue of previous forensic algorithm having troubles with areas which have extreme lighting or textual conditions. We utilize the Vision Transformer in our model to simultaneously 1) suppress the importance of the features collected at "extreme" regions, and 2) amplify regions containing different forensic traces. This method allows our solution to have much lower false alarm rate and miss detection rate in the decision making process. 

% (Do we need to say: We will show that localization results conforms with our intent. ?)

% Third, our solution not only generalizes over many types of manipulations, or combinations of them, (i.e ...)

% but also performs well with infinitely varying degrees of alterations. We achieved this by applying a training protocol using increasingly difficult-to-detect-manipulations datasets. This guides our model gradually towards achieving the best performance on ALL of the datasets combined. Without doing this, we found that the model cannot even train to convergence on our hardest dataset.

% Fourth, we conducted experiments which shows that our novel solution is transferable to images using transfer learning. We achieved state-of-the-art performance on many image manipulation datasets ... (list them)
% on both the detection and localization tasks.

% Finally, we meticulously conduct many ablation experiments to optimize the network architecture, and to provide theoretical/empirical grounds to support our model design. 

% Prior arts, especially ones which utilized deep learning, can be describe as having some feature extractor obtaining an embedding for every analysis window, which are then either fed straight to a decision module, or first compared, then combined and analyzed 

% Prior state-of-the-art algorithms [cite a lot] can be generally described as having a feature extractor obtain scene-content-independent, forensic embeddings for every analysis window, which are then examined jointly or separately to produce a final decision. However, as we will see later, these approaches are suboptimal when analyzing videos because: 1) the quality of video-forensic information in an analysis window is controlled by both its scene content and dynamic compression parameters, and, 2) real-life forgeries are context and spatially dependent. 






==> sections/revisions_old/03_training_protocol_v1.tex <==
\subsection{Progressively Difficult Manipulations Training Protocol}
\label{subsec:training_protocol}

The training protocol described in this section is necessary for our model to not only converge smoothly, but also attain a high degree of generalizability across many manipulations in different data distributions. This strategy involves training the network on progressively difficult manipulations, then fine-tuning it on all manipulations, and finally robust-training it with data from more diverse scene contents, lighting conditions and other manipulations. The progressively difficult manipulations are divided into three groups, ranking from lowest to highest difficulty: Simple Splicing, Visible Manipulations, and Invisible Manipulations. 

\textit{The Simple Splicing group} contains operations involved copying one or multiple regions of a video frame and pasting those on another video frame. These manipulations are easy to spot because there's no requirement about content matching between the source and the destination frame. During training, we make it even easier by requiring that the source frame and the destination frame must come from different camera models with fundamentally different forensic traces. 

\textit{The Visible Manipulations group} contains in-place operations on one or multiple localized regions of a video frame, such as: brightness adjustment, contrast enhancement, blurring, noise adding. We require that the strength of these manipulations must be high enough so that they are clearly visible on the victim video frame.

\textit{The Invisible Manipulations group} contains operations similar to those in the visible manipulations group, but their strengths must be low enough so that they cannot be detected with the human eye.

Our training protocol is as follows:
\begin{enumerate}[topsep=3pt]
\setlength\itemsep{-0.35em}
    \item Train the model on data from each group progressively.
    \item Fine-tune the model on data from all groups, but with a heavy emphasis on the invisible manipulations group.
    \item Robust-training the model using data with diverse scene contents, lighting conditions and different manipulations (if possible).
\end{enumerate}
Utilizing this training protocol, as we will show in our experiments, our proposed network achieves both strong performance and high degrees of generalizability.

% However, as we will show in the \hyperref[sec:experiments]{experiments} section, the performance on our datasets and "in-the-wild" datasets can be improved further by exposing our model to more diverse scene and lighting condition. Although Video-ACID has 12,000 videos, almost all of them are taken in or near a physical location (Philadelphia, USA). Hence, most outdoor videos contain urban scenery with trivial change in the amount of greenery, water, and sky. In addition, most indoor videos have little variation in lighting conditions. To increase the generalizing ability of our model, we augmented the training data with images from the (Image) Camera Model Identification Database [{\color{green}{cite this}}] (CMID), which contained 46,461 photos from 128 physical devices representing 70 different camera models. Utilizing this database, we created 3 similar datasets using the same techniques detailed above (section \ref{subsec:VCMS}, \ref{subsec:VPVM}, \ref{subsec:VPIM}): 
% \begin{enumerate}
%     \item \label{ICMS} Image Camera Model Splicing (ICMS)
%     \item \label{IPVM} Image Perceptually Visible Manipulations (IPVM)
%     \item \label{IPIM} Image Perceptually Invisible Manipulations (IPIM)
% \end{enumerate}
% We fine-tuned our network on all 6 datasets with the following composition: 10\% VCMS, 10\% VPVM, 70\% VPIM, 10\% ICMS, 10\% IPVM, 70\% IPIM. Since there are more samples, more scenes and more variation in lighting conditions in CMID, our network is able to boost its performance on all benchmarking metrics, especially localization ones. 

==> sections/revisions_old/03_training_protocol_v2_Shengbang.tex <==
\subsection{Multi-Stage Training Protocol}
\label{subsec:training_protocol}
% Overview
We divide the training protocol into five stages. The first three stages train the model for three datasets with increasing difficulty, where the previous training stage provide a good initialization for the next training stage. The last two stages train the model with multiple datasets with varying scene content to improve the generalizability of the model.    
% Objective
%The training protocol described in this section is necessary for our model to not only converge smoothly, but also attain a high degree of generalizability across many manipulations in different data distributions.
% process 
% This strategy involves training the network on progressively difficult manipulations, then fine-tuning it on all manipulations, and finally robust-training it with data from more diverse scene contents, lighting conditions and other manipulations.

For the first three stages, we train the model using the datasets with successively increasing challenge, to let the model progressively learn good features. In Stage 1, we use Video Camera Model Splicing Dataset (VCMS), which contains splicing content from other videos, and its features are consistent with what FFE learned. In Stage 2, we train the model with Video Perceptually Visible Manipulation Dataset (VPVM), which contains in-place perceptually visible manipulation regions. In Stage 3, we train the model with Video Perceptually Invisible Manipulation datasets (VPIM), which is similar with VPVM but the manipulation is perceptually invisible. Details about the creation of each dataset is provided in the following section.
We train the model in such order because experiments showed that it results in the smoothest loss decreasing during training. 
% divide 3  
%The progressively difficult manipulations are divided into three groups, ranking from lowest to highest difficulty: Simple Splicing, Visible Manipulations, and Invisible Manipulations. 
% one
%\textit{The Simple Splicing group} contains operations involved copying one or multiple regions of a video frame and pasting those on another video frame. These manipulations are easy to spot because there's no requirement about content matching between the source and the destination frame. During training, we make it even easier by requiring that the source frame and the destination frame must come from different camera models with fundamentally different forensic traces. 
% two
%\textit{The Visible Manipulations group} contains in-place operations on one or multiple localized regions of a video frame, such as: brightness adjustment, contrast enhancement, blurring, noise adding. We require that the strength of these manipulations must be high enough so that they are clearly visible on the victim video frame.
% three
%\textit{The Invisible Manipulations group} contains operations similar to those in the visible manipulations group, but their strengths must be low enough so that they cannot be detected with the human eye.

For the last two stages, we train the video with multiple dataset together to provide the model a more diverse training dataset. In stage 4, we fine-tune the model using all three dataset (VCMS, VPVM and VPIM). In stage 5, we further fine-tune the model using all three videos datasets together with three auxiliary image datasets. These three image datasets are created following similar pipelines with three video datasets. which results one with splicing contents, one with visible manipulation and one with invisible manipulations. These images are created from Camera Model Identification Database (CMID)\citelater{CMID} and are JPEG-compressed. We use the image datasets because camera-captured images can enhance the variety of distribution of training data, and experiments show that training with images significantly improve the performance and generalizability of the model.   

% combine, conquer
%Our training protocol is as follows:
%\begin{enumerate}[topsep=3pt]
%\setlength\itemsep{-0.35em}
%    \item Train the model on data from each group progressively.
%    \item Fine-tune the model on data from all groups, but with a heavy emphasis on the invisible manipulations group.
%    \item Robust-training the model using data with diverse scene contents, lighting conditions and different manipulations (if possible).
%\end{enumerate}
% Conclusion
%Utilizing this training protocol, as we will show in our experiments, our proposed network achieves both strong performance and high degrees of generalizability.

% However, as we will show in the \hyperref[sec:experiments]{experiments} section, the performance on our datasets and "in-the-wild" datasets can be improved further by exposing our model to more diverse scene and lighting condition. Although Video-ACID has 12,000 videos, almost all of them are taken in or near a physical location (Philadelphia, USA). Hence, most outdoor videos contain urban scenery with trivial change in the amount of greenery, water, and sky. In addition, most indoor videos have little variation in lighting conditions. To increase the generalizing ability of our model, we augmented the training data with images from the (Image) Camera Model Identification Database [{\color{green}{cite this}}] (CMID), which contained 46,461 photos from 128 physical devices representing 70 different camera models. Utilizing this database, we created 3 similar datasets using the same techniques detailed above (section \ref{subsec:VCMS}, \ref{subsec:VPVM}, \ref{subsec:VPIM}): 
% \begin{enumerate}
%     \item \label{ICMS} Image Camera Model Splicing (ICMS)
%     \item \label{IPVM} Image Perceptually Visible Manipulations (IPVM)
%     \item \label{IPIM} Image Perceptually Invisible Manipulations (IPIM)
% \end{enumerate}
% We fine-tuned our network on all 6 datasets with the following composition: 10\% VCMS, 10\% VPVM, 70\% VPIM, 10\% ICMS, 10\% IPVM, 70\% IPIM. Since there are more samples, more scenes and more variation in lighting conditions in CMID, our network is able to boost its performance on all benchmarking metrics, especially localization ones. 

==> sections/revisions_old/03_training_protocol_v3_MCS.tex <==
\subsection{Multi-Stage Training Protocol}
\label{subsec:training_protocol}
% Overview
%Out network training protocol consists of five stages.  


%In the first three stages, the network is trained with datasets of videos falsified using manipulations that are successively more difficult to detect. This enables the network to progressively learn better features by refining the features learned in the previous stage.  


%In each of the first three stages, our network is trained using a different dataset of videos made using different set of manipulations (e.g. splicing, editing, etc.).  
%The first three stages involve training our network using different datasets consisting of fake videos made using increasingly more difficult manipulations to detect.  
%The first three  stages train the network using three different datasets.  Each dataset introduces the network to fake videos made using increasingly more difficult manipulations to detect.
% three datasets with increasing difficulty, where the previous training stage provide a good initialization for the next training stage. 
%We divide the training protocol into five stages. The first three stages train the model for three datasets with increasing difficulty, where the previous training stage provide a good initialization for the next training stage. 
%
%The last two stages train the model with multiple datasets with varying scene content to improve the generalizability of the model.    
% Objective
%The training protocol described in this section is necessary for our model to not only converge smoothly, but also attain a high degree of generalizability across many manipulations in different data distributions.
% process 
% This strategy involves training the network on progressively difficult manipulations, then fine-tuning it on all manipulations, and finally robust-training it with data from more diverse scene contents, lighting conditions and other manipulations.

Our network training protocol consists of five stages.  
In the first three stages, the training datasets consist of videos falsified with manipulations that are successively more difficult to detect.  
This enables the network to progressively learn better features by refining those learned in the previous stage.  
 %rather than forcing it to identify these features on a challenging dataset and risk falling into 
%we train the model using the datasets with successively increasing challenge, to let the model progressively learn good features. 
In Stage 1, we use the Video Camera Model Splicing dataset (VCMS), which contains spliced content from other videos.  Because splicing induces source camera inconsistencies within a frame, the forensic embeddings learned by the FFE in the pre-training phase are well suited to identify these manipulations. 
%The forensic embeddings learned by the FFE during pre-training are already well suited identify these and its features are consistent with what FFE learned. 
%
%
%In Stage 2, we train the model with Video Perceptually Visible Manipulation Dataset (VPVM), which contains in-place perceptually visible manipulation regions. In Stage 3, we train the model with Video Perceptually Invisible Manipulation datasets (VPIM), which is similar with VPVM but with low manipulation strengths that are invisible to the human eye.
In Stages 2 and 3,  we train the network with the Video Perceptually Visible Manipulation dataset (VPVM) and Video Perceptually Invisible Manipulation datasets (VPIM), respectively.  These datasets, which are described in Section~\ref{sec:training_datasets},  contain videos manipulated using standard editing operations applied with different strengths.
%
%, which is similar with VPVM but with low manipulation strengths that are invisible to the human eye.
%
%
%
%Details about %the creation of 
%each dataset is provided in the following Section~\ref{sec:training_datasets}.  
 %Experiments showed that training on the datasets in this order resulted in the smoothest decrease in the loss.


%We train the model in such order because experiments showed that it results in the smoothest loss decreasing during training. 
% divide 3  
%The progressively difficult manipulations are divided into three groups, ranking from lowest to highest difficulty: Simple Splicing, Visible Manipulations, and Invisible Manipulations. 
% one
%\textit{The Simple Splicing group} contains operations involved copying one or multiple regions of a video frame and pasting those on another video frame. These manipulations are easy to spot because there's no requirement about content matching between the source and the destination frame. During training, we make it even easier by requiring that the source frame and the destination frame must come from different camera models with fundamentally different forensic traces. 
% two
%\textit{The Visible Manipulations group} contains in-place operations on one or multiple localized regions of a video frame, such as: brightness adjustment, contrast enhancement, blurring, noise adding. We require that the strength of these manipulations must be high enough so that they are clearly visible on the victim video frame.
% three
%\textit{The Invisible Manipulations group} contains operations similar to those in the visible manipulations group, but their strengths must be low enough so that they cannot be detected with the human eye.

In the last two stages, we %seek to 
improve the generalizability of our network by training on multiple datasets with varying manipulations and scene content.
%train the model using multiple datasets with varied scene content to improve the generalizability of the model.    
%For the last two stages, we train the video with multiple dataset together to provide the model a more diverse training dataset. 
In Stage 4, we fine-tune the network using all three previous datasets simultaneously (VCMS, VPVM and VPIM).  In Stage 5, we further fine-tune the model by incorporating three auxiliary datasets made from images in the Camera Model Identification Database (CMID) first used in \cite{Bayar_2018_ICASSP, MISLnet}.  %CMID data is used because it contains different scenes than those in the Video-ACID dataset, thus increasing 
%using all three videos previous datasets, as well as three auxiliary image datasets. 
%made from images in the Camera Model Identification Database (CMID) first used in \citelater{CMID}.  
We create these auxiliary training datasets from the CMID, because it captures scenes with different content and distribution than the Video-ACID dataset.  This increases the diversity of data on which our network is trained.  These auxiliary datasets are made using the same process used to create the three video datasets, resulting in one dataset with spliced content (ICMS), one with perceptually visible manipulations (IPVM), and one with perceptually invisible manipulations (IPIM).  
%Experiments show that training with these datasets significantly improve the generalizability of the model to other "in-the-wild" datasets.   

% combine, conquer
%Our training protocol is as follows:
%\begin{enumerate}[topsep=3pt]
%\setlength\itemsep{-0.35em}
%    \item Train the model on data from each group progressively.
%    \item Fine-tune the model on data from all groups, but with a heavy emphasis on the invisible manipulations group.
%    \item Robust-training the model using data with diverse scene contents, lighting conditions and different manipulations (if possible).
%\end{enumerate}
% Conclusion
%Utilizing this training protocol, as we will show in our experiments, our proposed network achieves both strong performance and high degrees of generalizability.

% However, as we will show in the \hyperref[sec:experiments]{experiments} section, the performance on our datasets and "in-the-wild" datasets can be improved further by exposing our model to more diverse scene and lighting condition. Although Video-ACID has 12,000 videos, almost all of them are taken in or near a physical location (Philadelphia, USA). Hence, most outdoor videos contain urban scenery with trivial change in the amount of greenery, water, and sky. In addition, most indoor videos have little variation in lighting conditions. To increase the generalizing ability of our model, we augmented the training data with images from the (Image) Camera Model Identification Database [{\color{green}{cite this}}] (CMID), which contained 46,461 photos from 128 physical devices representing 70 different camera models. Utilizing this database, we created 3 similar datasets using the same techniques detailed above (section \ref{subsec:VCMS}, \ref{subsec:VPVM}, \ref{subsec:VPIM}): 
% \begin{enumerate}
%     \item \label{ICMS} Image Camera Model Splicing (ICMS)
%     \item \label{IPVM} Image Perceptually Visible Manipulations (IPVM)
%     \item \label{IPIM} Image Perceptually Invisible Manipulations (IPIM)
% \end{enumerate}
% We fine-tuned our network on all 6 datasets with the following composition: 10\% VCMS, 10\% VPVM, 70\% VPIM, 10\% ICMS, 10\% IPVM, 70\% IPIM. Since there are more samples, more scenes and more variation in lighting conditions in CMID, our network is able to boost its performance on all benchmarking metrics, especially localization ones. 

==> sections/revisions_old/03_transformer_module_v1.tex <==
\subsection{Transformer-Based Attention Module}
\label{subsec:transformer_module}

The sequence of joint embeddings $[v_1, v_2 \cdots v_N] = v$ is first combined with a vector of 1D learnable spatial embeddings $s$, as commonly done in Vision Transformers, then passed to a Transformer-Based Attention Module, designed to produce a series of $L$ different spatial attention maps, $M \in \mathbb{R}^{N \times L}$. Each attention map is an $N \times 1$ vector, where each entry corresponds to the network’s attention score for the corresponding feature joint embedding at that position.

In this work, our Transformer network contains 12 encoder blocks stacked on top of one another, with each block having 12 attention heads. For each encoder, we use an input embedding size of $d_{embed} = 768$. The output of the transformer is passed to an ``attention squeeze'' layer which is a $1 \times 1$ 2D convolutional layer with $L$ filters. This ``squeezes'' down the high dimensional output of the transformer into a series of $L$ different $N \times 1$ spatial attention maps $m_{\ell}$. Through experiments, we determined that $L = 3$ achieve optimal performance and generalizability.


%%%%%%% NOTES %%%%%%%
% Reliability map estimation for CNN-based camera model attribution https://arxiv.org/pdf/1805.01946.pdf

% This module generates attention maps, $M \in \mathbb{R}^{N \times d_{maps}}$, from the spatially contextualized forensic embeddings, $SCP \in \mathbb{R}^{N \times d_{embed}}$. Each of these maps is used to emphasize regions with high quality forensic traces or potential manipulations and suppress regions with low quality forensic traces. 
% Prior works \citelater{cite} have shown that the quality of forensic traces is diminished in places where the entropy is either too low or too high. 
% Additionally, since video coding dynamically adjusts the compression parameters for each block in a frame, the attention maps may also normalize attenuated forensic signals across the whole frame, allowing for more accurate comparisons.
% Prior works \citelater{cite} have shown that the information capacity can be sufficiently measured using Shannon's entropy $\mathbf{H}$:
% \begin{align}
%         \mathbf{H}(x_p) = - \sum_{k=0}^{255} p_k ln(p_k)
% \end{align}
% where $p_k$ is the probability that a pixel has luminance value $k$ in the analysis window $x_p$.
% Using deep, multiheaded self-attention, each input low-level feature vector is transformed in a way that reflects the relationships between it and every other token in the sample.
% This enables the learnable templates to examine all the transformed embeddings and extract regions with aberrant forensic traces that are not affected by extreme lighting or texture conditions. In addition, since multiple templates give rise to multiple attention maps, the model can maximize the amount of information extracted from the Transformer's embeddings. 



==> sections/revisions_old/03_transformer_module_v2_Shengbang.tex <==
\subsection{Transformer-Based Attention Module}
\label{subsec:transformer_module}

The sequence of joint embeddings is passed to the transformer-based attention module, which is designed to produce a series of L different spatial attention maps. As commonly done in Vision Transformers, a vector of 1D learnable spatial embeddings is added to the joint embedding before being passed to the transformer. The transformer consists of twelve transformer encoder blocks stacked on top of one another. The output of the transformer is passed to an "Attentsion Squeeze" layer that consists of L $1\times 1$ Conv kernels, and are squeezed down to a series of L different $M\times N$ spatial attention maps $m_l$. Each each entry of the L attention maps $m_l$ corresponds to the network’s attention score for the corresponding feature joint embedding at that position. 

%%%%%%% NOTES %%%%%%%
% Reliability map estimation for CNN-based camera model attribution https://arxiv.org/pdf/1805.01946.pdf

% This module generates attention maps, $M \in \mathbb{R}^{N \times d_{maps}}$, from the spatially contextualized forensic embeddings, $SCP \in \mathbb{R}^{N \times d_{embed}}$. Each of these maps is used to emphasize regions with high quality forensic traces or potential manipulations and suppress regions with low quality forensic traces. 
% Prior works \citelater{cite} have shown that the quality of forensic traces is diminished in places where the entropy is either too low or too high. 
% Additionally, since video coding dynamically adjusts the compression parameters for each block in a frame, the attention maps may also normalize attenuated forensic signals across the whole frame, allowing for more accurate comparisons.
% Prior works \citelater{cite} have shown that the information capacity can be sufficiently measured using Shannon's entropy $\mathbf{H}$:
% \begin{align}
%         \mathbf{H}(x_p) = - \sum_{k=0}^{255} p_k ln(p_k)
% \end{align}
% where $p_k$ is the probability that a pixel has luminance value $k$ in the analysis window $x_p$.
% Using deep, multiheaded self-attention, each input low-level feature vector is transformed in a way that reflects the relationships between it and every other token in the sample.
% This enables the learnable templates to examine all the transformed embeddings and extract regions with aberrant forensic traces that are not affected by extreme lighting or texture conditions. In addition, since multiple templates give rise to multiple attention maps, the model can maximize the amount of information extracted from the Transformer's embeddings. 



==> sections/revisions_old/03_transformer_module_v3_MCS.tex <==
\subsection{Transformer-Based Attention Module}
\label{subsec:transformer_module}

The sequence of joint embeddings is passed to the transformer-based attention module, which is designed to produce a series of $L$ different spatial attention maps.
% As is commonly done when using vision transformers, 
To encode spatial position information, 
a vector of 1-D learnable spatial embeddings is added to the joint embeddings before being passed to the transformer. The transformer consists of twelve transformer encoder blocks stacked on top of one another. The output of the transformer is passed to an ``Attention Squeeze'' layer that consists of $L$, $1\times 1$ convolutional kernels.  This ``squeezes'' down the high dimensional output to a series of $L$ different $M\times N$ spatial attention maps $m_l$. Each each entry of the $L$ attention maps $m_l$ corresponds to the network’s attention score for the corresponding joint feature embedding at that position. 


%[width=84mm]
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/attention_maps_v2.png}

    \vspace*{-0.5\baselineskip}

    \caption{Example showing the effect of our attention module.  The attention map produced for this frame gives large weights (shown in red) to regions with high quality forensic information - i.e. it has sufficient texture, illumination, no blurring, etc.  Regions with low quality forensic information are given low weight (shown in blue).}

    \label{fig:spatial_attn_example}

    \vspace*{-0.5\baselineskip}

\end{figure}
%\caption{Example showing the effect of our spatial attention module.  The attention map produced for this frame gives large weights (shown in red) to regions with high quality forensic information - i.e. it has sufficient texture, illumination, no blurring, etc.).  Regions with low quality forensic information are given low weight (shown in blue). }
%The attention map gives low weight (shown in blue) to regions with poor forensic traces  - i.e low texture, poor illumination, etc.) and high weight to regions with high quality forensic traces (sufficient texture, good illumination).

Fig.~\ref{fig:spatial_attn_example} shows an example of a spatial attention map produced by our transformer-based attention module, as well as the corresponding the unaltered video frame.  From this example, we can see that VideoFACT attends to regions that contain high-quality forensic traces, i.e. regions with sufficient texture, illumination, etc.  By contrast, regions known to contain low-quality forensic information such as the sky are de-emphasized.  
%
Often, these regions will cause false alarms because their low-quality forensic traces will appear anomalous with respect to the rest of the traces throughout the scene.  By not attending to these regions, our network can avoid these false alarms. 


%By not attending to these regions, our network can avoid producing false alarms in regions where forensic traces appear anomalous due to low quality information as opposed to 


%%%%%%% NOTES %%%%%%%
% Reliability map estimation for CNN-based camera model attribution https://arxiv.org/pdf/1805.01946.pdf

% This module generates attention maps, $M \in \mathbb{R}^{N \times d_{maps}}$, from the spatially contextualized forensic embeddings, $SCP \in \mathbb{R}^{N \times d_{embed}}$. Each of these maps is used to emphasize regions with high quality forensic traces or potential manipulations and suppress regions with low quality forensic traces. 
% Prior works \citelater{cite} have shown that the quality of forensic traces is diminished in places where the entropy is either too low or too high. 
% Additionally, since video coding dynamically adjusts the compression parameters for each block in a frame, the attention maps may also normalize attenuated forensic signals across the whole frame, allowing for more accurate comparisons.
% Prior works \citelater{cite} have shown that the information capacity can be sufficiently measured using Shannon's entropy $\mathbf{H}$:
% \begin{align}
%         \mathbf{H}(x_p) = - \sum_{k=0}^{255} p_k ln(p_k)
% \end{align}
% where $p_k$ is the probability that a pixel has luminance value $k$ in the analysis window $x_p$.
% Using deep, multiheaded self-attention, each input low-level feature vector is transformed in a way that reflects the relationships between it and every other token in the sample.
% This enables the learnable templates to examine all the transformed embeddings and extract regions with aberrant forensic traces that are not affected by extreme lighting or texture conditions. In addition, since multiple templates give rise to multiple attention maps, the model can maximize the amount of information extracted from the Transformer's embeddings. 



==> sections/revisions_old/04_video_manip_datasets_v1.tex <==
\section{Video Manipulations Datasets}
\label{sec:training_datasets}

In this section, we describe the datasets we created to train our network according to the progressively difficult manipulations training protocol specified in section \ref{subsec:training_protocol}. Since our protocol needs video data containing three types of manipulation: Simple Splicing, Visible Manipulations, and Invisible Manipulations, we generate three different datasets, each dataset satisfying one type of manipulation. In this paper, they are referred to as:
\begin{enumerate}[topsep=3pt]
\setlength\itemsep{-0.35em}
    \item The Video Camera Model Splicing (VCMS) Dataset
    \item The Video Perceptually Visible Manipulations (VPVM) Dataset
    \item The Video Perceptually Invisible Manipulations (VPIM) Dataset
\end{enumerate}
All datasets were built from the Video Authentication and Camera Identification Database (Video-ACID), which contained over 12,000 short clips ($\approx$5.8 seconds on average) using 46 physical devices representing 36 unique video-camera models \citelater{cite this later https://ieee-dataport.org/documents/video-acid}.

\subheader{Ground-Truth Mask Generation Strategy}
\label{subsec:ground_truth_mask_gen}
In order to introduce manipulations into video, we pick random shapes of random sizes and orientations at one or several spatial locations in each video to perform tampering operations. We implement this strategy using ten basic shapes: rectangle, circle, ellipse, triangle, pentagon, heptagon, 5-pointed star, 8-pointed star, 12-pointed star, and 18-pointed star. In addition, these shapes are allowed to combine into highly complex morphologies with a 0.5 probability. We then create a binary mask by marking the pixels in areas specified by a random morphology of random sizes and orientations at a random location with 1s and the rest with 0s.

\subheader{The Video Camera Model Splicing Dataset}
\label{subsec:VCMS}
This dataset contains tampering operations in which one or multiple regions of a source frame is copied and pasted onto a destination frame. Using videos from Video-ACID, we create disjoint sets of 3200 videos for training, 520 videos for validation, and 280 videos for testing. Each video contains 30 frames or 1 second. For each set, we select half of the videos as source videos and the other half as destination videos. The set of the camera models in the source videos must be disjoint from that in the destination videos. Finally, for every source-destination video pair, we spliced each source frame into each destination frame according to a randomized binary mask specified above.

\subheader{Video Perceptually Visible Manipulations}
\label{subsec:VPVM}
The VPVM dataset contains perceptually visible tampering operations applying to one or multiple regions of a victim frame. These manipulations contain at least one of the following operations: changing brightness, contrast, saturation, and hue, adding random Gaussian blur, random motion blur, random box blur, and random Gaussian noise. The operations done to a victim frame and their strength are randomly selected. To ensure the manipulation is visible to the human eye, we continually manipulate the entire victim frames until the Structural Similarity Index Measure \citelater{cite}, $\text{SSIM}$, between manipulated and original frame obeys
\begin{align}
    \text{SSIM}(F_v, F_m) \le 0.9
\end{align}
where $F_v$ is the victim frame and $F_m$ is the manipulated frame. Then, we splice the areas, indicated by a random binary mask, from the manipulated frame onto the victim frame. We repeat this strategy for every frame of every video in the disjointed training, validation, and testing set, which contains 1600, 260, and 140 videos, respectively. 
% TODO: cite https://ieeexplore.ieee.org/document/1284395
% TODO: cite https://arxiv.org/pdf/2006.13846.pdf
% TODO: cite https://arxiv.org/pdf/1511.08861.pdf

\subheader{Video Perceptually Invisible Manipulations}
\label{subsec:VPIM}
The VPIM dataset is created using the same approach as the VPVM dataset. The only exception is that the strength of the operations is much lower, such that the $\text{SSIM}$, must obey:
\begin{align}
    0.98 \ge \text{SSIM}(F_v, F_m) \ge 0.94
\end{align}
Through meticulous manual testing, out of 1000 generated samples, 97.5\% of manipulated areas in the victim frames cannot be detected with the human eye.

% TODO: cite these:
% http://live.ece.utexas.edu/publications/2009/cl_spie09.pdf
% https://arxiv.org/pdf/2006.13846.pdf
% https://www.scirp.org/journal/paperinformation.aspx?paperid=90911
% https://library.imaging.org/ei/articles/28/13/art00010
% https://ieeexplore.ieee.org/document/5635337




==> sections/revisions_old/04_video_manip_datasets_v2_Shengbang.tex <==
\section{Video Manipulations Datasets}
\label{sec:training_datasets}

%In this section, we describe the datasets we created to train our network according to the progressively difficult manipulations training protocol specified in section \ref{subsec:training_protocol}. Since our protocol needs video data containing three types of manipulation: Simple Splicing, Visible Manipulations, and Invisible Manipulations, we generate three different datasets, each dataset satisfying one type of manipulation. In this paper, they are referred to as:
In this section, we describe three datasets created by our self for model training protocal mentioned in section \ref{subsec:training_protocol}.
% reason
These datasets provide the model with a learning path with progressively increasing difficulty.
% each contains one  
Each dataset are generated to contain one of three different type of manipulations: splicing, visible manipulations, and invisible manipulations. 
% name them
The Video Camera Model Splicing Dataset(VCMS) contains videos with contents spliced from other videos, the Video Perceptually Visible Manipulations Dataset(VPVM) contains videos with visible manipulations and the Video Perceptually Invisible Manipulations Dataset(VPIM) contains videos with invisible manipulations.
% source videos
All three datasets were built from the Video Authentication and Camera Identification Database (Video-ACID)~\citelater{cite this later https://ieee-dataport.org/documents/video-acid}, which contained over 12,000 short clips ($\approx$5.8 seconds on average) using 46 physical devices from 36 unique video-camera models.

\subheader{Ground-Truth Mask Generation Strategy}
\label{subsec:ground_truth_mask_gen}
%In order to introduce manipulations into video, we pick random shapes of random sizes and orientations at one or several spatial locations in each video to perform tampering operations. 
To introduce manipulations into a video frame, we randomly pick one or more shapes from 10 base shapes.
% We implement this strategy using ten basic shapes: rectangle, circle, ellipse, triangle, pentagon, heptagon, 5-pointed star, 8-pointed star, 12-pointed star, and 18-pointed star.
These 10 base shapes include rectangle, circle, ellipse, triangle, pentagon, heptagon, 5-pointed star, 8-pointed star, 12-pointed star, and 18-pointed star.
%In addition, these shapes are allowed to combine into highly complex morphologies with a 0.5 probability. 
we pick these shapes in a random size and a random orientation, then combine picked shapes together into complex morphologies with a 0.5 probability.
%We then create a binary mask by marking the pixels in areas specified by a random morphology of random sizes and orientations at a random location with 1s and the rest with 0s.
A ground-truth mask for that frame is created by randomly add these random shapes and combined morphologies as the manipulated region. 

\subheader{The Video Camera Model Splicing Dataset}
\label{subsec:VCMS}
This dataset contains videos where one or more of their regions are spliced from the videos with different camera models.
%Using videos from Video-ACID, we create disjoint sets of 3200 videos for training, 520 videos for validation, and 280 videos for testing.
From Video-ACID, we select 3200 videos for creating training set, 520 videos for creating validation set and 280 videos for creating testing set. [Need verification because test should be more than valid]
%Each video contains 30 frames or 1 second. For each set, we select half of the videos as source videos and the other half as destination videos. 
%The set of the camera models in the source videos must be disjoint from that in the destination videos.
For each set, we select half of the camera models to provide the source videos, and the other half to provide the destination videos. We pair the source and destination videos randomly.  
Then for each source and destination video, we randomly select a continuous 30-frames slice, and spliced the contents from the source videos to the destination videos according to the groud-truth masks for each frame.
%Finally, for every source-destination video pair, we spliced each source frame into each destination frame according to a randomized binary mask specified above.
This results in 1600 videos for training, 260 videos for validation, and 140 videos for testing.

\subheader{Video Perceptually Visible Manipulations}
\label{subsec:VPVM}
This dataset contains videos with perceptually visible tampering operations in one or multiple regions. Each video contains at least one of the following manipulations: brightness, contrast, saturation, and hue adjustments, random Gaussian, motion, and box blurring, and random Gaussian noise. 
The parameters of these manipulations are randomly selected. 

To create the dataset, we follow the similar strategy in creating VCMS dataset to select video frames, but only choose the destination videos. For each frame we first copy the frame as the source frame.
To create perceptually visible manipulations, we continually manipulate the source frame until the Structural Similarity Index Measure \citelater{cite} $\text{SSIM}$ between the original and source frame become less then 0.9.
%\begin{align}
%    \text{SSIM}(F_v, F_m) \le 0.9
%\end{align}
% where $F_v$ is the victim frame and $F_m$ is the manipulated frame. 
%Then, we splice the areas, indicated by a random binary mask, from the manipulated frame onto the victim frame. We repeat this strategy for every frame of every video in the disjointed training, validation, and testing set, which contains 1600, 260, and 140 videos, respectively. 
Then, we splice contents from manipulated source frame into original frame using the ground-truth masks. 
% TODO: cite https://ieeexplore.ieee.org/document/1284395
% TODO: cite https://arxiv.org/pdf/2006.13846.pdf
% TODO: cite https://arxiv.org/pdf/1511.08861.pdf
We repeat this strategy for every frame of every video in the training, validation, and testing videos. The number of videos in training, validation and testing set are the same with VCMS Dataset. 


\subheader{Video Perceptually Invisible Manipulations}
\label{subsec:VPIM}
The VPIM dataset is created using the same approach as the VPVM dataset. The only exception is that the visibility of manipulations are much lower. We achieve this by change the $\text{SSIM}$ criteria between original and manipulated frames to be 
\begin{align}
    0.98 \ge \text{SSIM}(F_v, F_m) \ge 0.94
\end{align}
Through manual testing by ourselves, the manipulated areas from 97.5\% out of 1000 generated frames cannot be found by the human eyes.

% TODO: cite these:
% http://live.ece.utexas.edu/publications/2009/cl_spie09.pdf
% https://arxiv.org/pdf/2006.13846.pdf
% https://www.scirp.org/journal/paperinformation.aspx?paperid=90911
% https://library.imaging.org/ei/articles/28/13/art00010
% https://ieeexplore.ieee.org/document/5635337




==> sections/revisions_old/04_video_manip_datasets_v3TDN.tex <==
\section{Video Manipulations Datasets}
\label{sec:training_datasets}

%In this section, we describe the datasets we created to train our network according to the progressively difficult manipulations training protocol specified in section \ref{subsec:training_protocol}. Since our protocol needs video data containing three types of manipulation: Simple Splicing, Visible Manipulations, and Invisible Manipulations, we generate three different datasets, each dataset satisfying one type of manipulation. In this paper, they are referred to as:
In this section, we describe three datasets created by our self for model training protocol mentioned in section \ref{subsec:training_protocol}.
% reason
These datasets provide the model with a learning path with progressively increasing difficulty.
% each contains one  
Each dataset is generated to contain one of three different type of manipulations: splicing, visible manipulations, and invisible manipulations. 
% name them
The Video Camera Model Splicing Dataset(VCMS) contains videos with contents spliced from other videos, the Video Perceptually Visible Manipulations Dataset(VPVM) contains videos with visible manipulations and the Video Perceptually Invisible Manipulations Dataset(VPIM) contains videos with invisible manipulations.
% source videos
All three datasets were built from the Video Authentication and Camera Identification Database (Video-ACID)~\citelater{cite this later https://ieee-dataport.org/documents/video-acid}, which contained over 12,000 short clips ($\approx$5.8 seconds on average) using 46 physical devices from 36 unique video-camera models.

\subheader{Ground-Truth Mask Generation Strategy}
\label{subsec:ground_truth_mask_gen}
%In order to introduce manipulations into video, we pick random shapes of random sizes and orientations at one or several spatial locations in each video to perform tampering operations. 
To introduce manipulations into a video frame, we randomly pick one or more shapes from 10 base shapes.
% We implement this strategy using ten basic shapes: rectangle, circle, ellipse, triangle, pentagon, heptagon, 5-pointed star, 8-pointed star, 12-pointed star, and 18-pointed star.
These 10 base shapes include rectangle, circle, ellipse, triangle, pentagon, heptagon, 5-pointed star, 8-pointed star, 12-pointed star, and 18-pointed star.
%In addition, these shapes are allowed to combine into highly complex morphologies with a 0.5 probability. 
we pick these shapes in a random size and a random orientation, then combine picked shapes together into complex morphologies with a 0.5 probability.
%We then create a binary mask by marking the pixels in areas specified by a random morphology of random sizes and orientations at a random location with 1s and the rest with 0s.
A ground-truth mask for that frame is created by randomly add these random shapes and combined morphologies as the manipulated region. 

\subheader{The Video Camera Model Splicing Dataset}
\label{subsec:VCMS}
This dataset contains videos where one or more of their regions are spliced from the videos with different camera models.
%Using videos from Video-ACID, we create disjoint sets of 3200 videos for training, 520 videos for validation, and 280 videos for testing.
From Video-ACID, we select 3200 videos for creating training set, 520 videos for creating validation set and 280 videos for creating testing set.
%Each video contains 30 frames or 1 second. For each set, we select half of the videos as source videos and the other half as destination videos. 
%The set of the camera models in the source videos must be disjoint from that in the destination videos.
For each set, we select half of the camera models to provide the source videos, and the other half to provide the destination videos. We pair the source and destination videos randomly.  
Then for each source and destination video, we randomly select a continuous 30-frames slice, and spliced the contents from the source videos to the destination videos according to the ground-truth masks for each frame. We then compress the destination video's authentic frames and the destination video's manipulated frames into two videos, one authentic, one altered. To create these videos, we use the H.264 video codec from the FFmpeg software package with the constant rate factor set at 23 and the frame rate set to 30 FPS. Finally, we extract all frames from these compressed videos for training and analysis.
%Finally, for every source-destination video pair, we spliced each source frame into each destination frame according to a randomized binary mask specified above.
This results in 3200 videos (96000 frames) for training, 520 videos (15600 frames) for validation, and 280 videos (8400 frames) for testing.

\subheader{Video Perceptually Visible Manipulations}
\label{subsec:VPVM}
This dataset contains videos with perceptually visible tampering operations in one or multiple regions. Each video contains at least one of the following manipulations: brightness, contrast, saturation, and hue adjustments, random Gaussian, motion, and box blurring, and random Gaussian noise. 
The parameters of these manipulations are randomly selected. 

To create the dataset, we follow the similar strategy in creating VCMS dataset to select video frames and create compressed videos, but only choose the destination videos. For each frame we first copy the frame as the source frame.
To create perceptually visible manipulations, we continually manipulate the source frame until the Structural Similarity Index Measure \citelater{cite} $\text{SSIM}$ between the original and source frame become less than 0.9.
%\begin{align}
%    \text{SSIM}(F_v, F_m) \le 0.9
%\end{align}
% where $F_v$ is the victim frame and $F_m$ is the manipulated frame. 
%Then, we splice the areas, indicated by a random binary mask, from the manipulated frame onto the victim frame. We repeat this strategy for every frame of every video in the disjointed training, validation, and testing set, which contains 1600, 260, and 140 videos, respectively. 
Then, we splice contents from manipulated source frame into original frame using the ground-truth masks. 
% TODO: cite https://ieeexplore.ieee.org/document/1284395
% TODO: cite https://arxiv.org/pdf/2006.13846.pdf
% TODO: cite https://arxiv.org/pdf/1511.08861.pdf
We repeat this strategy for every frame of every video in the training, validation, and testing videos. The number of videos in training, validation and testing set are the same with VCMS Dataset. 


\subheader{Video Perceptually Invisible Manipulations}
\label{subsec:VPIM}
The VPIM dataset is created using the same approach as the VPVM dataset. The only exception is that the visibility of manipulations are much lower. We achieve this by change the $\text{SSIM}$ criteria between original and manipulated frames to be 
\begin{align}
    0.98 \ge \text{SSIM}(F_v, F_m) \ge 0.94
\end{align}
Through manual testing by ourselves, the manipulated areas from 97.5\% out of 1000 generated frames cannot be found by the human eyes.

% TODO: cite these:
% http://live.ece.utexas.edu/publications/2009/cl_spie09.pdf
% https://arxiv.org/pdf/2006.13846.pdf
% https://www.scirp.org/journal/paperinformation.aspx?paperid=90911
% https://library.imaging.org/ei/articles/28/13/art00010
% https://ieeexplore.ieee.org/document/5635337

\subheader{Additional Datasets Created From Images}
\label{subsec:image_datasets}
To further improve our network's generalizability, as indicated in the training protocol (section \ref{subsec:training_protocol}), we expose the network to more scene diversity. To facilitate this, we generate additional datasets based on the images from the Camera Model Identification Database (CMID) \citelater{cite} only for training. These image datasets are created by following the exact same approach as the three video datasets above. The first image dataset will contain camera model splicing manipulations, the second will have perceptually visible manipulations, and the third will be consisted of perceptually invisible manipulations. Each image dataset contains 96000 training samples, 15600 validation samples, and 8400 testing samples.



==> sections/revisions_old/04_video_manip_datasets_v4_Shengbang.tex <==
\section{Experimental Video Datasets}
\label{sec:training_datasets}
Since there's not existing video manipulation dataset large enough to train and evaluate our proposed model, we create a series of new datasets with a variety of manipulation scales and types, and also select one existing dataset.
These datasets are divided into Set A and B. All datasets made by us will be made public upon publication.

\subsection{Set A: Video Manipulated Datasets}
We made three different datasets with different types of manipulation from Video-ACID~\citelater{videoacid} dataset. All three datasets are made using a similar procedure. First, we create ground-truth mask with multiple random components indicating tampering region of the video frames for each frame. Then we add manipulated content to the video frame using the mask. We also keep the original pristine frames for creating authentic videos. Finally we re-compressed the frames into manipulated and authentic videos using ffmpeg with H.264 encoding~\citelater{h.264} with the constant rate factor set to 23 and the frame rate set to 30 FPS.

We choose three different manipulation types and create datasets for each of them. Video Camera Model Splicing Dataset (VCMS) contains contents spliced from other videos. Video Perceptually Manipulation Dataset (VPVM) contains in-place perceptual visible manipulated regions, like brightness adjustment, contrast enhancement, and etc. Video Perceptually Invisible Manipulation Dataset (VPIM) contains also in-place but invisible manipulation in the videos.

For each dataset in this set, we made 3200 videos (96000 frames) for training,
520 videos (15600 frames) for validation, and 280 videos
(8400 frames) for testing.

\subsection{Set B: In-the-wild Manipulated Datasets}
The in-the-wild datasets contain 3 different, challenging manipulation with very different scene contents, and are used only for evaluation.
They are VideoSham~\citelater{videosham}, Inpainting Video~\citelater{Inpaint}, and Deepfake Video~\citelater{DF}

The VideoSham \citelater[cite] is made by Adobe Research, which contains high-quality videos manipulated by professional editors. Because this work focuses exclusively on identifying fake content, we excluded videos’ audio and those with temporal manipulations. 
Additionally, videos of resolution less than our network’s input size $1920 \times 1080$ were also excluded. 
% can be written in table
This results 7897 frames from 32 manipulated videos, and 12746 frames from 64 authentic videos.

The Inpainting Video is made by us using E2FGVI-HQ~\citelater{inpaint} to remove segmented objects, which are specified in the Densely Annotated Video Segmentation (DAVIS) dataset~\citelater{DAVIS}. Using the authors’ recommended settings, we generate 540p videos then resize them to 1080p so that they can be analyzed by our network. 
% can be written in tbale
We got 9312 frames from 90 videos for both authentic and manipulated videos.

The Deepfake Video is also made by us using Deepfacelab~\citelater{Deepfacelab}. It is generated from publicly available videos of celebrities download from YouTube. We make sure each video is in good illumination, no background replacing, so that it contains enough forensic features. 
%
We generated 10 deepfake videos and choose 10 other original videos. Then sampled 30 frames for each of the video.


\begin{comment}
%In this section, we describe the datasets we created to train our network according to the progressively difficult manipulations training protocol specified in section \ref{subsec:training_protocol}. Since our protocol needs video data containing three types of manipulation: Simple Splicing, Visible Manipulations, and Invisible Manipulations, we generate three different datasets, each dataset satisfying one type of manipulation. In this paper, they are referred to as:
Since there's not existing video manipulation dataset we can use to train our proposed model, we create a new video manipulation dataset with a variety of manipulation scales and types.
In this section, we describe three video manipulation datasets and three image manipulation we created for model training protocol mentioned in section \ref{subsec:training_protocol}.
% reason
These datasets provide the model with a learning path with progressively increasing difficulty.
% each contains one  
As mentioned above, each dataset is generated to contain one of three different type of manipulations: splicing, visible manipulations, and invisible manipulations. 
% name them
%The Video Camera Model Splicing Dataset(VCMS) contains videos with contents spliced from other videos, the Video Perceptually Visible Manipulations Dataset(VPVM) contains videos with visible manipulations and the Video Perceptually Invisible Manipulations Dataset(VPIM) contains videos with invisible manipulations.
% source videos
All three videos datasets were built from the Video Authentication and Camera Identification Database (Video-ACID)~\citelater{cite this later https://ieee-dataport.org/documents/video-acid}, which contained over 12,000 short clips ($\approx$5.8 seconds on average) from 36 unique video-camera models. All three image datasets were built from Camera Model Identification Dataset (CMID), which contains images from 70 camera models.

\subheader{Ground-Truth Mask Generation}
\label{subsec:ground_truth_mask_gen}
%In order to introduce manipulations into video, we pick random shapes of random sizes and orientations at one or several spatial locations in each video to perform tampering operations. 
We first create ground truth mask for each video frame / images. To introduce manipulations, we randomly pick one or more shapes from 10 base shapes.
% We implement this strategy using ten basic shapes: rectangle, circle, ellipse, triangle, pentagon, heptagon, 5-pointed star, 8-pointed star, 12-pointed star, and 18-pointed star.
These 10 base shapes include rectangle, circle, ellipse, triangle, pentagon, heptagon, 5-pointed star, 8-pointed star, 12-pointed star, and 18-pointed star.
%In addition, these shapes are allowed to combine into highly complex morphologies with a 0.5 probability. 
we pick these shapes in a random size and a random orientation, then combine the selected shapes together into complex morphologies with a 0.5 probability.
%We then create a binary mask by marking the pixels in areas specified by a random morphology of random sizes and orientations at a random location with 1s and the rest with 0s.
A ground-truth mask for that frame is created by randomly add these random shapes and combined morphologies as the manipulated region. 

\subheader{The Video Camera Model Splicing Dataset}
\label{subsec:VCMS}
This dataset contains videos where one or more of their regions are spliced from the videos with different camera models.
%Using videos from Video-ACID, we create disjoint sets of 3200 videos for training, 520 videos for validation, and 280 videos for testing.
From Video-ACID, we select 3200 videos for creating training set, 520 videos for creating validation set and 280 videos for creating testing set.
%Each video contains 30 frames or 1 second. For each set, we select half of the videos as source videos and the other half as destination videos. 
%The set of the camera models in the source videos must be disjoint from that in the destination videos.
For each set, we select half of the camera models to provide the source videos, and the other half to provide the destination videos. We pair the source and destination videos randomly.  
Then for each source and destination video, we randomly select a continuous 30-frames slice, and spliced the contents from the source videos to the destination videos according to the ground-truth masks for each frame. We then compress the  manipulated destination frames into a new manipulated video. We also decode and recompress the original destination videos as the authentic videos. 
When creating videos, we use the H.264 video codec from the FFmpeg software package with the constant rate factor set at 23 and the frame rate set to 30 FPS. 
This results in 3200 videos (96000 frames) for training, 520 videos (15600 frames) for validation, and 280 videos (8400 frames) for testing.
Finally, we extract all frames from these compressed videos for training and analysis.
%Finally, for every source-destination video pair, we spliced each source frame into each destination frame according to a randomized binary mask specified above.

\subheader{Video Perceptually Visible Manipulations}
\label{subsec:VPVM}
This dataset contains videos with perceptually visible tampering operations in one or multiple regions. Each video contains at least one of the following manipulations: brightness, contrast, saturation, and hue adjustments, random Gaussian, motion, and box blurring, and random Gaussian noise. 
The parameters of these manipulations are randomly selected. 

To create tise dataset, we follow the similar pathway in creating VCMS dataset  but only choose the destination videos. For each frame we first copy the frame as the source frame, then continually manipulate the source frame until the Structural Similarity Index Measure \citelater{cite} $\text{SSIM}$ between the original and source frame become less than 0.9.
%\begin{align}
%    \text{SSIM}(F_v, F_m) \le 0.9
%\end{align}
% where $F_v$ is the victim frame and $F_m$ is the manipulated frame. 
%Then, we splice the areas, indicated by a random binary mask, from the manipulated frame onto the victim frame. We repeat this strategy for every frame of every video in the disjointed training, validation, and testing set, which contains 1600, 260, and 140 videos, respectively. 
Then, we splice contents from manipulated source frame into original frame using the ground-truth masks. 
% TODO: cite https://ieeexplore.ieee.org/document/1284395
% TODO: cite https://arxiv.org/pdf/2006.13846.pdf
% TODO: cite https://arxiv.org/pdf/1511.08861.pdf
We repeat this strategy for every frame of every video.

\subheader{Video Perceptually Invisible Manipulations}
\label{subsec:VPIM}
The VPIM dataset is created using the same approach as the VPVM dataset. The only exception is that the visibility of manipulations are much lower. We achieve this by change the $\text{SSIM}$ criteria between original and manipulated frames to be 
\begin{align}
    0.98 \ge \text{SSIM}(F_v, F_m) \ge 0.94
\end{align}
Through manual testing by ourselves, the manipulated areas from 97.5\% out of 1000 generated frames cannot be found by the human eyes.

% TODO: cite these:
% http://live.ece.utexas.edu/publications/2009/cl_spie09.pdf
% https://arxiv.org/pdf/2006.13846.pdf
% https://www.scirp.org/journal/paperinformation.aspx?paperid=90911
% https://library.imaging.org/ei/articles/28/13/art00010
% https://ieeexplore.ieee.org/document/5635337

\subheader{Additional Datasets Created From Images}
\label{subsec:image_datasets}
These three image datasets are to provide the model more scene diversity and improve our network's generalizability during training. These image datasets are created by following the exact same approach as the three video datasets above. The first image dataset will contain camera model splicing manipulations (ICMS), the second will have perceptually visible manipulations (IPVM), and the third will be consisted of perceptually invisible manipulations (IPIM). Each image dataset contains 96000 training images.%, 15600 validation images, and 8400 testing samples.
\end{comment}


==> sections/revisions_old/04_video_manip_datasets_v5_MCS.tex <==
% 04_video_manip_datasets_v5_MCS.tex


\section{Video Forgery Datasets}
\label{sec:training_datasets}
%Currently, there are no publicly available datasets of manipulated video large enough to train %video 
%forgery detection and localization networks.  Similarly, there are almost no datasets of maniplated video suitable to evaluate our network, with the noteable exception of the Adobe VideoSham dataset, which was released in July 2022~\cite{mittal2022videoSham}.  


Currently, there are no publicly available datasets of manipulated video large enough to train %video 
forgery detection and localization networks.  Similarly, there are almost no datasets suitable to evaluate such networks, with the noteable exception of the Adobe VideoSham dataset, which was released in July 2022~\cite{mittal2022videoSham}.  
%
To address this issue, we created a series of new video manipulation datasets for training and evaluating our network.  These are divided into two subsets.  Set A contains videos modified using standard manipulations, e.g. splicing and local editing, etc.  Set B contains ``in-the-wild'' videos made using more sophisticated editing operations such as inpainting, deepfakes, etc.  All datasets will be made publicly available upon publication of this paper.


%Since there's not existing video manipulation dataset large enough to train and evaluate our proposed model, we create a series of new datasets with a variety of manipulation scales and types, and also select one existing dataset. These datasets are divided into Set A and B. All datasets made by us will be made public upon publication.

\subsection{Set A: Standard Video Manipulations Datasets}
%We made three different datasets of videos modified using different types of standard manipulations from the Video-ACID~\cite{hosler2019video} dataset. 

%We made three  datasets of modified videos by applying standard manipulations to videos from the Video-ACID~\cite{hosler2019video} dataset.  
We made three  datasets %of modified videos created 
by applying different sets of standard manipulations to videos from the Video-ACID~\cite{hosler2019video} dataset.  
All three datasets were made using a common procedure.  
First, we created binary ground-truth masks specifying the tamper regions for each video.  These tamper regions correspond to multiple randomly chosen shapes with random sizes, orientations, and placements within a frame.
% First, we created ground-truth masks with multiple random components indicating tampering region of the video frames for each frame. 
Fake videos were created by choosing a mask, then manipulating content within the tamper region.  Pristine copies of each original video were also retained to create a set of authentic videos.  All video frames (both manipulated and authentic) were re-encoded as H.264 videos using FFmpeg~\cite{FFmpeg} with a constant rate factor of 23 and a 30 FPS frame rate.

%the frames into manipulated and authentic videos using ffmpeg with H.264 encoding~\citelater{h.264} with the constant rate factor set to 23 and the frame rate set to 30 FPS.

Each dataset in Set A corresponds to a different manipulation type.  The \textbf{Video Camera Model Splicing (VCMS)} dataset  contains videos with content spliced in from other videos.  The \textbf{Video Perceptually Visible Manipulation (VPVM)} dataset contains content modified using common editing operations such as contrast enhancement, smoothing, sharpening, blurring, etc. applied with strengths that can be visually detected.  
The \textbf{Video Perceptually Invisible Manipulation (VPIM)} dataset was made in a similar fashion to the VPVM, but using much smaller manipulation strengths to create challenging forgeries. 
%For each dataset in this set, 
For each dataset, we made 3200 videos (96000 frames) for training,
520 videos (15600 frames) for validation, and 280 videos
(8400 frames) for testing.

% to VPVM, but the manipulation strengths were chosen to invisible to the human eye.

%The Video Perceptually Invisible Manipulation (VPIM) dataset was made in a similar fashion to VPVM, but the manipulation strengths were chosen to invisible to the human eye.

%We choose three different manipulation types and create datasets for each of them. Video Camera Model Splicing Dataset (VCMS) contains contents spliced from other videos. Video Perceptually Manipulation Dataset (VPVM) contains in-place perceptual visible manipulated regions, like brightness adjustment, contrast enhancement, and etc. Video Perceptually Invisible Manipulation Dataset (VPIM) contains also in-place but invisible manipulation in the videos.

\input{tables/training_stages_params}

\subsection{Set B: In-the-Wild Manipulated Datasets}

We used three ``in-the-wild'' datasets to evaluate our network: VideoSham~\cite{mittal2022videoSham} created by Adobe Research, and both the Inpainted Video and Deepfake Video datasets created by us.  These datasets contain advanced, challenging manipulations applied to videos with scene content that significantly differs from our training datasets.
%as well as varied scene content that differs from our training datasets.


%The in-the-wild datasets contain 3 different, challenging manipulation with very different scene contents, and are used only for evaluation.
%They are VideoSham~\citelater{videosham}, Inpainting Video~\citelater{Inpaint}, and Deepfake Video~\citelater{DF}


\textbf{VideoSham}~\cite{mittal2022videoSham} contains high-quality videos manipulated by professional editors using multiple techniques. Because this work focuses exclusively on identifying fake content, we excluded videos with audio track or temporal manipulations. Additionally, videos of with resolution less than our network’s input size of $1920 \times 1080$ pixels were also excluded. 
% can be written in table
This resulted in 7897 frames from 32 manipulated videos, and 12746 frames from 64 authentic videos.

%The VideoSham \citelater[cite] is made by Adobe Research, which contains high-quality videos manipulated by professional editors. Because this work focuses exclusively on identifying fake content, we excluded videos’ audio and those with temporal manipulations. 
%Additionally, videos of resolution less than our network’s input size $1920 \times 1080$ were also excluded. 
%This results 7897 frames from 32 manipulated videos, and 12746 frames from 64 authentic videos.

%The Inpainted Video dataset was made by using E2FGVI-HQ~\citelater{inpaint} to remove segmented objects, which are specified in the Densely Annotated Video Segmentation (DAVIS) dataset~\citelater{DAVIS}. Using the authors’ recommended settings, we generate 540p videos then resize them to 1080p so that they can be analyzed by our network.  We got 9312 frames from 90 videos for both authentic and manipulated videos.


%The Inpainted Video dataset was made by using E2FGVI-HQ~\citelater{inpaint} to remove  objects specified by segmentation masks from videos in the Densely Annotated Video Segmentation (DAVIS) dataset~\citelater{DAVIS}.   


Our \textbf{Inpainted Video} dataset was made by using inpainting to remove objects specified by segmentation masks from videos in the Densely Annotated Video Segmentation (DAVIS) dataset~\cite{pont2017DAVIS}.  Inpainting was performed with E2FGVI-HQ~\cite{E2FGVI} using the authors' recommended settings, producing output videos in 540p resolution.  They were then resized to 1080p so that they could be analyzed by our network.  This dataset contains  both authentic and manipulated subsets that each contain  of 9312 frames from 90 videos.
%This dataset contains subsets of both authentic and manipulated videos that each contain  of 9312 frames from 90 videos.


%This was done using the  authors’ recommended settings, we generate 540p videos then resize them to 1080p so that they can be analyzed by our network.  We got 9312 frames from 90 videos for both authentic and manipulated videos.

%Our Deepfake Video dataset was made by  using DeepFaceLab~\citelater{Deepfacelab} to create deepfakes from a set of publicly available videos of celebrities downloaded from YouTube.  




Our \textbf{Deepfake Video} dataset was made by  creating deepfakes from a set of publicly available videos of celebrities downloaded from YouTube.  These deepfakes were generated using DeepFaceLab~\cite{DeepFaceLab} to ensure that all fake videos were of 1080p resolution, created as a video rather than a sequence of individually compressed images, and utilized deepfake creation software that is currently most commonly used in the wild.
Our dataset consists of a manipulated subset of 300 frames from 10 high-quality deepfake videos and  an unaltered subset of 300 frames from 10 original videos.
%
We note that this dataset was created to evaluate and demonstrate our network's ability to detect a wide variety of video forgeries.  Our purpose is not to create a dedicated deepfake detector.


%These videos were chosen to have only a single face, no background replacement
%We did not use existing datasets such as the DeefakeTIMIT,  DFDC, or FaceForensics++ datasets because we wanted to ensure that videos are all in 1080p resolution and were made using current deepfake creation software.  

%. It is generated from publicly available videos of celebrities download from YouTube. We make sure each video is in good illumination, no background replacing, so that it contains enough forensic features. We generated 10 deepfake videos and choose 10 other original videos. Then sampled 30 frames for each of the video.

%Our Deepfake Video is also made by us using Deepfacelab~\citelater{Deepfacelab}. It is generated from publicly available videos of celebrities download from YouTube. We make sure each video is in good illumination, no background replacing, so that it contains enough forensic features. We generated 10 deepfake videos and choose 10 other original videos. Then sampled 30 frames for each of the video.


\begin{comment}
%In this section, we describe the datasets we created to train our network according to the progressively difficult manipulations training protocol specified in section \ref{subsec:training_protocol}. Since our protocol needs video data containing three types of manipulation: Simple Splicing, Visible Manipulations, and Invisible Manipulations, we generate three different datasets, each dataset satisfying one type of manipulation. In this paper, they are referred to as:
Since there's not existing video manipulation dataset we can use to train our proposed model, we create a new video manipulation dataset with a variety of manipulation scales and types.
In this section, we describe three video manipulation datasets and three image manipulation we created for model training protocol mentioned in section \ref{subsec:training_protocol}.
% reason
These datasets provide the model with a learning path with progressively increasing difficulty.
% each contains one  
As mentioned above, each dataset is generated to contain one of three different type of manipulations: splicing, visible manipulations, and invisible manipulations. 
% name them
%The Video Camera Model Splicing Dataset(VCMS) contains videos with contents spliced from other videos, the Video Perceptually Visible Manipulations Dataset(VPVM) contains videos with visible manipulations and the Video Perceptually Invisible Manipulations Dataset(VPIM) contains videos with invisible manipulations.
% source videos
All three videos datasets were built from the Video Authentication and Camera Identification Database (Video-ACID)~\citelater{cite this later https://ieee-dataport.org/documents/video-acid}, which contained over 12,000 short clips ($\approx$5.8 seconds on average) from 36 unique video-camera models. All three image datasets were built from Camera Model Identification Dataset (CMID), which contains images from 70 camera models.

\subheader{Ground-Truth Mask Generation}
\label{subsec:ground_truth_mask_gen}
%In order to introduce manipulations into video, we pick random shapes of random sizes and orientations at one or several spatial locations in each video to perform tampering operations. 
We first create ground truth mask for each video frame / images. To introduce manipulations, we randomly pick one or more shapes from 10 base shapes.
% We implement this strategy using ten basic shapes: rectangle, circle, ellipse, triangle, pentagon, heptagon, 5-pointed star, 8-pointed star, 12-pointed star, and 18-pointed star.
These 10 base shapes include rectangle, circle, ellipse, triangle, pentagon, heptagon, 5-pointed star, 8-pointed star, 12-pointed star, and 18-pointed star.
%In addition, these shapes are allowed to combine into highly complex morphologies with a 0.5 probability. 
we pick these shapes in a random size and a random orientation, then combine the selected shapes together into complex morphologies with a 0.5 probability.
%We then create a binary mask by marking the pixels in areas specified by a random morphology of random sizes and orientations at a random location with 1s and the rest with 0s.
A ground-truth mask for that frame is created by randomly add these random shapes and combined morphologies as the manipulated region. 

\subheader{The Video Camera Model Splicing Dataset}
\label{subsec:VCMS}
This dataset contains videos where one or more of their regions are spliced from the videos with different camera models.
%Using videos from Video-ACID, we create disjoint sets of 3200 videos for training, 520 videos for validation, and 280 videos for testing.
From Video-ACID, we select 3200 videos for creating training set, 520 videos for creating validation set and 280 videos for creating testing set.
%Each video contains 30 frames or 1 second. For each set, we select half of the videos as source videos and the other half as destination videos. 
%The set of the camera models in the source videos must be disjoint from that in the destination videos.
For each set, we select half of the camera models to provide the source videos, and the other half to provide the destination videos. We pair the source and destination videos randomly.  
Then for each source and destination video, we randomly select a continuous 30-frames slice, and spliced the contents from the source videos to the destination videos according to the ground-truth masks for each frame. We then compress the  manipulated destination frames into a new manipulated video. We also decode and recompress the original destination videos as the authentic videos. 
When creating videos, we use the H.264 video codec from the FFmpeg software package with the constant rate factor set at 23 and the frame rate set to 30 FPS. 
This results in 3200 videos (96000 frames) for training, 520 videos (15600 frames) for validation, and 280 videos (8400 frames) for testing.
Finally, we extract all frames from these compressed videos for training and analysis.
%Finally, for every source-destination video pair, we spliced each source frame into each destination frame according to a randomized binary mask specified above.

\subheader{Video Perceptually Visible Manipulations}
\label{subsec:VPVM}
This dataset contains videos with perceptually visible tampering operations in one or multiple regions. Each video contains at least one of the following manipulations: brightness, contrast, saturation, and hue adjustments, random Gaussian, motion, and box blurring, and random Gaussian noise. 
The parameters of these manipulations are randomly selected. 

To create tise dataset, we follow the similar pathway in creating VCMS dataset  but only choose the destination videos. For each frame we first copy the frame as the source frame, then continually manipulate the source frame until the Structural Similarity Index Measure \citelater{cite} $\text{SSIM}$ between the original and source frame become less than 0.9.
%\begin{align}
%    \text{SSIM}(F_v, F_m) \le 0.9
%\end{align}
% where $F_v$ is the victim frame and $F_m$ is the manipulated frame. 
%Then, we splice the areas, indicated by a random binary mask, from the manipulated frame onto the victim frame. We repeat this strategy for every frame of every video in the disjointed training, validation, and testing set, which contains 1600, 260, and 140 videos, respectively. 
Then, we splice contents from manipulated source frame into original frame using the ground-truth masks. 
% TODO: cite https://ieeexplore.ieee.org/document/1284395
% TODO: cite https://arxiv.org/pdf/2006.13846.pdf
% TODO: cite https://arxiv.org/pdf/1511.08861.pdf
We repeat this strategy for every frame of every video.

\subheader{Video Perceptually Invisible Manipulations}
\label{subsec:VPIM}
The VPIM dataset is created using the same approach as the VPVM dataset. The only exception is that the visibility of manipulations are much lower. We achieve this by change the $\text{SSIM}$ criteria between original and manipulated frames to be 
\begin{align}
    0.98 \ge \text{SSIM}(F_v, F_m) \ge 0.94
\end{align}
Through manual testing by ourselves, the manipulated areas from 97.5\% out of 1000 generated frames cannot be found by the human eyes.

% TODO: cite these:
% http://live.ece.utexas.edu/publications/2009/cl_spie09.pdf
% https://arxiv.org/pdf/2006.13846.pdf
% https://www.scirp.org/journal/paperinformation.aspx?paperid=90911
% https://library.imaging.org/ei/articles/28/13/art00010
% https://ieeexplore.ieee.org/document/5635337

\subheader{Additional Datasets Created From Images}
\label{subsec:image_datasets}
These three image datasets are to provide the model more scene diversity and improve our network's generalizability during training. These image datasets are created by following the exact same approach as the three video datasets above. The first image dataset will contain camera model splicing manipulations (ICMS), the second will have perceptually visible manipulations (IPVM), and the third will be consisted of perceptually invisible manipulations (IPIM). Each image dataset contains 96000 training images.%, 15600 validation images, and 8400 testing samples.
\end{comment}


==> sections/revisions_old/05_comparison_v1.tex <==
\subsection{Comparison with prior works}
\label{subsec:comparison_with_prior_works}

Now, we compare our algorithm against top-performing ones in the field of multimedia forensics: Forensic Similarity Graph (FSG) \citelater{cite}, EXIFnet \citelater{cite}, Noiseprint \citelater{cite}, ManTra-Net \citelater{cite}, and MVSS-Net \citelater{cite}. These algorithms represent a broad spectrum of successful techniques (i.e., abnormal edge detection and aberrant noise or residual detection) using different architectural designs (fully convolutional, Siamese, and multi-view attention networks). We also note that Noiseprint and ManTra-Net are primarily designed to produce localization masks. Hence, to make fair frame-level detection comparisons with Noiseprint and Mantra-Net, we obtain a frame-level detection score by averaging the normalized the per-pixel detection probabilities.

\subheader{Group A datasets}
Table \ref{table:results_on_our_datasets} shows the performance comparison between competing architectures and ours. Our architecture is the top performer in all categories. Surprisingly, in the most straightforward and noticeable tampering scenarios (VCMS, VPVM), previously successful image forensic algorithms fail to produce \textit{any} meaningful predictions. On the VPIM test set, these techniques (both edge and noise-based), interestingly, cannot make sense of the local tampering operations even though some of these operations were encountered in training \citelater{cite}. Therefore, we can see that state-of-the-art image forensic algorithms do no better than random guessing. On the contrary, our proposed approach correctly determines if a video frame has been tampered with and points out the manipulation region. This demonstrates that combining the model's design and our training protocol creates a strong system against video tampering. 

\subheader{Group B datasets} 
Table \ref{table:results_on_itw_datasets} presents the performance metrics comparison between our algorithms and others on three different "in-the-wild" datasets. Again, the disadvantages of using previously successful image forensics algorithms show here. 

First, the VideoSham dataset contains professionally edited video clips using Adobe After Effects. Hence, the quality of the manipulations is very high. This means that the editors pay close attention to the edge, scene, and context of the subjects, objects, or texts they are adding in or taking out. Therefore, excluding some obvious splicing, most manipulations are hard to detect with the human eye. Additionally, many edits are confined to tiny areas (i.e., adding/removing a small bird in a zoomed-out sky), much smaller than our minimum analysis window ($128 \times 128$ pixels). Hence, we see our network retaining smaller gains over competing algorithms, for example, comparing to Mantra-Net, we have a lead of 0.103 in detection ACC and a gain of 0.200 in localization F1. However, because other algorithms do little to no better than random guessing, our strong positive performance is especially consequential.

Second, as the Inpainted Video dataset is generated using the E2FGVI-HQ \citelater{cite} algorithm, it represents the tests in which synthetic contents produced by deep neural networks are inserted into a video. Our model retains a considerable lead in both frame-level and pixel-level detection performance. In particular, comparing to EXIFnet, our detection mAP is 0.147 higher and our localization F1 is 0.056 better. We note that our localization metrics are lowered (compared to those datasets seen in training) because the generation process requires the video to be resized, which significantly damages, alters, or smoothens some forensic and contextual information \citelater{cite}. However, our network is still able to largely labeled the correct manipulated areas, albeit some authentic areas are false-alarmed. 

Third, .... VideoMatting...



==> sections/revisions_old/05_comparison_v1_Shengbang.tex <==
\subsection{Detection and Localization Performance}
\label{subsec:comparison_with_prior_works}
%We evaluated our proposed algorithm on datasets in group A and B. 
We evaluate our proposed approach on both group A and B datasets, and compare the results with other competing image-based anomaly detection and localization algorithms. 
%Now, we compare our algorithm against top-performing ones in the field of multimedia forensics: 
The competing methods includes Forensic Similarity Graph (FSG) \citelater{cite}, EXIFnet \citelater{cite}, Noiseprint \citelater{cite}, ManTra-Net \citelater{cite}, and MVSS-Net \citelater{cite}. These algorithms represent a broad spectrum of successful techniques on anomaly localization and/or detection in images. 
We note that Noiseprint and Mantra-Net do not automatically perform detection.
To make fair frame-level comparisons on detection, we averaging the normalized per-pixel localization probabilities as the predicted scores of manipulation detection.

\subheader{Group A Seen datasets}
Table \ref{table:results_on_our_datasets} shows the performance of our proposed method and the competing algorithms. 
%Our architecture is the top performer in all categories. Surprisingly, in the most straightforward and noticeable tampering scenarios (VCMS, VPVM), previously successful image forensic algorithms fail to produce \textit{any} meaningful predictions. On the VPIM test set, these techniques (both edge and noise-based), interestingly, cannot make sense of the local tampering operations even though some of these operations were encountered in training \citelater{cite}. Therefore, we can see that state-of-the-art image forensic algorithms do no better than random guessing. On the contrary, our proposed approach correctly determines if a video frame has been tampered with and points out the manipulation region. This demonstrates that combining the model's design and our training protocol creates a strong system against video tampering. 
Through Table \ref{table:results_on_our_datasets} we show that our proposed approach achieve a strong performance and outperforms all other competing algorithms. Though our model performance drop in invisible manipulations in VPIM, it can still have a mAP of 0.869 for detection and a F-1 score of 0.547 for localization. These results  show that our proposed method can successfully detect and localize the manipulation contents in videos. 
While our performance are high, these competing algorithms cannot detect and localize the manipulated content in the videos. Even on splicing videos in VCMS, the competing algorithms still performs close to random guess. These are consistent with the difference compression method between images and videos

\subheader{Group B "in-the-wild" datasets} 
Table \ref{table:results_on_itw_datasets} presents the performance metrics comparison between our algorithms and others on three different "in-the-wild" datasets. Again, the disadvantages of using previously successful image forensics algorithms show here. 

First, the VideoSham dataset contains professionally edited video clips using Adobe After Effects. Hence, the quality of the manipulations is very high. This means that the editors pay close attention to the edge, scene, and context of the subjects, objects, or texts they are adding in or taking out. Therefore, excluding some obvious splicing, most manipulations are hard to detect with the human eye. Additionally, many edits are confined to tiny areas (i.e., adding/removing a small bird in a zoomed-out sky), much smaller than our minimum analysis window ($128 \times 128$ pixels). Hence, we see our network retaining smaller gains over competing algorithms, for example, comparing to Mantra-Net, we have a lead of 0.103 in detection ACC and a gain of 0.200 in localization F1. However, because other algorithms do little to no better than random guessing, our strong positive performance is especially consequential.

Second, as the Inpainted Video dataset is generated using the E2FGVI-HQ \citelater{cite} algorithm, it represents the tests in which synthetic contents produced by deep neural networks are inserted into a video. Our model retains a considerable lead in both frame-level and pixel-level detection performance. In particular, comparing to EXIFnet, our detection mAP is 0.147 higher and our localization F1 is 0.056 better. We note that our localization metrics are lowered (compared to those datasets seen in training) because the generation process requires the video to be resized, which significantly damages, alters, or smoothens some forensic and contextual information \citelater{cite}. However, our network is still able to largely labeled the correct manipulated areas, albeit some authentic areas are false-alarmed. 

Third, .... VideoMatting...



==> sections/revisions_old/05_comparison_v2_MCS.tex <==
\subsection{Detection and Localization Performance}
\label{subsec:comparison_with_prior_works}
%We evaluated our proposed algorithm on datasets in group A and B. 


%We compared the performance of our network to several competing networks on the six evaluation datasets described in Section~\ref{sec:training_datasets}

We evaluated the performance of our network on the six evaluation datasets described in Section~\ref{sec:training_datasets} and compared to several competing methods.
%We compared the performance of our network to several competing methods, including 
These include Forensic Similarity Graphs (FSG) \citelater{cite}, EXIFnet \citelater{cite}, Noiseprint \citelater{cite}, ManTra-Net \citelater{cite}, and MVSS-Net \citelater{cite}, and represent represent a broad spectrum of successful techniques for performing forgery detection and localization in images.  
We note that Noiseprint and Mantra-Net do not automatically perform detection.  To fairly compare against these networks, we obtain frame-level detection scores by computing the average normalized per-pixel detection probability.





\subheader{Set A: Standard Video Manipulations}
Table \ref{table:results_on_our_datasets} shows the performance of our proposed network and competing networks on the three Standard Video Manipulations datasets in Set A.






%Our architecture is the top performer in all categories. Surprisingly, in the most straightforward and noticeable tampering scenarios (VCMS, VPVM), previously successful image forensic algorithms fail to produce \textit{any} meaningful predictions. On the VPIM test set, these techniques (both edge and noise-based), interestingly, cannot make sense of the local tampering operations even though some of these operations were encountered in training \citelater{cite}. Therefore, we can see that state-of-the-art image forensic algorithms do no better than random guessing. On the contrary, our proposed approach correctly determines if a video frame has been tampered with and points out the manipulation region. This demonstrates that combining the model's design and our training protocol creates a strong system against video tampering. 
Through Table \ref{table:results_on_our_datasets} we show that our proposed approach achieve a strong performance and outperforms all other competing algorithms. Though our model performance drop in invisible manipulations in VPIM, it can still have a mAP of 0.869 for detection and a F-1 score of 0.547 for localization. These results  show that our proposed method can successfully detect and localize the manipulation contents in videos. 
While our performance are high, these competing algorithms cannot detect and localize the manipulated content in the videos. Even on splicing videos in VCMS, the competing algorithms still performs close to random guess. These are consistent with the difference compression method between images and videos

\subheader{Group B "in-the-wild" datasets} 
Table \ref{table:results_on_itw_datasets} presents the performance metrics comparison between our algorithms and others on three different "in-the-wild" datasets. Again, the disadvantages of using previously successful image forensics algorithms show here. 

First, the VideoSham dataset contains professionally edited video clips using Adobe After Effects. Hence, the quality of the manipulations is very high. This means that the editors pay close attention to the edge, scene, and context of the subjects, objects, or texts they are adding in or taking out. Therefore, excluding some obvious splicing, most manipulations are hard to detect with the human eye. Additionally, many edits are confined to tiny areas (i.e., adding/removing a small bird in a zoomed-out sky), much smaller than our minimum analysis window ($128 \times 128$ pixels). Hence, we see our network retaining smaller gains over competing algorithms, for example, comparing to Mantra-Net, we have a lead of 0.103 in detection ACC and a gain of 0.200 in localization F1. However, because other algorithms do little to no better than random guessing, our strong positive performance is especially consequential.

Second, as the Inpainted Video dataset is generated using the E2FGVI-HQ \citelater{cite} algorithm, it represents the tests in which synthetic contents produced by deep neural networks are inserted into a video. Our model retains a considerable lead in both frame-level and pixel-level detection performance. In particular, comparing to EXIFnet, our detection mAP is 0.147 higher and our localization F1 is 0.056 better. We note that our localization metrics are lowered (compared to those datasets seen in training) because the generation process requires the video to be resized, which significantly damages, alters, or smoothens some forensic and contextual information \citelater{cite}. However, our network is still able to largely labeled the correct manipulated areas, albeit some authentic areas are false-alarmed. 

Third, .... VideoMatting...



==> sections/revisions_old/05_comparison_v3_Shengbang.tex <==
\subsection{Detection and Localization Performance}
\label{subsec:comparison_with_prior_works}
%We evaluated our proposed algorithm on datasets in group A and B. 


%We compared the performance of our network to several competing networks on the six evaluation datasets described in Section~\ref{sec:training_datasets}

We evaluated the performance of our network on the six evaluation datasets described in Section~\ref{sec:training_datasets} and compared to several competing methods.
%We compared the performance of our network to several competing methods, including 
These include Forensic Similarity Graphs (FSG) \citelater{cite}, EXIFnet \citelater{cite}, Noiseprint \citelater{cite}, ManTra-Net \citelater{cite}, and MVSS-Net \citelater{cite}, representing a broad spectrum of successful techniques for performing forgery detection and localization in images.  
We note that Noiseprint and Mantra-Net do not automatically perform detection.  To fairly compare against these networks, we obtain frame-level detection scores by computing the average normalized per-pixel detection probability.





\subheader{Set A: Standard Video Manipulations}
Table \ref{table:results_on_our_datasets} shows the performance of our proposed network and competing networks on the three Standard Video Manipulations datasets in Set A.
We show that out approach performs best by a large margin in every dataset. The only exception is MVSSNet's localization on VCMS, where we perform comparably.
By contrast, the existing networks largely do no better than random guess. 
This phenomenon can be clearly seen in both Table \ref{table:results_on_our_datasets} and the qualitative results presented in Fig \ref{fig:localization_results}, which was also observed in benchmarking experiments reported in the VideoSham paper~\citelater{VideoSham}.
The set A overall results shows that video forgeries exhibit different effects than image forgeries, which existing networks are unable to adapt to.





%Our architecture is the top performer in all categories. Surprisingly, in the most straightforward and noticeable tampering scenarios (VCMS, VPVM), previously successful image forensic algorithms fail to produce \textit{any} meaningful predictions. On the VPIM test set, these techniques (both edge and noise-based), interestingly, cannot make sense of the local tampering operations even though some of these operations were encountered in training \citelater{cite}. Therefore, we can see that state-of-the-art image forensic algorithms do no better than random guessing. On the contrary, our proposed approach correctly determines if a video frame has been tampered with and points out the manipulation region. This demonstrates that combining the model's design and our training protocol creates a strong system against video tampering. 

 

%Through Table \ref{table:results_on_our_datasets} we show that our proposed approach achieve a strong performance and outperforms all other competing algorithms.
%Though our model performance drop in invisible manipulations in VPIM, it can still have a mAP of 0.869 for detection and a F-1 score of 0.547 for localization. 
%These results  show that our proposed method can successfully detect and localize the manipulation contents in videos. 


%Even on splicing videos in VCMS, competing algorithms still perform close to random guess. These are consistent with the difference compression method between images and videos

\subheader{Set B "In-the-Wild" Datasets} 
Table \ref{table:results_on_itw_datasets} shows the performance of our proposed method and existing networks on the three "in-the-wild" datasets, which consists much more complex and challenging forgeries. 
Across all datasets, we uniformly perform the best across all datasets, while other approaches still largely fail. When other approaches don't fail completely, their performance are unstable across different datasets. This reinforce the observation on Set A and can be seen in both Table \ref{table:results_on_itw_datasets} and Fig \ref{fig:localization_results}.

In Deepfake Video, note that our algorithm isn't explicitly designed to detect deepfakes and doesn't exploit useful semantic information such as human face or natural motion. Despite this, our results demonstrate that we can still achieve reasonable performance on these challenging forgeries.

In Inpainted Video, this data has been rescaled significantly to make it 1080p resolution. It is well-known that rescaling significantly downgrades the quality of forensic information. Despite this, we can still achieve good detection and localization performance.

In VideoSham, which contains very high-quality and challenging forgeries, Many falsified regions are small and even much smaller than our analysis window. Our approach still achieve a significantly better detection result, and the best localization over existing algorithms.



\begin{comment}
Table \ref{table:results_on_itw_datasets} presents the performance comparison between our algorithms and others on three different "in-the-wild" datasets. 
%Again, the disadvantages of using previously successful image forensics algorithms show here.
We note that we don't explicitly train on these datasets, nor training on similar types of manipulations. 
Though our performance drop to a lower level, it still outperforms all other competing algorithms. 
We achieve 0.782 detection mAP in Inpainted Video dataset, which shows a significant advantage comparing to edge-based methods (like MVSS-Net) since there's no obvious edge in such scenarios. In Deepfake video dataset, we also achieve a significant higher localization score. We also note that these deepfake videos also contain low-quality forensic region such as dark blank region due to aspect rotation, captions, and watermarks. Our proposed method shows we somewhat overcome these contents even though we don't train to recognize these regions. On VideoSham, editing are well-refined and have multiple different types of editing 


First, the VideoSham dataset contains professionally edited video clips using Adobe After Effects. Hence, the quality of the manipulations is very high. This means that the editors pay close attention to the edge, scene, and context of the subjects, objects, or texts they are adding in or taking out. Therefore, excluding some obvious splicing, most manipulations are hard to detect with the human eye. Additionally, many edits are confined to tiny areas (i.e., adding/removing a small bird in a zoomed-out sky), much smaller than our minimum analysis window ($128 \times 128$ pixels). Hence, we see our network retaining smaller gains over competing algorithms, for example, comparing to Mantra-Net, we have a lead of 0.103 in detection ACC and a gain of 0.200 in localization F1. However, because other algorithms do little to no better than random guessing, our strong positive performance is especially consequential.

Second, as the Inpainted Video dataset is generated using the E2FGVI-HQ \citelater{cite} algorithm, it represents the tests in which synthetic contents produced by deep neural networks are inserted into a video. Our model retains a considerable lead in both frame-level and pixel-level detection performance. In particular, comparing to EXIFnet, our detection mAP is 0.147 higher and our localization F1 is 0.056 better. We note that our localization metrics are lowered (compared to those datasets seen in training) because the generation process requires the video to be resized, which significantly damages, alters, or smoothens some forensic and contextual information \citelater{cite}. However, our network is still able to largely labeled the correct manipulated areas, albeit some authentic areas are false-alarmed. 

Third, .... VideoMatting...

\end{comment}

==> sections/revisions_old/05_comparison_v4_MCS.tex <==
\subsection{Detection and Localization Performance}
\label{subsec:comparison_with_prior_works}
%We evaluated our proposed algorithm on datasets in group A and B. 


%We compared the performance of our network to several competing networks on the six evaluation datasets described in Section~\ref{sec:training_datasets}

%We evaluated the performance of our network on the six evaluation datasets described in Section~\ref{sec:training_datasets} and compared to several competing methods.
%We compared the performance of our network to several competing methods, including 
We compared the performance of VideoFACT to several existing image forensic networks including 
%These include 
Forensic Similarity Graphs (FSG) \cite{FSG}, EXIFnet \cite{EXIFnet}, Noiseprint \cite{Noiseprint}, ManTra-Net \cite{ManTra-Net}, and MVSS-Net \cite{MVSS-Net}, representing a broad spectrum of successful techniques for performing forgery detection and localization in images.  
We note that Noiseprint and Mantra-Net do not automatically perform detection.  To fairly compare against these networks, we obtain frame-level detection scores by computing the average normalized per-pixel detection probability.





\subheader{Set A: Standard Video Manipulations}
Table \ref{table:results_on_our_datasets} shows the performance of our proposed network and competing networks on the three Standard Video Manipulations datasets in Set A.
These results show that VideoFACT achieves the best performance by a large margin on these datasets. The only exception is for  the VCMS dataset, where MVSS-Net's localization performance is slightly better than ours, though still comparable.
Except for this case, existing networks largely do no better than a random guess (i.e. $\mbox{mAP}=0.5$ and $\mbox{MCC}=0$).  This phenomenon can be clearly seen in both Table~\ref{table:results_on_our_datasets} and the qualitative results presented in Fig~\ref{fig:localization_results}.  These results reinforce similar findings reported in the VideoSham paper~\cite{mittal2022videoSham}, that is, existing networks are unable to adapt to forensic differences between image and video forgeries.


%We show that out approach performs best by a large margin in every dataset. 
%The only exception is MVSSNet's localization on VCMS, where we perform comparably. By contrast, the existing networks largely do no better than random guess. This phenomenon can be clearly seen in both Table \ref{table:results_on_our_datasets} and the qualitative results presented in Fig \ref{fig:localization_results}, which was also observed in benchmarking experiments reported in the VideoSham paper~\citelater{VideoSham}. The set A overall results shows that video forgeries exhibit different effects than image forgeries, which existing networks are unable to adapt to.





%Our architecture is the top performer in all categories. Surprisingly, in the most straightforward and noticeable tampering scenarios (VCMS, VPVM), previously successful image forensic algorithms fail to produce \textit{any} meaningful predictions. On the VPIM test set, these techniques (both edge and noise-based), interestingly, cannot make sense of the local tampering operations even though some of these operations were encountered in training \citelater{cite}. Therefore, we can see that state-of-the-art image forensic algorithms do no better than random guessing. On the contrary, our proposed approach correctly determines if a video frame has been tampered with and points out the manipulation region. This demonstrates that combining the model's design and our training protocol creates a strong system against video tampering. 

 

%Through Table \ref{table:results_on_our_datasets} we show that our proposed approach achieve a strong performance and outperforms all other competing algorithms.
%Though our model performance drop in invisible manipulations in VPIM, it can still have a mAP of 0.869 for detection and a F-1 score of 0.547 for localization. 
%These results  show that our proposed method can successfully detect and localize the manipulation contents in videos. 


%Even on splicing videos in VCMS, competing algorithms still perform close to random guess. These are consistent with the difference compression method between images and videos

\subheader{Set B: ``In-the-Wild'' Datasets} 
%
Table \ref{table:results_on_itw_datasets} shows the performance of our network and existing networks on the three ``in-the-wild'' datasets, which consists much more complex and challenging forgeries. 
These results show that VideoFACT uniformly achieves the best detection and localization performance over all three datasets.  By contrast, existing approaches typically fail on these challenging datasets.  This can be observed in the qualitative results presented in Fig.~\ref{fig:localization_results}.  %Existing networks that do not fail completely are unable to achieve consistently non-random performance across all datasets.  
These results further solidify our observations on Set A and results reported in the VideoSham paper~\cite{VideoSham} that existing image forensic networks largely fail on falsified videos.





%Across all datasets, we uniformly perform the best across all datasets, while other approaches still largely fail. When other approaches don't fail completely, their performance are unstable across different datasets. This reinforce the observation on Set A and can be seen in both Table \ref{table:results_on_itw_datasets} and Fig \ref{fig:localization_results}.

For the Deepfake Video dataset, we note that while our network significantly outperforms image forensic networks, it is unlikely to outperform dedicated deepfake detectors~\cite{Huang_2022_TIFS, Zhao_2021_CVPR, Luo_2021_CVPR, Jiang_2020_CVPR}.  This is because our network doesn't leverage useful semantic information such human face %or natural motion 
models that deepfake detectors typically do.  Despite this, these results show that our network can still achieve reasonable performance %on these challenging forgeries
without explicitly training on deepfakes. 

%In Deepfake Video, note that our algorithm isn't explicitly designed to detect deepfakes and doesn't exploit useful semantic information such as human face or natural motion. Despite this, our results demonstrate that we can still achieve reasonable performance on these challenging forgeries.

Additionally, we note that videos in the Inpainted Video dataset have been resized up to  1080p resolution.  This is important because it is well-known that rescaling significantly downgrades the quality of forensic information.  Despite this, we can still achieve good detection and localization performance on this dataset. 
%
%One reason that existing networks fail on this dataset is likely because most networks are trained to identify added or enhanced content, not removed content.



%In Inpainted Video, this data has been rescaled significantly to make it 1080p resolution. It is well-known that rescaling significantly downgrades the quality of forensic information. Despite this, we can still achieve good detection and localization performance.

The results we obtain on the VideoSham dataset are  influenced by the size of the falsified region in each video.  Some of these videos contain fake content that is much smaller than the size of our network's $128 \times 128$ analysis windows.  %These small forgeries represent an important challenge 
Our network has a difficult time identifying these forgeries.  Despite this, we still achieve %consistently 
better performance than other existing image forensic networks on this dataset.


%In VideoSham, which contains very high-quality and challenging forgeries, Many falsified regions are small and even much smaller than our analysis window. Our approach still achieve a significantly better detection result, and the best localization over existing algorithms.




==> sections/revisions_old/05_discussion_v1.tex <==
\subsection{Discussion}
\label{subsec:discussion}

\subheader{Speculation on why image forensic algorithms fail on videos}
From the results above, we observed that the forensic features, in which image forensic algorithms learned to extract, may not be transferable to videos. Unlike images, compression parameters within a frame are locally non-uniform, i.e., there are over 75 macroblock types \citelater{cite h264}, with each having different sizes and compression parameters, based on the past, current and future content. Hence, approaches, which make decisions based solely on comparing forensic information from different analysis windows, often produce lots of false alarm due to each block's forensic information being degraded or distorted unevenly. 

\textbf{Our algorithm}, contrarily, based its decision on all the available forensic, contextual and spatial information. Hence, our model obtains a more holistic view of the processing history contained in a video frame. We notice that it performs well when the tampering content's area is greater or equal to our analysis window. Furthermore, we found that on rare occasions, we fail to identify objects spliced into super textured region, such as grasses, tiled roads, dense forest, and extremely dark region (see Figure \todolater{cite a figure}). We suspect that this is because our training data lack such examples - the majority of the Video-ACID and the Image-CMID contain daytime, urban scenery on or near a single physical location. Therefore, it is possible that we can raise the performance of our network by including samples with more diverse conditions into our training data. 


%%%%% NOTES %%%%%
% Observing the results shown above, we believe these reasons may have contributed to the failing of previous techniques on videos:
% \begin{itemize}
%     \item Forensic features learned in images may not be transferred to videos.
%     \item Unlike images, compression parameters on a video frame are non-unified. There are over 75 macroblock types \citelater{cite h264}, with each having different sizes and compression parameters, based on the past, current and future content. In addition to being context-adaptive, video codecs like h.264 are also bitrate-adaptive. Therefore, forensic algorithms trained on images, which ignore contextual information, are likely to find the forensic information to be different in every analysis window, and not able make good comparisons between them.
%     \item Image forensic approaches often fail when encounter images with regions that have extreme lighting conditions (overly saturated, overly darkened), or abnormally high pixel frequency \citelater{cite}. We speculate that the information capacity of these regions are either too low, or too high. If the forensic information is stored on a very low entropic region, its quality maybe degraded, and contrarily, if it is stored on a very high entropic region, it is often distorted. Hence, the forensic features extracted from these areas may need to be suppressed. 
% \end{itemize} 

==> sections/revisions_old/05_discussion_v1_Shengbang.tex <==
\subsection{Discussion}
\label{subsec:discussion}

\subheader{Image forensic algorithms on Videos Manipulation}
From the results above, we observed that the image forensic algorithms for forgery detection and localization do not perform well on videos. This might indicate that the forensic features of images do not transfer well to videos. Which is consistent with the different compression way between images and videos. H.264 video encoding \citelater{cite h264} might results varying micro-block forensic traces in a frame due to adaptive compression methods. Hence, the approaches trained on images could often produce lots of false alarm on video frames. On the contrary, our model is trained to adaptive to such video encoding methods and results a much better performance.

\subheader{Attention Mechanism} We notice that it performs well when the tampering content's area is greater or equal to our analysis window. Furthermore, we found that on rare occasions, we fail to identify objects spliced into high-texture or low-texture region, such as grasses, tiled roads, dense forest, and extremely dark region (see Figure \todolater{cite a figure}). We suspect that this is because our training data lack such examples. The majority of the Video-ACID and the Image-CMID contain daytime, urban scenery on or near a single physical location. Therefore, it is possible that we can raise the performance of our network by including samples with more diverse conditions into our training data.



%%%%% NOTES %%%%%
% Observing the results shown above, we believe these reasons may have contributed to the failing of previous techniques on videos:
% \begin{itemize}
%     \item Forensic features learned in images may not be transferred to videos.
%     \item Unlike images, compression parameters on a video frame are non-unified. There are over 75 macroblock types \citelater{cite h264}, with each having different sizes and compression parameters, based on the past, current and future content. In addition to being context-adaptive, video codecs like h.264 are also bitrate-adaptive. Therefore, forensic algorithms trained on images, which ignore contextual information, are likely to find the forensic information to be different in every analysis window, and not able make good comparisons between them.
%     \item Image forensic approaches often fail when encounter images with regions that have extreme lighting conditions (overly saturated, overly darkened), or abnormally high pixel frequency \citelater{cite}. We speculate that the information capacity of these regions are either too low, or too high. If the forensic information is stored on a very low entropic region, its quality maybe degraded, and contrarily, if it is stored on a very high entropic region, it is often distorted. Hence, the forensic features extracted from these areas may need to be suppressed. 
% \end{itemize} 

==> sections/revisions_old/05_discussion_v2_MCS.tex <==
\subsection{Discussion}
\label{subsec:discussion}



From the results presented in Tables~\ref{table:results_on_our_datasets} and \ref{table:results_on_itw_datasets}, we can see that existing approaches, which reported strong performance on image forgeries, largely fail on video.  
There are multiple reasons why this may occurs.

\subheader{Effects of Video Compression}
%
Coding and compression is well-known to have a significant effect on forensic traces~\cite{Kirchner_2010_TSOP, Popescu_2005_ITSP, Bayar_2017_ICASSP}.
One key reason why existing networks suffer significant performance decreases on video is likely due to differences between image and video compression.

Existing forgery detection networks are trained and validated using images.  While many of these networks are resilient to JPEG 
%compression 
effects, it is important to note that JPEG operates in the same manner throughout an image, irrespective of the underlying scene content.  
% As a result, JPEG has a uniform effect on the underlying forensic traces throughout an image.
As a result, JPEG has a uniform effect on the forensic traces throughout an image. 
%\textit{which existing networks can often compensate for.}

By contrast, video compression does not operate in a spatially uniform manner.  Modern  standards like H.264 utilize a large number of macroblock types within a single frame, which are chosen based on the underlying scene content, motion, and several other factors~\cite{H264}.
Different macroblock types employ different coding techniques and parameters, resulting in different regional compression strengths throughout a frame.  This can induce localized inconsistencies in forensic traces, which will cause existing networks to incorrectly flag some regions as fake or manipulated.
%
%Coding and compression is well known to have a significant effect on forensic traces.  %While images and videos both typically undergo compression, 
%Important differences between image and video compression likely leads to effects that significantly decrease the performance existing networks.

%Existing forgery detection networks are trained and validated using images.  While many of these networks are resilient to image compression effects, image compression is substantially different than video coding.  JPEG compression operates in a uniform manner throughout an image irrespective of the underlying scene content.  As a result, JPEG has a uniform effect on the underlying forensic traces throughout an image.

%By contrast, video coding does not operate in a spatially uniform manner.  Modern  standards like H.264 utilize a wide variety of macroblock types within a single frame, which are chosen based on the underlying scene content, motion, and several other factors. Different macroblock types employ different coding techniques and parameters, resulting in different local compression strengths throughout a video frame.  This, in turn, can induce localized inconsistencies in forensic traces, which will result in existing networks incorrectly flagging content as fake or manipulated.

% maybe swap "false detection" for false alarm for 
\subheader{False Alarm Effects}
%
Another important reason why our network outperforms existing networks is its ability to avoid certain types of false alarms in unmanipulated regions.  An example of this can be seen in Fig.~\ref{fig:falsification_example}.  
Here, existing networks produce false alarms in different ways that can be grouped according to how each network operates.

One set of existing approaches, such as EXIFnet, FSG, and Noiseprint, identify fake content by searching for anomalous forensic traces.  These networks will produce false alarms in scene regions that contain little forensic information such as the sky.  This is because these networks will often mistake low quality forensic traces for anomalous traces.

Another set of approaches, such as ManTra-Net and MVSS-Net,  seek to learn good forgery detection features by analyzing noise residuals and edge information.  These techniques can false alarm when highly salient foreground objects naturally exhibit different statistics from background objects.  This effect occurs in the man sitting on the rock in Fig.~\ref{fig:falsification_example}.  This natural variation will cause the noise residuals and edge information in the foreground objects to appear anomalous to these networks.

\subheader{How Our Network Overcomes These Effects}
%\subheader{Overcoming These Effects}
%\subheader{Overcoming Compression and False Alarmm Effects}
Our network's use of context embeddings and spatial attention enables it to be much more resilient to the effects described above.
%to video compression effects and false alarm effects than existing work.  
%By utilizing local context information from the scene, our network is able to learn how to control for local variations in forensic traces induced by video compression.
%Our deep, transformer-based spatial attention module is able to learn which scene regions contain sufficient forensic information to attend to when making detection and localization decisions. This enables it to avoid many of the false alarm issues faced by other networks.
%
Our deep attention module allows our network to learn which scene regions contain high quality forensic information. 
Therefore, VideoFACT relies more heavily on these regions when making decisions and avoid many of the false alarm issues faced by other networks.  
Additionally, local context information enables our network to control for local variations in forensic traces induced by video compression as well as naturally occurring statistical variations induced by scene content.

%Our deep attention module enables our network to learn which scene regions contain high quality forensic information.  
%\subheader{Limitations and Failure Cases}
\subheader{Failure Cases and Limitations}
%
%When examining videos in the ``in-the-wild" datasets, we identified several common failure cases experienced by our network. 
We identified several common failure cases experienced by our network by examining videos in the  ``in-the-wild'' datasets. 
Specifically, our network often miss-detects when: (1) The falsified region is very small, in particular when its area is much smaller than our $128\times 128$ pixels analysis window. (2) Both the manipulated region and background have similar poor lighting conditions, and (3) The manipulated region has been altered by color swaps.  %We note that this manipulation is noticeably different from others encounterd by our network during training.  
%
Additionally, our network has limitations including: (1) It doesn't exploit temporal effects or correlations between frames. 
%information that can be gathered by examining dependencies between frames. 
(2) Our current implementation is only suitable for a fixed input video resolution of 1080p.


%Limitations of our approach: (1) don't exploit temporal effects - additional information can be gleaned by exploiting dependencies between frames (2) current implementation is only for fixed input size of 1080p

%%%%% NOTES %%%%%
% Observing the results shown above, we believe these reasons may have contributed to the failing of previous techniques on videos:
% \begin{itemize}
%     \item Forensic features learned in images may not be transferred to videos.
%     \item Unlike images, compression parameters on a video frame are non-unified. There are over 75 macroblock types \citelater{cite h264}, with each having different sizes and compression parameters, based on the past, current and future content. In addition to being context-adaptive, video codecs like h.264 are also bitrate-adaptive. Therefore, forensic algorithms trained on images, which ignore contextual information, are likely to find the forensic information to be different in every analysis window, and not able make good comparisons between them.
%     \item Image forensic approaches often fail when encounter images with regions that have extreme lighting conditions (overly saturated, overly darkened), or abnormally high pixel frequency \citelater{cite}. We speculate that the information capacity of these regions are either too low, or too high. If the forensic information is stored on a very low entropic region, its quality maybe degraded, and contrarily, if it is stored on a very high entropic region, it is often distorted. Hence, the forensic features extracted from these areas may need to be suppressed. 
% \end{itemize} 

==> sections/revisions_old/05_experimental_setup_v1.tex <==
\subsection{Experimental Setup}
\label{subsec:experimental_setup}

\subheader{Datasets} 
We evaluated the performance of our proposed network on multiple datasets. These datasets are divided into two groups, A and B. Group A consists of videos that have been falsified using manipulations that our network has encountered during training. Contrarily, Group B consists of ``in-the-wild'' videos that have been edited using manipulations and editing operations that were never encountered during training.  Furthermore, the scene content differs substantially from the training data. Particularly, Group A has the VCMS, the VPVM, and the VPIM dataset, and Group B has the VideoSham, the VideoMatting, and the Inpainted Video dataset.

\textit{The VideoSham dataset} \citelater{cite}, made by Adobe Research, contains high-quality videos manipulated by professional editors. Because this work focuses exclusively on identifying fake content, we excluded videos with audio or temporal manipulations. Additionally, videos of resolution less than $1080 \times 1920$, our network's input size, were also excluded. 

\textit{The VideoMatting dataset} \citelater{cite} has videos consisting of a subject or object in the foreground and background, which is matted (replaced) using video matting algorithms.

\textit{The Inpainted Video dataset} is created by applying a state-of-the-art video inpainting technique - E2FGVI-HQ \citelater{cite} to remove segmented objects, which are specified in the Densely Annotated Video Segmentation (DAVIS) dataset \citelater{cite}, by inpainting them out of a scene. Using the authors' recommended settings, we generate 540p videos then resize them to 1080p so that they can be analyzed by our network. Note that resizing has been proven by prior works \citelater{cite} to have a great influence upon the forensic traces in the original frame. Hence, this is an important source of data distribution mismatch that we will explore in the sections below.

\input{tables/summary_test_datasets}

\subheader{Evaluation Metrics} 
For frame-level manipulation detection, we report the mean average precision (mAP) for each dataset. Also, we provide the average accuracy (ACC) per datasets using a unified threshold of 0.5 to reflect real-world's performance.

For forgery localization, i.e., pixel-level manipulation detection, we pick 0.5 as the threshold and use F1 and MCC scores to evaluate the correlation between the predicted and the ground-truth localization mask. Since these scores describe the localization performance, they are only evaluated on manipulated samples. 

\subheader{Training Implementation} We implemented our models using PyTorch and trained them on an NVIDIA RTX 3090. The input size is $1080 \times 1920$ ($\text{height} \times \text{width}$). We first pretrained the FFE on the Video-ACID dataset using the Stochastic Gradient Descent (SGD) optimizer with an initial learning rate of $1.0\mathrm{e}{-3}$, momentum of $0.95$, and an exponential decay-rate of $0.5$ for every $2$ epochs. We let MISLnet trained until its training loss stopped improving. 
After pretraining the FFE, we trained the entire network following the five stages described in section \ref{subsec:training_protocol} with different training parameters shown in Table \ref{table:training_stages_parameters}. Throughout the stages, we set $\lambda = 0.4$, and we stop training when validation loss stop decreasing.

\input{tables/training_stages_params}

\input{tables/results_vcms_vpvm_vpim}

\input{tables/results_in_the_wild}


==> sections/revisions_old/05_experimental_setup_v1_Shengbang.tex <==
\subsection{Experimental Setup}
\label{subsec:experimental_setup}

\subheader{Training Implementation} We implemented our models using PyTorch and trained them on an NVIDIA RTX 3090. The input size is $1080 \times 1920$ ($\text{height} \times \text{width}$). We first pretrained the FFE on the Video-ACID dataset using the Stochastic Gradient Descent (SGD) optimizer with an initial learning rate of $1.0\mathrm{e}{-3}$, momentum of $0.95$, and an exponential decay-rate of $0.5$ for every $2$ epochs. We let FFE trained until its training loss stopped improving and discard the classification output layer. 
After pretraining the FFE, we trained the entire network following the five stages described in section \ref{subsec:training_protocol} with different training parameters shown in Table \ref{table:training_stages_parameters}. Throughout the stages, we set $\lambda = 0.4$, and we stop training when validation loss stop decreasing. After training, we evaluate the performance of our proposed approach as shown in the following.

\subheader{Evaluation Datasets} 
We evaluated the frame-level performance of our proposed network on videos from Set A's testing set and Set B.



\begin{comment}
We evaluated the performance of our proposed network on multiple video datasets. These datasets are divided into two groups. Group A consists of videos that has been seen by the model during training, which consists of test sets of VCMS, the VPVM, and the VPIM dataset.  Group B consists of ``in-the-wild'' videos that have manipulations and edited content that were never seen by the model during training, which consists of the VideoSham, VideoMatting and Inpainted Video dataset. Group B dataset are only used for evaluation.

[Might need Revision, VideoMatting]

The VideoSham dataset \citelater{cite} is made by Adobe Research, which contains high-quality videos manipulated by professional editors. Because this work focuses exclusively on identifying fake content, we excluded videos' audio and those with temporal manipulations. Additionally, videos of resolution less than our network's input size $1080 \times 1920$ were also excluded. 

The VideoMatting dataset \citelater{cite} has videos consisting of a subject or object in the foreground and background, which is matted (replaced) using video matting algorithms.

The Inpainted Video dataset is created by applying E2FGVI-HQ \citelater{cite} to remove segmented objects, which are specified in the Densely Annotated Video Segmentation (DAVIS) dataset \citelater{cite}. Using the authors' recommended settings, we generate 540p videos then resize them to 1080p so that they can be analyzed by our network. Note that resizing has been proven by prior works \citelater{cite} to have a great influence upon the forensic traces in the original frame. Hence, this is an important source of data distribution mismatch that we will explore in the sections below.
\end{comment}

%\input{tables/summary_test_datasets}

\subheader{Evaluation Metrics} 
For frame-level manipulation detection, we report the mean average precision (mAP) for each dataset. Also, we provide the average accuracy (ACC) per datasets using a unified threshold of 0.5 to reflect real-world's performance.

For forgery pixel-level manipulation localization, we pick 0.5 as the threshold and use F1 and MCC scores to evaluate the correlation between the predicted and the ground-truth localization mask. Since these scores describe the localization performance, they are only evaluated on manipulated samples. 



\input{tables/training_stages_params}

\input{tables/results_vcms_vpvm_vpim}

\input{tables/results_in_the_wild}


==> sections/revisions_old/05_experimental_setup_v2_MCS.tex <==
% 05_experimental_setup_v2_MCS

%\subsection{Experimental Setup}
%\label{subsec:experimental_setup}

\subheader{Training Implementation} We implemented our network using PyTorch and trained it using an NVIDIA RTX 3090. The network input size is $1080 \times 1920$ pixels %($\text{height} \times \text{width}$). 
(a single 1080p frame).  
We first pre-trained the FFE on the Video-ACID dataset using the Stochastic Gradient Descent (SGD) optimizer with an initial learning rate of $1.0\mathrm{e}{-3}$, momentum of $0.95$, and an exponential decay-rate of $0.5$ for every $2$ epochs. 
% We let the FFE train until its training loss stopped improving, then discarded the classification output layer. 
After pretraining the FFE, we trained the entire network following the five stages described in Section \ref{subsec:training_protocol} with different training parameters shown in Table \ref{table:training_stages_parameters}. Throughout the stages, we set $\alpha = 0.4$.
%, and we stop training when validation loss stop decreasing. 
%After training, we evaluate the performance of our proposed approach as shown in the following.

\subheader{Evaluation Datasets} 
%We evaluated the frame-level performance of our proposed network on videos from Set A's testing set and Set B.
We evaluated the frame-level performance of our proposed network and competing networks  on the six datasets described in Section~\ref{sec:training_datasets}.



\begin{comment}
We evaluated the performance of our proposed network on multiple video datasets. These datasets are divided into two groups. Group A consists of videos that has been seen by the model during training, which consists of test sets of VCMS, the VPVM, and the VPIM dataset.  Group B consists of ``in-the-wild'' videos that have manipulations and edited content that were never seen by the model during training, which consists of the VideoSham, VideoMatting and Inpainted Video dataset. Group B dataset are only used for evaluation.

[Might need Revision, VideoMatting]

The VideoSham dataset \citelater{cite} is made by Adobe Research, which contains high-quality videos manipulated by professional editors. Because this work focuses exclusively on identifying fake content, we excluded videos' audio and those with temporal manipulations. Additionally, videos of resolution less than our network's input size $1080 \times 1920$ were also excluded. 

The VideoMatting dataset \citelater{cite} has videos consisting of a subject or object in the foreground and background, which is matted (replaced) using video matting algorithms.

The Inpainted Video dataset is created by applying E2FGVI-HQ \citelater{cite} to remove segmented objects, which are specified in the Densely Annotated Video Segmentation (DAVIS) dataset \citelater{cite}. Using the authors' recommended settings, we generate 540p videos then resize them to 1080p so that they can be analyzed by our network. Note that resizing has been proven by prior works \citelater{cite} to have a great influence upon the forensic traces in the original frame. Hence, this is an important source of data distribution mismatch that we will explore in the sections below.
\end{comment}

%\input{tables/summary_test_datasets}

\subheader{Evaluation Metrics} 
For frame-level manipulation detection, we report the mean average precision (mAP) for each dataset. Also, we provide the average accuracy (ACC) per datasets using a unified threshold of 0.5 to reflect real-world's performance.
%
For forgery localization (i.e. pixel-level manipulation detecton) we %pick 0.5 as the threshold and 
use F1 and MCC scores to evaluate the correlation between the  ground-truth and predicted masks, which are binarized with a threshold of~0.5. 
%Since these scores describe the localization performance, they are only evaluated on manipulated samples. 






==> sections/revisions_old/05_experimental_setup_v3_Shengbang.tex <==
% 05_experimental_setup_v2_MCS

\subsection{Experimental Setup}
\label{subsec:experimental_setup}

\subheader{Training Implementation} We implemented our network using PyTorch and trained it using an NVIDIA RTX 3090. The network input size is $1080 \times 1920$ pixels %($\text{height} \times \text{width}$). 
(a single 1080p frame).  
We first pre-trained the FFE on the Video-ACID dataset using the Stochastic Gradient Descent (SGD) optimizer with an initial learning rate of $1.0\mathrm{e}{-3}$, momentum of $0.95$, and an exponential decay-rate of $0.5$ for every $2$ epochs. We let the FFE train until its training loss stopped improving, then discarded the classification output layer. 
After pretraining the FFE, we trained the entire network following the five stages described in Section \ref{subsec:training_protocol} with different training parameters shown in Table \ref{table:training_stages_parameters}. Throughout the stages, we set $\lambda = 0.4$, and we stop training when validation loss stop decreasing. After training, we evaluate the performance of our proposed approach as shown in the following.

\subheader{Evaluation Datasets} 
%We evaluated the frame-level performance of our proposed network on videos from Set A's testing set and Set B.
We evaluated the %frame-level 
performance of our proposed network and 
%competing
several existing image forensic 
networks on the six datasets described in Section~\ref{sec:training_datasets}.



\begin{comment}
We evaluated the performance of our proposed network on multiple video datasets. These datasets are divided into two groups. Group A consists of videos that has been seen by the model during training, which consists of test sets of VCMS, the VPVM, and the VPIM dataset.  Group B consists of ``in-the-wild'' videos that have manipulations and edited content that were never seen by the model during training, which consists of the VideoSham, VideoMatting and Inpainted Video dataset. Group B dataset are only used for evaluation.

[Might need Revision, VideoMatting]

The VideoSham dataset \citelater{cite} is made by Adobe Research, which contains high-quality videos manipulated by professional editors. Because this work focuses exclusively on identifying fake content, we excluded videos' audio and those with temporal manipulations. Additionally, videos of resolution less than our network's input size $1080 \times 1920$ were also excluded. 

The VideoMatting dataset \citelater{cite} has videos consisting of a subject or object in the foreground and background, which is matted (replaced) using video matting algorithms.

The Inpainted Video dataset is created by applying E2FGVI-HQ \citelater{cite} to remove segmented objects, which are specified in the Densely Annotated Video Segmentation (DAVIS) dataset \citelater{cite}. Using the authors' recommended settings, we generate 540p videos then resize them to 1080p so that they can be analyzed by our network. Note that resizing has been proven by prior works \citelater{cite} to have a great influence upon the forensic traces in the original frame. Hence, this is an important source of data distribution mismatch that we will explore in the sections below.
\end{comment}

%\input{tables/summary_test_datasets}

\subheader{Evaluation Metrics} 
For frame-level manipulation detection, we report the mean average precision (mAP) for each dataset. Also, we provide the average accuracy (ACC) per datasets using a unified threshold of 0.5 to reflect real-world's performance.

For forgery localization (i.e. pixel-level manipulation detecton) we %pick 0.5 as the threshold and 
use F1 and MCC scores to evaluate the correlation between the  ground-truth and predicted localization masks, which are binarized with a threshold of 0.5. Since these scores describe the localization performance, they are only evaluated on manipulated samples. 



\input{tables/training_stages_params}

\input{tables/results_vcms_vpvm_vpim}

\input{tables/results_in_the_wild}


==> sections/revisions_old/05_experiments_v1.tex <==
\section{Experiments}
\label{sec:experiments}


==> sections/revisions_old/05_proposed_perf_v1.tex <==
\subsection{Proposed Network's Performance}
\label{subsec:proposed_network_performance}

We evaluated our proposed algorithm on datasets in group A and B. As we have seen in Table \ref{table:results_on_our_datasets}, which shows the performance on datasets in group A, our network displays very strong detection and localization performance across all three datasets in group A. Particularly, on VCMS and VPVM, the detection mAPs are above 0.98, and the localization F1s are above 0.52. Although there is a slight performance drop regarding the VPIM dataset, this is expected because the level of manipulation is so minute that it is not visible to the human eye. Furthermore, this degree of alteration is unlikely to be applied in practice because real forgeries need to have a perceptual effect.

In Table \ref{table:results_on_itw_datasets}, we again see strong performance among the ``in-the-wild'' datasets. For example, we obtained a detection mAP of 0.691 on VideoSham and 0.782 on Inpainted Video. Note that our model's results on group B datasets are lower than those in group A, but this is anticipated as we explicitly did not train on them. Our network has never seen these types of tampering operations or any of these data distributions. Therefore, this shows that our method is highly transferable to data from other sources with other manipulations.

Specifically on VideoSham, we notice that many forgeries are very small, i.e., on the order of tens of pixels - much smaller than our analysis window (and below the minimum size that many algorithms are able to resolve). Therefore, considering this dataset's high-level of difficulty, we still attained good detection and localization performance. This is very significant because the authors of this dataset found that both existing algorithms and human evaluators they benchmarked against did no better than random guess (similar to what we see here).
% - if we have the table of detection vs. forgery size, it would be good to reference here

On the Inpainted Video dataset, we see lower performance due to the distributional mismatch: all videos are resized. Resizing is well known throughout forensics to degrade the performance of forensic algorithms. Despite this and the fact that our network has never seen inpainted videos before, we were still able to detect and localize fake contents in these videos. This proves that our proposed approach is performant and highly transferable.

Regarding the VideoMatting dataset, ....
% - need to understand performance of video matting

% Need to interpret these results here, and probably reference a figure that we have not yet made with all of the images of identification resutls.



==> sections/revisions_old/05_proposed_perf_v1_Shengbang.tex <==
\subsection{Proposed Network's Performance}
\label{subsec:proposed_network_performance}

%We evaluated our proposed algorithm on datasets in group A and B. 
We evaluate our proposed approach on both group A and B datasets, and compare the results with other competing image-based anomaly detection adn localization algorithms. 
%As we have seen in Table \ref{table:results_on_our_datasets}, which shows the performance on datasets in group A, our network displays very strong detection and localization performance across all three datasets in group A. 
The results on seen manipulation in Group A are shown in Table \ref{table:results_on_our_datasets} and the results on "in-the-wild" videos in Group B are shown in Table \ref{table:results_on_itw_datasets}.
Through Table \ref{table:results_on_our_datasets} we show that our proposed approach achieve a strong performance and outperform all other competing algorithms. Though our model performance drop in invisible manipulations in VPIM, it can still have a mAP of 0.869 for detection and a F-1 score of 0.547 for localization. This is consistent with our expectation, since the manipulation is in small scale and has highest difficulty to learn by the model. 
While our performance are high, these competing algorithms cannot detect and localize the manipulated content in the videos and performs close to random guess. These results are consistent with the difference compression method between images and videos. 

%Particularly, on VCMS and VPVM, the detection mAPs are above 0.98, and the localization F1s are above 0.52. 
%Although there is a slight performance drop regarding the VPIM dataset, this is expected because the level of manipulation is so minute that it is not visible to the human eye. 
%Furthermore, this degree of alteration is unlikely to be applied in practice because real forgeries need to have a perceptual effect.

%In the  Table \ref{table:results_on_itw_datasets}, we again see strong performance among the ``in-the-wild'' datasets. 
For the "in-the-wild" videos, through Table \ref{table:results_on_itw_datasets} we show our proposed method transfer to the "in-the-wild" manipulated videos.
For example, we obtained a detection mAP of 0.691 on VideoSham and 0.782 on Inpainted Video. 
%Note that our model's results on group B datasets are lower than those in group A, but this is anticipated as we explicitly did not train on them. 
These index are lower than those in group A, but this is anticipated as we did not explicitly train on these datasets with different scenes and contents distribution. 
\citelater{Need Results}

%Our network has never seen these types of tampering operations or any of these data distributions. 
Therefore, this shows that our method is highly transferable to data from other sources with other manipulations.

Specifically on VideoSham, we notice that many forgeries are very small, i.e., on the order of tens of pixels - much smaller than our analysis window (and below the minimum size that many algorithms are able to resolve). Therefore, considering this dataset's high-level of difficulty, we still attained good detection and localization performance. This is very significant because the authors of this dataset found that both existing algorithms and human evaluators they benchmarked against did no better than random guess (similar to what we see here).
% - if we have the table of detection vs. forgery size, it would be good to reference here

On the Inpainted Video dataset, we see lower performance due to the distributional mismatch: all videos are resized. Resizing is well known throughout forensics to degrade the performance of forensic algorithms. Despite this and the fact that our network has never seen inpainted videos before, we were still able to detect and localize fake contents in these videos. This proves that our proposed approach is performant and highly transferable.

Regarding the VideoMatting dataset, ....
% - need to understand performance of video matting

% Need to interpret these results here, and probably reference a figure that we have not yet made with all of the images of identification resutls.



==> sections/revisions_old/06_ablation_study_v1.tex <==
\section{Ablation Study}
\label{sec:ablation_study}

We conducted multiple ablation experiments to validate the design choices of various components in our network and reveal the importance of these components on the overall architecture. First, we show the necessity of low-level feature extractors - the Forensic Feature Extractor (FFE) and the Contextual Feature Extractor (CFE). Second, we demonstrate that the Transformer-Based Attention Module provides a significant performance boost and strong generalizability. Finally, we justify our proposed approach when combining the transformer's attention map and the spatially contextualized forensic features. For a fair comparison, we trained each of the proposed model's variants with the same training protocol specified in section \ref{subsec:training_protocol} and assessed their performance on VideoSham. The summary of our experiments is shown in Table \ref{table:ablation_evaluations}.

%  to judge their ability to generalize over manipulations not seen during training and different data distributions. Overall, our goal is to find the architectural design that has the highest level of generalizability

\input{tables/results_ablations}

\subheader{Influence of FFE}
Comparing no FFE with our proposed approach, we see that the detection mAP drops from 0.691 to 0.646 and localization F1 from 0.258 to 0.209. Therefore, the FFE is necessary to boost both overall performance and increase the model's generalizability.

\subheader{Influence of CFE}
Without the CFE, we observe a significant reduction in performance in every metric. This result shows that contextual information is crucial in the network getting a more comprehensive picture of the forensic information contained in the input frame.

% For example, on VideoSham, the detection mAP drops from 0.691 to 0.635 and localization F1 on from 0.258 to 0.163. 

\subheader{Influence of the Transformer-Based Attention Module}
In this model variant, we remove the entire Transformer-Based Attention Module. Hence, the contextualized forensic embeddings are fed directly into the detector and the localizer networks. This variant results in a substantial performance drop across the board. On VideoSham, the detection metrics suggest that this network only does slightly better than random guessing. Therefore, the Transformer-Based Attention Module is pivotal in 1) analyzing and transforming spatial, contextual, and forensic information and 2) producing the attention maps for downstream analysis. 

\subheader{Influence of the Transformer}
We measure the importance of the Transformer itself by replacing it with six fully connected layers with ReLU as the activation function. In this scenario, the model performs at level close to random guessing. Therefore, this cements the necessity of the Transformer for our network.

\subheader{Influence of the Attention Squeeze}
In this scenario, we connect the output of the Transformer directly to the detector and localizer, bypassing the Attention Squeeze component. From Table \ref{table:ablation_evaluations}, we see that this variant underperforms in both detection and localization. In particular, the detection mAP drops from 0.691 to 0.656 and the localization MCC drops from 0.168 to 0.120. Hence, the Attention Squeeze component is essential in boosting the model's generalizability. We also try 1, 3 (proposed) and 10 attention maps, the results shows that the 3 attention maps yields the best performance.

% Since the Transformer network transforms the spatially contextualized features using deep self-attention blocks, it is interesting to gauge the performance of only using these transformed embeddings for detection and localization

\subheader{Influence of different feature fusion approaches}
Instead of the proposed fusion method, we concatenate all three sets of weighted spatially contextualized forensic embeddings. Table \ref{table:ablation_evaluations} shows that this variant achieves strong performance across the board but falls short in VideoSham. Although the detection performance is similar to the proposed network, the localization metrics both drop significantly (i.e., F1 dropping from 0.258 to 0.162 and MCC from 0.168 to 0.091). Therefore, the proposed method is optimal for generalizability.


==> sections/revisions_old/06_ablation_study_v1_Shengbang.tex <==
\section{Ablation Study}
\label{sec:ablation_study}

%We conducted multiple ablation experiments to validate the design choices of various components in our network and reveal the importance of these components on the overall architecture.
We conducted multiple ablation experiments to validate 
%the design choices of various components in our network and reveal 
the importance of various components in VideoFACT's architecture. 
%First, we show the necessity of the FFE and the CFE. Second, we demonstrate that the Transformer-Based Attention Module provides a significant performance boost and strong generalizability. Finally, we justify our proposed approach when combining the transformer's attention map and the spatially contextualized forensic features. For a fair comparison, we
We trained each of the network variants using the same settings as the proposed method and assessed their performance on VideoSham. 
A summary of our experiments is shown in Table \ref{table:ablation_evaluations}.

%  to judge their ability to generalize over manipulations not seen during training and different data distributions. Overall, our goal is to find the architectural design that has the highest level of generalizability

\input{tables/results_ablations}

\subheader{Influence of FFE}
Removing FFE, we see the detection mAP drops from 0.691 to 0.646 and localization F1 from 0.258 to 0.209. This shows that the FFE is necessary to boost both performance and generalizability.

\subheader{Influence of CFE}
Without the CFE, every metric has a significant reduction. This shows that contextual information is crucial in the network getting a more comprehensive picture of the video forensic information.

% For example, on VideoSham, the detection mAP drops from 0.691 to 0.635 and localization F1 on from 0.258 to 0.163. 

\subheader{Influence of the Transformer-Based Attention Module}
In this model variant, we removed the entire Transformer-Based Attention Module. The joint embeddings were fed directly into the detector and the localizer networks. This variant resulted in a substantial performance drop across the board. The detection metrics suggest that this network only does slightly better than random guess. Therefore, this module is a critical part of VideoFACT.

\subheader{Influence of the Transformer}
We measure the importance of the Transformer itself by replacing it with six fully connected layers with ReLU as the activation function. In this scenario, the model performs at a level close to random guess. Therefore, this cements the necessity of the Transformer for our network.

\subheader{Influence of the Attention Squeeze}
In this scenario, we connect the output of the Transformer directly to the detector and localizer, bypassing the Attention Squeeze component. From Table \ref{table:ablation_evaluations}, we see that this variant underperforms in both detection and localization. Hence, the Attention Squeeze component is essential in boosting the model's generalizability. We also try using 1, 3 (proposed) and 10 attention maps.  Results show that using 3 attention maps yields the best performance.

% Since the Transformer network transforms the spatially contextualized features using deep self-attention blocks, it is interesting to gauge the performance of only using these transformed embeddings for detection and localization

\subheader{Influence of different Feature Refinement approaches}
Instead of the proposed approach, we concatenate all three sets of weighted spatially contextualized forensic embeddings. Results show that both detection and localization performance drop significantly. Therefore, the proposed method is the optimal choice.


==> sections/revisions_old/07_conclusion_v1.tex <==
\section{Conclusion}
\label{sec:conclusion}
% new approach
In this paper, we proposed a new network that can detect and localize a broad range of video manipulations.
% method
We do this by combining forensic, context and spatial embeddings, extracted over a video frame, and using a deep attention mechanism to emphasize or de-emphasize regions depending on the quality and quantity of their forensic information. This allows our network to achieve strong performance and a high degree of generalizability. 
% We also propose a new dataset
To train and evaluate our model, we also create a new dataset contains diverse types and strengths of manipulation.
% we demonstrate we can detect video manipulation, and provide visual results and exp
Through multiple experiments and examples, we show that our approach can successfully detect and localize video forgery in both the Standard Video Manipulations datasets and the ``in-the-wild'' datasets.
% our approach overcome vidoe compression and low false alarm due to inconsistent quality
With examples, we show that our approach can handle video compression and inconsistent forensic quality, which can causes false alarm in previous image-based forgery detection and localization algorithms.
% we show the approch architecture nessary through ablation study.
Finally, we demonstrate the necessity of each designed component through an extensive series of ablation studies.


==> sections/revisions_old/07_conclusion_v2_MCS.tex <==
\section{Conclusion}
\label{sec:conclusion}
% new approach


In this paper, we propose a new network, VideoFACT, to detect and localize a broad range of video forgeries and manipulations.   Our network does this by utilizing both forensic embeddings to capture traces left by manipulation, context embeddings to exploit forensic traces' conditional dependencies upon scene content, and spatial attention provided by a deep, transformer-based attention mechanism.
%
We creates several new video forgery datasets, which we used along with the Adobe VideoSham dataset to experimentally evaluate our network's performance.
Our results show that our proposed network is able to identify a diverse set of video forgeries, including those not encountered during training.  Furthermore, our results show that existing image forensic networks largely fail to identify fake content in video.


%In this paper, we proposed a new network that can detect and localize a broad range of video manipulations.We do this by combining forensic, context and spatial embeddings, extracted over a video frame, and using a deep attention mechanism to emphasize or de-emphasize regions depending on the quality and quantity of their forensic information. This allows our network to achieve strong performance and a high degree of generalizability. 
% We also propose a new dataset
%To train and evaluate our model, we also create a new dataset contains diverse types and strengths of manipulation.
% we demonstrate we can detect video manipulation, and provide visual results and exp
%Through multiple experiments and examples, we show that our approach can successfully detect and localize video forgery in both the Standard Video Manipulations datasets and the ``in-the-wild'' datasets.
% our approach overcome vidoe compression and low false alarm due to inconsistent quality
%With examples, we show that our approach can handle video compression and inconsistent forensic quality, which can causes false alarm in previous image-based forgery detection and localization algorithms.
% we show the approch architecture nessary through ablation study.
%Finally, we demonstrate the necessity of each designed component through an extensive series of ablation studies.


==> tables/results_joined_all_ds.tex <==
\begin{table*}[!t]

	\vspace*{-0.5\baselineskip}

    \centering
    \setlength\extrarowheight{-1.7pt}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{
        >{\hspace{0pt}}m{0.150\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        >{\hspace{0pt}}m{0.000\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        >{\hspace{0pt}}m{0.000\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        |>{\hspace{0pt}}m{0.000\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        >{\hspace{0pt}}m{0.000\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        >{\hspace{0pt}}m{0.000\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
        >{\hspace{0pt}}m{0.055\linewidth}
    } 
        \hline

        \multicolumn{1}{>{\hspace{0pt}}m{0.100\linewidth}}{\multirow{2}{0.700\linewidth}{\hspace{0pt}\Centering{}\textbf{Method}}} & 
        \multicolumn{3}{>{\Centering\hspace{-27pt}}m{0.150\linewidth}}{\textbf{VCMS}} &  & 
        \multicolumn{3}{>{\Centering\hspace{-27pt}}m{0.150\linewidth}}{\textbf{VPVM}} &  & 
        \multicolumn{3}{>{\Centering\hspace{-27pt}}m{0.150\linewidth}|}{\textbf{VPIM}} & 
        
        &
        \multicolumn{3}{>{\Centering\hspace{-27pt}}m{0.150\linewidth}}{\textbf{Deepfake Video}} &  & 
        \multicolumn{3}{>{\Centering\hspace{-27pt}}m{0.150\linewidth}}{\textbf{Inpainted Video}} &  & 
        \multicolumn{3}{>{\Centering\hspace{-27pt}}m{0.150\linewidth}}{\textbf{VideoSham}} \\

        \cline{2-4}\cline{6-8}\cline{10-12}\cline{13-16}\cline{18-20}\cline{22-24}

        \multicolumn{1}{>{\Centering\hspace{0pt}}m{0.040\linewidth}}{} & 
        \textit{Det. mAP} & \textit{Loc. MCC} & \textit{Loc. F1} &  & 
        \textit{Det. mAP} & \textit{Loc. MCC} & \textit{Loc. F1} &  & 
        \textit{Det. mAP} & \textit{Loc. MCC} & \textit{Loc. F1} &  & 
        \textit{Det. mAP} & \textit{Loc. MCC} & \textit{Loc. F1} &  & 
        \textit{Det. mAP} & \textit{Loc. MCC} & \textit{Loc. F1} &  & 
        \textit{Det. mAP} & \textit{Loc. MCC} & \textit{Loc. F1} \\ 

        \hline

        FSG \citelater{cite} 
        & 0.445 & 0.001 & 0.064 & 
        & 0.431 & 0.004 & 0.067 & 
        & 0.485 & 0.011 & 0.065 & 
        & 0.450 & 0.204 & 0.137 & 
        & 0.386 & 0.208 & 0.302 & 
        & 0.596 & 0.162 & 0.246 \\
        EXIFnet \citelater{cite} 
        & 0.610 & 0.208 & 0.230 & 
        & 0.568 & 0.213 & 0.236 & 
        & 0.509 & 0.026 & 0.124 & 
        & 0.447 & 0.180 & 0.133 & 
        & 0.635 & 0.160 & 0.244 & 
        & 0.584 & 0.148 & 0.246 \\ 
        Noiseprint \citelater{cite} 
        & 0.521 & 0.041 & 0.030 & 
        & 0.495 & 0.012 & 0.013 & 
        & 0.511 & 0.010 & 0.010 & 
        & 0.591 & 0.010 & 0.062 & 
        & 0.601 & 0.091 & 0.232 & 
        & 0.422 & 0.034 & 0.206 \\ 
        ManTra-Net \citelater{cite} 
        & 0.451 & 0.079 & 0.114 & 
        & 0.526 & 0.110 & 0.145 & 
        & 0.513 & 0.025 & 0.064 & 
        & 0.450 & 0.004 & 0.042 & 
        & 0.499 & 0.009 & 0.055 &
        & 0.551 & 0.009 & 0.058 \\  
        MVSS-Net \citelater{cite} 
        & 0.883 & \textbf{0.545} & \textbf{0.557} & 
        & 0.644 & 0.267 & 0.279 & 
        & 0.482 & 0.018 & 0.042 & 
        & 0.464 & 0.199 & 0.189 & 
        & 0.341 & 0.058 & 0.227 & 
        & 0.595 & 0.142 & 0.096 \\ 

        \hline

        \textbf{Ours} 
        & \textbf{0.995} & 0.530          & 0.526          & 
        & \textbf{0.980} & \textbf{0.676} & \textbf{0.697} & 
        & \textbf{0.869} & \textbf{0.515} & \textbf{0.547} & 
        & \textbf{0.666} & \textbf{0.415} & \textbf{0.410} &  
        & \textbf{0.782} & \textbf{0.225} & \textbf{0.309} &
        & \textbf{0.691} & \textbf{0.193} & \textbf{0.312} \\  

        \hline
    \end{tabular}
    }

	\vspace*{-0.5\baselineskip}    
    
    \caption{\label{table:results_on_all_datasets} Frame-level and pixel-level performance on all datasets in Group A - VCMS, VPVM, VPIM and Group B - Deepfake Video, Inpainted Video \citelater{cite}, VideoSham \citelater{cite}}
    
    \vspace*{-0.5\baselineskip}
    
\end{table*}

